Certified Everlasting Functional Encryption

Computational security in cryptography has a risk that computational assumptions underlying the security are broken in the future. One solution is to construct information-theoretically-secure protocols, but many cryptographic primitives are known to be impossible (or unlikely) to have information-theoretical security even in the quantum world. A nice compromise (intrinsic to quantum) is certified everlasting security, which roughly means the following. A receiver with possession of quantum encrypted data can issue a certificate that shows that the receiver has deleted the encrypted data. If the certificate is valid, the security is guaranteed even if the receiver becomes computationally unbounded. Although several cryptographic primitives, such as commitments and zero-knowledge, have been made certified everlasting secure, there are many other important primitives that are not known to be certified everlasting secure. In this paper, we introduce certified everlasting FE. In this primitive, the receiver with the ciphertext of a message m and the functional decryption key of a function f can obtain f(m) and nothing else. The security holds even if the adversary becomes computationally unbounded after issuing a valid certificate. We, first, construct certified everlasting FE for P/poly circuits where only a single key query is allowed for the adversary. We, then, extend it to q-bounded one for NC1 circuits where q-bounded means that q key queries are allowed for the adversary with an a priori bounded polynomial q. For the construction of certified everlasting FE, we introduce and construct certified everlasting versions of secret-key encryption, public-key encryption, receiver non-committing encryption, and a garbling scheme, which are of independent interest.

==> Old_FE.tex <==
\subsection{Construction of Single-Key Certified Everlasting Functional Encryption with Adaptive Security}\label{sec:const_fe_adapt}
In this section, we present how to construct a single-key certified everlasting functional encryption scheme with adaptive security from a certified everlasting functional encryption scheme with non-adaptive security and a certified everlasting RNC scheme.

\paragraph{Our single-key certified everlasting FE scheme with adaptive security.}
In this section, we present how to construct a single-key certified everlasting functional encryption scheme with adaptive security $\Sigma_{\mathsf{cefe}}=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$ from a single-key certified everlasting functional encryption scheme with non-adaptive security
$\Sigma_{\mathsf{nad}}=\mathsf{NAD}.(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$
and a certified everlasting RNCE scheme for quantum message $\Sigma_{\mathsf{cence}}=\NCE.(\Setup,\keygen,\Enc,\Dec,\Fake,\Reveal,\Delete,\Vrfy)$.
\begin{description}
\item[$\Setup(1^\secp)$:]$ $
\begin{itemize}
    \item Generate $(\mathsf{nad}.\MPK,\mathsf{nad}.\MSK)\la\mathsf{NAD}.\Setup(1^\secp)$.
    \item Generate $(\nce.\pk,\nce.\sk,\nce.\MSK)\la\NCE.\Setup(1^{\secp})$.
    \item Output $\MPK\seteq(\nce.\pk,\mathsf{nad}.\MPK)$ and $\MSK\seteq (\nce.\MSK,\mathsf{nad}.\MSK)$.
\end{itemize}
\item[$\keygen(\MSK,f)$:]$ $
\begin{itemize}
    \item Parse $\MSK=(\nce.\MSK,\mathsf{nad}.\MSK)$.
    \item Compute $\mathsf{nad}.\sk_f\la\mathsf{NAD}.\keygen(\mathsf{nad}.\MSK,f)$.
    \item Compute $\nce.\sk\la\NCE.\keygen(\nce.\MSK)$.
    \item Output $\sk_f\seteq (\nce.\sk,\mathsf{nad}.\sk_f)$.
\end{itemize}
\item[$\Enc(\MPK,m)$:]$ $
\begin{itemize}
    \item Parse $\MPK=(\nce.\pk,\mathsf{nad}.\MPK)$.
    \item Compute $(\mathsf{nad}.\vk,\mathsf{nad}.\ct)\la\mathsf{NAD}.\Enc(\mathsf{nad}.\MPK,m)$.
    \item Compute $(\nce.\vk,\nce.\ct)\la\NCE.\Enc(\nce.\pk,\mathsf{nad}.\ct)$.
    \item Output $\vk\seteq(\mathsf{nad}.\vk,\nce.\vk)$ and $\ct\seteq \nce.\ct$.
\end{itemize}
\item[$\Dec(\sk_f,\ct)$:]$ $
\begin{itemize}
    \item Parse $\sk_f=(\nce.\sk,\mathsf{nad}.\sk_f)$ and $\ct=\nce.\ct$.
    \item Compute $\mathsf{nad}.\ct^*\la\NCE.\Dec(\nce.\sk,\nce.\ct)$.
    \item Compute $y\la\mathsf{NAD}.\Dec(\mathsf{nad}.\sk_f,\mathsf{nad}.\ct^*)$.
    \item Output $y$.
\end{itemize}
\item[$\Delete_0(\ct)$:]$ $
\begin{itemize}
    \item Parse $\ct=\nce.\ct$.
    \item Compute $\nce.\cert_0\la\NCE.\Delete_0(\nce.\ct)$.
    \item Output $\cert_0\seteq\nce.\cert_0$.
\end{itemize}
\item[$\Delete_1(\sk_f,\ct)$:]$ $
\begin{itemize}
    \item Parse $\sk_f=(\nce.\sk,\mathsf{nad}.\sk_f)$ and $\ct=\nce.\ct$.
    \item Compute $(\mathsf{nce}.\cert_1,\mathsf{nad}.\ct^*)\la\NCE.\Delete_1(\nce.\ct,\nce.\sk)$.
    \item Compute $\mathsf{nad}.\cert\la\mathsf{NAD}.\Delete(\mathsf{nad}.\ct^*)$.
    \item Output $\cert_1\seteq(\mathsf{nad}.\cert,\nce.\cert_1)$.
\end{itemize}
\item[$\Vrfy_0(\vk,\cert_0)$:]$ $
\begin{itemize}
    \item Parse $\vk=(\mathsf{nad}.\vk,\nce.\vk)$ and $\cert_0=\nce.\cert_0$.
    \item Output $\top$ if $\top\la\NCE.\Vrfy_0(\nce.\vk,\nce.\cert_0)$.
    Otherwise, output $\bot$.
\end{itemize}
\item[$\Vrfy_1(\vk,\sk_f,\cert)$:]$ $
\begin{itemize}
    \item Parse $\vk=(\mathsf{nad}.\vk,\nce.\vk)$ and $\cert=(\mathsf{nad}.\cert_1,\nce.\cert_1)$.
    \item Output $\top$ if $\top\la\mathsf{NAD}.\Vrfy_1(\mathsf{nad}.\vk,\mathsf{nad}.\cert_1)$ and $\top\la\NCE.\Vrfy_1(\nce.\vk,\nce.\sk_f,\nce.\cert_1)$.
    Otherwise, output $\bot$.
    \end{itemize}
\end{description}
\paragraph{Correctness:}
Decryption correctness easily follows from decryption correctness of $\Sigma_{\mathsf{nad}}$ and $\Sigma_{\mathsf{cence}}$.
Verification correctness easily follows from decryption correctness of $\Sigma_{\mathsf{nad}}$ and verification correctness $\Sigma_{\mathsf{cence}}$.
\paragraph{Security:}
We prove the following two theorems.
\begin{theorem}\label{thm:comp_security_single_ad}
If $\Sigma_{\mathsf{nad}}$ satisfies the single-key non-adaptive security and $\Sigma_{\mathsf{cence}}$ satisfies the RNC security, 
$\Sigma_{\mathsf{cefe}}$ satisfies the single-key adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:comp_security_single_ad}]
The proof is similar to that of \cref{thm:comp_security_single_ad}.
\end{proof}

\begin{theorem}\label{thm:ever_security_single_ad}
If $\Sigma_{\mathsf{nad}}$ satisfies the single-key certified everlasting non-adaptive security and $\Sigma_{\mathsf{cence}}$ satisfies the certified everlasting RNC security, 
$\Sigma_{\mathsf{cefe}}$ satisfies the single-key certified everlasting adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:ever_security_single_ad}]
Obviously, the security holds against an adversary which makes an function query before it makes a challenge query.
This is because $\Sigma_{\mathsf{nad}}$ is single-key certified everlasting non-adaptive secure.
Hence, we consider the adversary $\cA$ which makes an function query after it makes a challenge query.
For clarity, we describe how the experiment works against the adversary $\cA\seteq(\cA_1,\cA_2)$
consisting of any QPT adversary $\cA_1$ and any unbounded time adversary $\cA_2$.
\begin{description}
\item[$\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)$:]This is the original experiment.
\begin{enumerate}
    \item The challenger generates $(\mathsf{nad}.\MPK,\mathsf{nad}.\MSK)\la\mathsf{NAD}.\Setup(1^\secp)$ and $(\nce.\pk,\nce.\MSK)\la\NCE.\Setup(1^{\secp})$, and sends $(\nce.\pk,\mathsf{nad}.\MPK)$ to $\cA_1$.
    \item $\cA_1$ submits a message pair $(m_0,m_1)\in\Ms$ to the challenger.
    The challenger computes 
    $(\mathsf{nad}.\vk,\mathsf{nad}.\CT)\la \mathsf{NAD}.\Enc(\mathsf{nad}.\MPK,m_b)$ and 
    $(\nce.\vk,\nce.\ct)\la\NCE.\Enc(\nce.\pk,\mathsf{nad}.\ct)$,
    and sends $\nce.\CT$ to $\cA_1$.
    \item $\cA_1$ is allowed to make arbitrary an function query at most one time.
    For the function query, the challenger receives $f\in\mathcal{F}$,  
    computes $\nce.\sk\la\NCE.\keygen(\nce.\MSK)$
    and $\mathsf{nad}.\sk_{f}\la\mathsf{NAD}.\keygen(\mathsf{nad}.\MSK,f)$,
    and sends $(\nce.\sk,\mathsf{nad}.\sk_{f})$ to $\cA_1$.
    Let $j$ be the number of times $\cA_1$ has made key queries.
    \item $\cA_1$ does the following.
    \begin{itemize}
        \item If $j=0$, $\cA_1$ sends $\nce.\cert_0$ to the challenger and its internal state to $\cA_2$.
        \item If $j=1$, $\cA_1$ sends $(\nce.\cert_1,\mathsf{nad}.\cert)$ to the challenger and its internal state to $\cA_2$.
    \end{itemize}
    \item The challenger does the following.
    \begin{itemize}
        \item If $j=0$, the challenger computes $\NCE.\Vrfy(\nce.\vk,\nce.\cert_0)$.
        If the result is $\bot$, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
        Otherwise, the challenger outputs $\top$ and sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
        \item If $j=1$, the challenger computes $\NCE.\Vrfy(\nce.\vk,\nce.\sk,\nce.\cert_1)$ and $\mathsf{NAD}.\Vrfy(\mathsf{nad}.\vk,\mathsf{nad}.\cert)$.
        If the results are $\bot$, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
        Otherwise, the challenger outputs $\top$ and sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
    \end{itemize}
    \item $\cA_2$ outputs $b'$.
    \item The experiment outputs $b'$ if $f(m_0)=f(m_1)$ and the challenger outputs $\top$. Otherwise,the experiment outputs $\bot$.
\end{enumerate}
What we have to prove is that 
\begin{align}
    \advc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp)
\seteq \abs{\Pr[ \expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, 0)=1] - \Pr[ \expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, 1)=1] }\leq \negl(\secp).
\end{align}
We define the following sequence of hybrids.
\item[$\sfhyb{1}{}(b)$:] $ $
This is identical to $\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, b)$ except for the following two points. 
First, the challenger computes $(\nce.\vk,\widetilde{\nce.\ct},\nce.\aux)\la\NCE.\Fake(\nce.\pk,\nce.\MSK)$ instead of computing $(\nce.\vk,\nce.\ct)\la\NCE.\Enc(\nce.\pk,\mathsf{nad}.\ct)$.
Second, the challenger computes $\widetilde{\nce.\sk}\la \NCE.\Reveal(\nce.\pk,\nce.\MSK,\nce.\aux,\mathsf{nad}.\ct)$ instead of computing $\nce.\sk\la\NCE.\keygen(\nce.\MSK)$.
\end{description}
\cref{thm:ever_security_single_ad} easily follows from \cref{prop:exp_hyb_1_cefe_si_ad} and \cref{prop:hyb_1_hyb_2_cefe_si_ad}.
(Whose proof is given later.)
\end{proof}

\begin{proposition}\label{prop:exp_hyb_1_cefe_si_ad}
If $\Sigma_{\mathsf{cence}}$ is certified everlasting RNC secure, 
it holds that
\begin{align}
\abs{\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]-\Pr[\sfhyb{1}{}(b)=1]}\leq\negl(\secp)
\end{align}
for $b\in\bit$.
\end{proposition}

\begin{proposition}\label{prop:hyb_1_hyb_2_cefe_si_ad}
If $\Sigma_{\mathsf{nad}}$ is single-key certified everlasting non-adaptive secure,
it holds that
\begin{align}
    \abs{\Pr[\sfhyb{1}{}(0)=1]-\Pr[\sfhyb{1}{}(1)=1]}\leq\negl(\secp).
\end{align}
\end{proposition}

\begin{proof}[Proof of \cref{prop:exp_hyb_1_cefe_si_ad}]
We assume that $\abs{\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is non-negligible, and consruct an adversary $\cB$ that breaks the certified everlasting RNC security of $\Sigma_{\mathsf{cefe}}$.
Let us describe how $\cB$ works below.
\begin{enumerate}
    \item $\cB$ receives $\nce.\pk$ from the challenger of $\expd{\Sigma_{\mathsf{cence}},\cB}{cert}{ever}{rec}{nc}(\secp,b')$,
    generates $(\mathsf{nad}.\MPK,\mathsf{nad}.\MSK)\la \mathsf{NAD}.\keygen(1^\secp)$,
    and sends $(\nce.\pk,\mathsf{nad}.\MPK)$ to $\cA_1$.
    \item $\cB$ receives a message pair $(m_0,m_1)\in\Ms$, computes $(\mathsf{nad}.\vk,\mathsf{nad}.\ct)\la\mathsf{NAD}.\Enc(\mathsf{nad}.\MPK,m_b)$, sends
    $\mathsf{nad}.\ct$ to the challenger, receives $\nce.\ct^*$ from $\cA_1$, and sends $\nce.\ct^*$ to $\cA_1$.
    \item $\cA_1$ is allowed to send an function query $f$.
    If $\cB$ receives an function $f$, $\cB$ generates $\mathsf{nad}.\sk_f\la\mathsf{NAD}.\keygen(\mathsf{nad}.\MSK,f)$, call a key query to the challenger, receives $\nce.\sk^*$ from the challenger, and sends $(\nce.\sk^*,\mathsf{nad}.\sk_f)$ to $\cA_1$.
    Let $j$ be the number of times $\cA_1$ has made key queries.
    \item $\cA_1$ does the following.
    \begin{itemize}
        \item If $j=0$, $\cA_1$ sends $\nce.\cert_0$ to $\cB$ and its internal state to $\cA_2$.
        \item If $j=1$, $\cA_1$ sends $(\nce.\cert_1,\mathsf{nad}.\cert)$ to $\cB$ and its internal state to $\cA_2$.
    \end{itemize}
    \item $\cB$ does the following.
    \begin{itemize}
        \item If $j=0$, $\cB$ sends $\nce.\cert_0$ to the challenger, and receives $\nce.\MSK$ or $\bot$ from the challenger.
        If $\cB$ receives $\bot$, it outputs $\bot$, sends $\bot$ to $\cA_2$, and aborts.
        Otherwise, $\cB$ outputs $\top$ and sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
        \item If $j=1$, $\cB$ sends $\nce.\cert_1$ to the challenger, and receives $\nce.\MSK$ or $\bot$ from the challenger.
        $\cB$ computes $\mathsf{NAD}.\Vrfy(\mathsf{nad}.\vk,\mathsf{nad}.\cert)$.
        If $\cB$ receives $\bot$ from the challenger or $\bot\la\mathsf{NAD}.\Vrfy(\mathsf{nad}.\vk,\mathsf{nad}.\cert)$,
        $\cB$ outputs $\bot$, sends $\bot$ to $\cA_2$, and aborts.
        Otherwise, $\cB$ outputs $\top$ and sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
    \end{itemize}
    \item $\cA_2$ outputs $b''$.
    \item The experiment outputs $b''$ if $f(m_0)=f(m_1)$ and the challenger outputs $\top$. Otherwise, the experiment outputs $b''$. 
\end{enumerate}
It is clear that $\Pr[1\la\cB|b'=0]=\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]$ and $\Pr[1\la\cB|b'=1]=\Pr[\sfhyb{1}{}(b)=1]$.
By assumption, $\abs{\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is non-negligible, and therefore $\abs{\Pr[1\la\cB|b'=0]-\Pr[1\la\cB|b'=1]}$ is non-negligible, which contradicts the certified everlasting RNC security of $\Sigma_{\mathsf{cence}}$. 

\begin{proof}[Proof of \cref{prop:hyb_1_hyb_2_cefe_si_ad}]
We assume that $\abs{\Pr[\sfhyb{1}{}(0)=1]-\Pr[\sfhyb{1}{}(1)=1]}$ is non-negligible, and construct an adversary $\cB$ that breaks the certified everlasting RNC security of $\Sigma_{\mathsf{nad}}$.
Let us describe how $\cB$ works below.
\begin{enumerate}
    \item $\cB$ receives $\mathsf{nad}.\MPK$ from the challenger of $\expd{\Sigma_{\mathsf{nad}},\cB}{cert}{ever}{non}{adapt}(\secp,b)$, 
    generates $(\nce.\pk,\nce.\MSK)\la\NCE.\Setup(1^\secp)$, and sends $(\nce.\pk,\mathsf{nad}.\MPK)$ to $\cA_1$.
    \item $\cB$ receives a challenge query $(m_0,m_1)\in\Ms$ from $\cA_1$, computes $(\nce.\vk,\widetilde{\nce.\ct},\nce.\aux)\la\NCE.\Fake(\nce.\pk,\nce.\MSK)$ and sends $\nce.\ct$ to $\cA_1$.
    \item $\cB$ sends a challenge query $(m_0,m_1)\in\Ms$ to the challenger, receives $\mathsf{nad}.\ct$ from the challenger, and computes $\widetilde{\nce.\sk}\la\NCE.\Reveal(\nce.\pk,\nce.\MSK,\nce.\aux,\mathsf{nad}.\ct)$.
    \item
    $\cA_1$ is allowed to make an function query at most one time before it make a challenge query.
    For a key query, $\cB$ receives $f$ from $\cA_1$, sends $f$ to the challenger as an function query, receives $\mathsf{nad}.\sk_f$ from the challenger, and sends $(\widetilde{\nce.\sk},\mathsf{nad}.\sk_f)$ to $\cA_1$. Let $j$ be the number of times that $\cA_1$ has made key queries.
    \item $\cA_1$ does the following.
    \begin{itemize}
        \item If $j=0$, $\cA_1$ sends $\nce.\cert_0$ to $\cB$ and its internal state to $\cA_2$.
        \item If $j=1$, $\cA_1$ sends $(\nce.\cert_1,\mathsf{nad}.\cert)$ to $\cB$ and its internal state to $\cA_2$.
    \end{itemize}
    \item $\cB$ does the following.
    \begin{itemize}
        \item If $j=0$, $\cB$ computes $\NCE.\Vrfy_0(\nce.\vk,\nce.\cert_0)$.
        If the result is $\bot$, $\cB$ outputs $\bot$, sends $\bot$ to $\cA_2$, and aborts.
        Otherwise, $\cB$ outputs $\top$, and sends $(\nce.\MSK,!!!\mathsf{nad}.\MSK!!!)$ to $\cA_2$.
        \item If $j=1$, $\cB$ sends $\mathsf{nad}.\cert$ to the challenger, and receives $\mathsf{nad}.\MSK$ or $\bot$ from the challenger.
        $\cB$ computes $\NCE.\Vrfy_1(\nce.\vk,\widetilde{\nce.\sk},\nce.\aux)$.
        If $\cB$ receives $\bot$ from the challenger or $\bot\la\NCE.\Vrfy_1(\nce.\vk,\widetilde{\nce.\sk},\nce.\aux)$, $\cB$ outputs $\bot$, sends $\bot$ to $\cA_2$, and aborts.
        Otherwise, $\cB$ outputs $\top$, and sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
    \end{itemize}
    \item $\cA_2$ outputs $b'$.
    \item The experiment outputs $b'$ if $f(m_0)=f(m_1)$ and the challenger outputs $\top$. Otherwise, the experiment outputs $b'$. 
\end{enumerate}
\end{proof}
\end{proof}





kokokara ind-base
\section{Certified Everlasting Functional Encryption}\label{sec:function_encryption}

\subsection{Definition}
\taiga{Below, the space is not correctly defined.}
\begin{definition}[$q$-Bounded Certified Everlasting Functional Encryption]\label{def:cert_ever_func}
Let $\secp$ be a security parameter and let $p$, $r$, $s$, $t$ and $u$ be some polynomials. 
A $q$-bounded certified everlasting functional encryption scheme for a class of functions $\mathcal{F}$
is of a tuple of algorithm
$\Sigma=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$
with plaintext space $\Ms\seteq\bit^n$, ciphertext space $\Cs:= \cQ^{\otimes p(\lambda)}$,
public key space $\mathcal{PK}:=\{0,1\}^{r(\lambda)}$,
master secret key space $\mathcal{MSK}\seteq \bit^{s(\lambda)}$,
secret key space $\mathcal{SK}\seteq \bit^{t(\lambda)}$
and deletion certificate space $\mathcal{D}:= \{0,1\}^{u(\lambda)}$.
\begin{description}
    \item[$\Setup(1^\secp)\ra(\MPK,\MSK)$:]
    The setup algorithm takes the security parameter $1^\secp$ as input, and outputs a public key $\MPK\in\mathcal{PK}$
    and a master secret key $\MSK\in\mathcal{MSK}$.
    \item[$\keygen(\MSK,f)\ra\sk_f$:]
    The keygeneration algorithm takes $\MSK$ and $f\in\mathcal{F}$ as input,
    and outputs a secret key $\sk_f\in\mathcal{SK}$.
    \item[$\Enc(\MPK,m)\ra (\vk,\CT)$:]
    The encryption algorithm takes $\MPK$ and $m\in\Ms$ as input,
     and outputs a verification key $\vk\in\mathcal{VK}$ and a ciphertext $\CT\in \Cs$.
    \item[$\Dec(\sk_f,\CT)\ra (y,\widehat{\ct})$ $\mbox{\bf  or }\bot$:]
    The decryption algorithm takes $\sk_f$ and $\CT$ as input, and outputs $y$ and $\widehat{\ct}\in\Cs$ or $\bot$.
    \item[$\Delete(\CT)\ra \cert$:]
    The deletion algorithm takes $\CT$ as input, and outputs a classical certificate $\cert$.
    \item[$\Vrfy(\vk,\cert)\ra \top \mbox{ {\bf or} } \bot$:]
    The verification algorithm $\Vrfy$ takes $\vk$ and $\cert$ as input,
    and outputs $\top$ or $\bot$.
\end{description}
\end{definition}

\begin{definition}[Correctness for Certified Everlasting Functional Encryption]\label{def:correctness_cert_ever_func}
There are three types of correctness.
The first is evaluation correctness,
the second is verification correctness,
and the third is rewind correctness.

\paragraph{Evaluation Correctness:}
There exists a negligible function $\negl$ such that for any $\secp\in \N$, $m\in\Ms$ and $f\in\mathcal{F}$,
\begin{align}
\Pr\left[
y\ne f(m)
\ \middle |
\begin{array}{ll}
(\MPK,\MSK)\la\Setup(1^\secp)\\
\sk_f\la\keygen(\MSK,f)\\
(\vk,\CT)\lrun \Enc(\MPK,m)\\
(y,\widehat{\ct})\la\Dec(\sk_f,\ct)
\end{array}
\right] 
\le\negl(\secp).
\end{align}





\paragraph{Verification Correctness:}
There exists a negligible function $\negl$ such that $\secp\in\N$, $m\in \Ms$,
\begin{align}
\Pr\left[
\Vrfy(\vk,\cert)\neq\bot
\ \middle |
\begin{array}{ll}
(\MPK,\MSK)\la\Setup(1^\secp)\\
(\vk,\CT)\lrun \Enc(\MPK,m)\\
\cert\la\Delete(\CT)
\end{array}
\right] 
\leq
\negl(\secp).
\end{align}

\paragraph{Rewind Correctness:}
There exists a negligible function $\negl$ such that for any $\secp\in \N$, $m\in\Ms$ and $f\in\mathcal{F}$,
\begin{align}
\Pr\left[
\frac{1}{2}\norm{\ct-\widehat{\ct}}_{\tr}\leq \negl(\lambda)
\ \middle |
\begin{array}{ll}
(\MPK,\MSK)\la\Setup(1^\secp)\\
\sk_f\la\keygen(\MSK,f)\\
(\vk,\CT)\lrun \Enc(\MPK,m)\\
(y,\widehat{\ct})\la\Dec(\sk_f,\ct)
\end{array}
\right] 
\leq1-\negl(\lambda).
\end{align}

{\color{red}
\paragraph{Modification Correctness:} There exists a negligible function $\negl$ and a modification algorithm $\Modify$ such that for any $\secp\in \N$ and $m\in\Ms$, 
\begin{align}
\Pr\left[
\Vrfy(\vk,\cert')\neq\top
\ \middle |
\begin{array}{ll}
(\MPK,\MSK)\la\Setup(1^\secp)\\
\sk_f\lrun \keygen(\MSK,f)\\
(\vk,\ct) \lrun \Enc(\MPK,m)\\
a,b\la\bit^*\\
\cert^* \lrun \Delete(Z^bX^a\ct X^aZ^b)\\
\cert'\lrun \Modify(a,b,\cert^*)  
\end{array}
\right] 
\leq
\negl(\secp).
\end{align}
}
\end{definition}
\begin{remark}
We note that modification correctness is not necessary for certified everlasting FE in itself.
But, we need modification correctness to prove that our construction of functional encryption with adaptive security in \cref{sec:const_fe_adapt} satisfies verification correctness.
We also note that rewind correctness is necessary for FE.
This is because, in a FE scheme, a receiver with $(\ct,\{\sk_{f_i}\}_{i\in[j]})$ should be able to obtain $\{f_i(x)\}_{i\in[j]}$.
However, a decryption algorithm might break a quantum ciphertext $\ct$, and thus the receiver may not obtain $\{f_i(x)\}_{i\in[j]}$.
Rewind correctness guarantees that a decryption algorithm does not break a quantum ciphertext $\ct$ and thus that the receiver obtains $\{f_i(x)\}_{i\in[j]}$ correctly.
\end{remark}


\begin{definition}[$q$-Bounded Non-Adaptive Security for Certified Everlasting Functional Encryption]\label{def:non_ada_security_cert_ever_func}
Let $q$ be a polynomial of $\lambda$.
Let $\Sigma=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$ be a $q$-bounded certified everlasting functional encryption scheme.
We consider the following security experiment $\expa{\Sigma,\cA}{non}{\mathsf{adapt}}(\secp,b)$.
\begin{enumerate}
    \item The challenger runs $(\MPK,\MSK)\la \Setup(1^\secp)$ and sends $\MPK$ to $\cA$.
    \item $\cA$ can make at most $q$ key queries at first and one challenge query after that.
    \begin{itemize}
    \item[{\bf Key Query.}] $\cA$ is allowed to make arbitrary function queries at most $q$ times.
    For the $\ell$-th key query, the challenger receives $f_\ell\in\mathcal{F}$, 
    computes $\sk_{f_\ell}\la\keygen(\MSK,f_\ell)$
    and sends $\sk_{f_\ell}$ to $\cA$.
    \item[{\bf Challenge Query.}] $\cA$ submits a message pair $(m_0,m_1)\in\Ms$ to the challenger.
    The challenger computes 
    $(\vk,\CT)\la \Enc(\MPK,m_b)$ and 
    sends $\CT$ to $\cA$.
    \end{itemize}
    \item $\cA$ outputs $b'$.
    \item The experiment outputs $b'$ if $f_i(m_0)=f_i(m_1)$ for all $i\in[q]$.
    Otherwise the experiment outputs $\bot$.
\end{enumerate}
We say that the $\Sigma$ is $q$-bounded non-adaptive secure if for any $QPT$ adversary $\cA$ it holds that
\begin{align}
\advb{\Sigma,\cA}{non}{adapt}(\secp) \seteq \abs{\Pr[\expa{\Sigma,\cA}{non}{\mathsf{adapt}}(\secp,0)=1]  - \Pr[\expa{\Sigma,\cA}{non}{\mathsf{adapt}}(\secp,1)=1]} \leq \negl(\secp).
\end{align}
We further say that the $\Sigma$ is single-key non-adaptive secure if $q=1$.
\end{definition}

\begin{definition}[$q$-Bounded Adaptive Security for Certified Everlasting Functional Encryption]\label{def:ada_security_cert_ever_func}
Let $\Sigma=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$ be a $q$-bounded certified everlasting functional encryption scheme.
And let $q$ be a polynomial of $\lambda$.
We consider the following security experiment $\Expt{\Sigma,\cA}{\mathsf{adapt}}(\secp,b)$.
\begin{enumerate}
    \item The challenger runs $(\MPK,\MSK)\la \Setup(1^\secp)$ and sends $\MPK$ to $\cA$.
    \item $\cA$ can make at most $q$ key queries and one challenge query in any order.
    \begin{itemize}
    \item[{\bf Key Query.}] $\cA$ is allowed to make arbitrary function queries at most $q$ times.
    For the $\ell$-th key query, the challenger receives $f_\ell\in\mathcal{F}$,   
    computes $\sk_{f_\ell}\la\keygen(\MSK,f_\ell)$
    and sends $\sk_{f_\ell}$ to $\cA$.
    \item[{\bf Challenge Query.}] $\cA$ submits a message pair $(m_0,m_1)\in\Ms$ to the challenger.
    The challenger computes 
    $(\vk,\CT)\la \Enc(\MPK,m_b)$ and 
    sends $\CT$ to $\cA$.
    \end{itemize}
    \item $\cA$ outputs $b'$.
    \item The experiment outputs $b'$ if $f_i(m_0)=f_i(m_1)$ for all $i\in[q]$.
    Otherwise the experiment outputs $\bot$.
\end{enumerate}
We say that the $\Sigma$ is $q$-bounded adaptive secure if for any $QPT$ adversary $\cA$ it holds that
\begin{align}
\adva{\Sigma,\cA}{adapt}(\secp) \seteq \abs{\Pr[\Expt{\Sigma,\cA}{\mathsf{adapt}}(\secp,0)=1]  - \Pr[\Expt{\Sigma,\cA}{\mathsf{adapt}}(\secp,1)=1]} \leq \negl(\secp).
\end{align}
We further say that the $\Sigma$ is single-key adaptive secure if $q=1$.
\end{definition}




\begin{definition}[$q$-Bounded Certified Everlasting Non-Adaptive Security for Certified Everlasting Functional Encryption]\label{def:cert_ever_non_adapt_security_cert_ever_func}
Let $\Sigma=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$ be a $q$-bounded certified everlasting functional encryption scheme.
And let $q$ be a polynomial of $\lambda$.
We consider the following security experiment $\expd{\Sigma,\cA}{cert}{ever}{non}{adapt}(\secp,b)$.
\begin{enumerate}
    \item The challenger runs $(\MPK,\MSK)\la \Setup(1^\secp)$ and sends $\MPK$ to $\cA_1$.
    \item $\cA_1$ can make at most $q$ key queries at first and one challenge query after that.
    \begin{itemize}
    \item[{\bf Key Query.}] $\cA_1$ is allowed to make arbitrary function queries at most $q$ times.
    For the $\ell$-th key query, the challenger receives $f_\ell\in\mathcal{F}$,  
    computes $\sk_{f_\ell}\la\keygen(\MSK,f_\ell)$
    and sends $\sk_{f_\ell}$ to $\cA_1$.
    \item[{\bf Challenge Query.}] $\cA_1$ submits a message pair $(m_0,m_1)\in\Ms$ to the challenger.
    The challenger computes 
    $(\vk,\CT)\la \Enc(\MPK,m_b)$ and 
    sends $\CT$ to $\cA_1$.
    \end{itemize}
    \item At some point, $\cA_1$ sends $\cert$ to the challenger and the internal state to $\cA_2$.
    \item The challenger computes $\Vrfy(\vk,\cert)$.
    If the output is $\bot$, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$. Else the challenger outputs $\top$ and sends $\MSK$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item The experiment outputs $b'$ if $f_\ell(m_0)=f_\ell(m_1)$ for all $\ell\in[q]$ and the challenger outputs $\top$.
    Otherwise the experiment outputs $\bot$.
\end{enumerate}
We say that the $\Sigma$ is $q$-bounded certified everlasting non-adaptive secure if for any QPT $\cA_1$ and any unbounded $\cA_2$, it holds that
\begin{align}
\advd{\Sigma,\cA}{cert}{ever}{non}{adapt}(\secp) \seteq \abs{\Pr[\expd{\Sigma,\cA}{cert}{ever}{non}{adapt}(\secp,0)=1]  - \Pr[\expd{\Sigma,\cA}{cert}{ever}{non}{adapt}(\secp,1)=1]} \leq \negl(\secp).
\end{align}
We further say that the $\Sigma$ is single-key certified everlasting non-adaptive secure if $q=1$.
\end{definition}

\begin{definition}[$q$-Bounded Certified Everlasting Adaptive Security for Certified Everlasting Functional Encryption]\label{def:cert_ever_adapt_security_cert_ever_func}
Let $\Sigma=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$ be a $q$-bounded certified everlasting functional encryption scheme.
And let $q$ be a polynomial of $\lambda$.
We consider the following security experiment $\expc{\Sigma,\cA}{cert}{ever}{adapt}(\secp,b)$.
\begin{enumerate}
    \item The challenger runs $(\MPK,\MSK)\la \Setup(1^\secp)$ and sends $\MPK$ to $\cA_1$.
    \item $\cA_1$ can make at most $q$ key queries and one challenge query in any order.
    \begin{itemize}
    \item[{\bf Key Query.}] $\cA_1$ is allowed to make arbitrary function queries at most $q$ times.
    For the $\ell$-th key query, the challenger receives $f_\ell\in\mathcal{F}$,  
    computes $\sk_{f_\ell}\la\keygen(\MSK,f_\ell)$
    and sends $\sk_{f_\ell}$ to $\cA_1$.
    \item[{\bf Challenge Query.}] $\cA_1$ submits a message pair $(m_0,m_1)\in\Ms$ to the challenger.
    The challenger computes 
    $(\vk,\CT)\la \Enc(\MPK,m_b)$ and 
    sends $\CT$ to $\cA_1$.
    \end{itemize}
    \item At some point, $\cA_1$ sends $\cert$ to the challenger and the internal state to $\cA_2$.
    \item The challenger computes $\Vrfy(\vk,\cert)$.
    If the output is $\bot$, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$. Else the challenger outputs $\top$ and sends $\MSK$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item The experiment outputs $b'$ if $f_\ell(m_0)=f_\ell(m_1)$ for all $\ell\in[q]$ and the challenger outputs $\top$.
    Otherwise the experiment outputs $\bot$.
\end{enumerate}
We say that the $\Sigma$ is $q$-bounded certified everlasting adaptive secure if for any QPT $\cA_1$ and any unbounded $\cA_2$, it holds that
\begin{align}
\advc{\Sigma,\cA}{cert}{ever}{adapt}(\secp) \seteq \abs{\Pr[\expc{\Sigma,\cA}{cert}{ever}{adapt}(\secp,0)=1]  - \Pr[\expc{\Sigma,\cA}{cert}{ever}{adapt}(\secp,1)=1]} \leq \negl(\secp).
\end{align}
We further say that the $\Sigma$ is single-key certified everlasting adaptive secure if $q=1$.
\end{definition}


\subsection{Construction of Single-Key Certified Everlasting Functional Encryption with Non-Adaptive Security}\label{sec:const_func_non_adapt}
In this section, we present how to construct a single-key certified everlasting functional encryption scheme with non-adaptive security from 
a certified everlasting garbling scheme and a certified everlasting PKE scheme.

\paragraph{Our single-key certified everlasting FE scheme with non-adaptive security.}
We use a universal circuit $U(\cdot,x)$ in which a plaintext $x$ is hard-wired, takes as an input a function $f$ and outputs $f(x)$.
Let $s\seteq |f|$.
We construct a single-key certified everlasting functional encryption scheme with non-adaptive security $\Sigma_{\mathsf{cefe}}=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$
from a certified everlasting garbling scheme $\Sigma_{\mathsf{cegc}}=\mathsf{GC}.(\Samp,\Garble,\Eval,\Delete,\Vrfy)$
and a certified everlasting PKE scheme $\Sigma_{\mathsf{cepk}}=\PKE.(\keygen,\Enc,\Dec,\Delete,\Vrfy)$.

\begin{description}
\item[$\Setup(1^\secp)$:] $ $
\begin{itemize}
    \item Generate $(\pke.\pk_{i,\alpha},\pke.\sk_{i,\alpha})\la\PKE.\keygen(1^\secp)$ for every $i\in [s]$ and $\alpha\in\bit$.
    \item Output $\MPK\seteq \{\pke.\pk_{i,\alpha}\}_{i\in[s],\alpha\in\{0,1\}}$ and $\MSK\seteq \{\pke.\sk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$.
\end{itemize}
\item[$\keygen(\MSK,f)$:] $ $
\begin{itemize}
    \item Parse $\MSK=\{\pke.\sk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ and $f=(f_1,\cdots,f_s)$.
    \item Output $\sk_f\seteq (f,\{\pke.\sk_{i,f[i]}\}_{i\in[s]})$.
\end{itemize}
\item[$\Enc(\MPK,m)$:]$ $
\begin{itemize}
    \item Parse $\MPK=\{\pke.\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$.
    \item Compute $\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit}\la\mathsf{GC}.\Samp(1^\secp)$
    \item Compute $(\widetilde{U},\mathsf{gc}.\vk)\la\mathsf{GC}.\Garble(1^\secp,U(\cdot,m),\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$.
    \item For every $i\in[s]$ and $\alpha\in\bit$, compute $(\pke.\ct_{i,\alpha},\pke.\vk_{i,\alpha})\la\PKE.\Enc(\pke.\pk_{i,\alpha},L_{i,\alpha})$.
    \item Output $\vk\seteq (\mathsf{gc}.\vk,\{\pke.\vk_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$
    and $\CT\seteq (\widetilde{U},\{\pke.\ct_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$.
\end{itemize}
\item[$\Dec(\sk_f,\ct)$:] $ $
\begin{itemize}
    \item Parse $\sk_f=(f,\{\pke.\sk_i\}_{i\in[s]})$ and $\ct=(\widetilde{U},\{\pke.\ct_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$.
    \item For every $i\in [s]$, compute $(L_i,\widehat{\pke.\ct}_{i,f[i]})\la\PKE.\Dec(\pke.\sk_{i},\pke.\ct_{i,f[i]})$.
    Let us denote $\widehat{\pke.\ct}_{i,f[i]\oplus 1}\seteq \pke.\ct_{i,f[i]\oplus 1}$.
    %\footnote{From the correctness and the gentle measurement lemma, there exists the decryption algorithm that does not break the quantum ciphertext $\pke.\ct_{i,f[i]}$ for each $i\in[s]$.}.
    \item Compute $(y,\widehat{U})\la \mathsf{GC}.\Eval(\widetilde{U},\{L_i\}_{i\in[s]})$
    %\footnote{From the correctness and the gentle measurement lemma, there exists the evaluation algorithm that does not break the quantum garbled circuit $\widetilde{U}$.}.
    \item Output $y$ and $\ct=(\widehat{U},\{\widehat{\pke.\ct}_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$.
\end{itemize}
\item[$\Delete(\CT)$:] $ $
\begin{itemize}
    \item Parse $\ct=(\widetilde{U},\{\pke.\ct_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$.
    \item Compute $\mathsf{gc}.\cert\la\mathsf{GC}.\Delete(\widetilde{U})$.
    \item For every $i\in[s]$ and $\alpha\in\bit$, compute $\pke.\cert_{i,\alpha}\la\PKE.\Delete(\pke.\ct_{i,\alpha})$.
    \item Output $\cert\seteq (\mathsf{gc}.\cert,\{\pke.\cert_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$.
\end{itemize}
\item[$\Vrfy(\vk,\cert)$:] $ $
\begin{itemize}
    \item Parse $\vk=(\mathsf{gc}.\vk,\{\pke.\vk_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ and $\cert=(\mathsf{gc}.\cert,\{\pke.\cert_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$.
    \item Output $\top$ if $\top\la\mathsf{GC}.\Vrfy(\mathsf{gc}.\vk,\mathsf{gc}.\cert)$ and $\top\la\PKE.\Vrfy(\pke.\vk_{i,\alpha},\pke.\cert_{i,\alpha})$ for every $i\in[s]$ and $\alpha\in\bit$.
    Otherwise output $\bot$.
\end{itemize}
\end{description}

\paragraph{Correctness:}
Decryption correctness easily follows from the decryption correctness of $\Sigma_{\mathsf{cegc}}$ and $\Sigma_{\mathsf{cepk}}$.
Verification correctness easily follow from the verification correctness of $\Sigma_{\mathsf{cegc}}$ and $\Sigma_{\mathsf{cepk}}$.
Rewind correctness easily follows from the rewind correctness of $\Sigma_{\mathsf{cegc}}$ and $\Sigma_{\mathsf{cepk}}$.
Modification correctness easily follows from the modification correctness of $\Sigma_{\mathsf{cegc}}$ and $\Sigma_{\mathsf{cepk}}$.

\paragraph{Security:}
We prove the following two theorems.
\begin{theorem}\label{thm:func_non_ad_seucirty}
If $\Sigma_{\mathsf{cegc}}$ satisfies the selective security and $\Sigma_{\mathsf{cepk}}$ satisfies  the IND-CPA security,
$\Sigma_{\mathsf{cefe}}$ satisfies single-key non-adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:func_non_ad_seucirty}]
The proof is similar to that of \cref{thm:func_ever_non_ad_security}.
\end{proof}

\begin{theorem}\label{thm:func_ever_non_ad_security}
If $\Sigma_{\mathsf{cegc}}$ satisfies the certified everlasting selective security and $\Sigma_{\mathsf{cepk}}$ satisfies the certified everlasting IND-CPA security,
$\Sigma_{\mathsf{cefe}}$ satisfies the single-key certified everlasting non-adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:func_ever_non_ad_security}]
For clarity, we describe how the experiment works against an adversary $\cA\coloneqq (\cA_1,\cA_2)$ consisting of any QPT adversary $\cA_1$ and any unbounded time adversary $\cA_2$.
\begin{description}
\item [$\expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp,b)$:] This is the original experiment.
\begin{enumerate}
    \item The challenger generates $(\pke.\pk_{i,\alpha},\pke.\sk_{i,\alpha})\la\PKE.\keygen(1^\secp)$ for every $i\in [s]$ and $\alpha\in\bit$, and sends
    $\{\pke.\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_1$.
    \item\label{step:function_query_single_fe}
    $\cA_1$ is allowed to call a key query at most one time.
    If a key query is called,
    the challenger receives an function query $f$ from $\cA_1$ and sends $(f,\{\pke.\sk_{i,f[i]}\}_{i\in[s]})$ to $\cA_1$.
    \item $\cA_1$ chooses $(m_0,m_1)\in\Ms^2$ and sends $(m_0,m_1)$ to the challenger.
    \item \label{step:encryption_single_fe}
    The challenger computes $\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit}\la\mathsf{GC}.\Samp(1^\secp)$, $(\widetilde{U},\mathsf{gc}.\vk)\la\mathsf{GC}.\Garble(1^\secp,U(\cdot,m_b),\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$, and
    $(\pke.\vk_{i,\alpha},\pke.\ct_{i,\alpha})\la\PKE.\Enc(\pke.\pk_{i,\alpha},L_{i,\alpha})$ for every $i\in[s]$ and $\alpha\in\bit$,
    and sends $(\widetilde{U},\{\pke.\ct_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ to $\cA_1$.
    \item $\cA_1$ sends $(\mathsf{gc}.\cert,\{\pke.\cert_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ to the challenger and sends its internal state to $\cA_2$.
    \item If $\top\la \mathsf{GC}.\Vrfy(\mathsf{gc}.\vk,\mathsf{gc}.\cert)$, and $\top\la\PKE.\Vrfy(\pke.\vk_{i,\alpha},\pke.\cert_{i,\alpha})$ for every $i\in[s]$ and $\alpha\in\bit$, the challenger outputs $\top$ and  sends $\{\pke.\sk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item The experiment outputs $b'$ if $f(m_0)=f(m_1)$ and the challenger outputs $\top$.
    Otherwise, the experiment outputs $\bot$.
\end{enumerate}
What we have to prove is that 
\begin{align}
    \advd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp)
\seteq \abs{\Pr[ \expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, 0)=1] - \Pr[ \expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, 1)=1] }\leq \negl(\secp).
\end{align}
\end{description}
We define the following sequence of hybrids.
\item[$\sfhyb{1}{}(b)$:]This is identical to $\expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, b)$ except for the following three points.
First, the challenger generates $f\in\bit^s$ on the condition $f(m_0)=f(m_1)$ if a key query is not called.
Second, the challenger randomly generates $L^*_{i,f[i]\oplus 1}\la \mathcal{L}$ for every $i\in[s]$ in step~\ref{step:function_query_single_fe}.
Third, 
the challenger computes 
$(\pke.\vk_{i,f[i]\oplus 1},\pke.\ct_{i,f[i]\oplus 1})\la\PKE.\Enc(\pke.\pk_{i,f[i]\oplus 1},L^*_{i,f[i]\oplus 1})$ for every $i\in[s]$ instead of computing 
$(\pke.\vk_{i,f[i]\oplus 1},\pke.\ct_{i,f[i]\oplus 1})\la\PKE.\Enc(\pke.\pk_{i,f[i]\oplus 1},L_{i,f[i]\oplus 1})$ for every $i\in[s]$.

\item[$\sfhyb{2}{}(b)$:]This is identical to $\sfhyb{1}{}(b)$ except for the following point.
The challenger computes $(\widetilde{C},\mathsf{gc}.\vk)\la\GC.\Sim(1^\secp,1^{|C|},U(f,m_b),\{L_{i,f[i]}\}_{i\in[s]})$
in step~\ref{step:encryption_single_fe} instead of computing $(\widetilde{U},\mathsf{gc}.\vk)\la\mathsf{GC}.\Garble(1^\secp,U(\cdot,m_b),\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ in  step~\ref{step:encryption_single_fe}.

\begin{proposition}\label{prop:Exp_Hyb_1_non_ad_fe}
If $\Sigma_{\mathsf{cepk}}$ satisfies the certified everlasting IND-CPA security,
\begin{align}
    \abs{\Pr[\expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, b)=1]-\Pr[\sfhyb{1}{}(b)=1]}\leq\negl(\lambda).
\end{align}
for $b\in\bit$.
\end{proposition}
\begin{proof}[Proof of \cref{prop:Exp_Hyb_1_non_ad_fe}]
We assume that $\abs{\Pr[\expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is non-negligible, and construct an adversary $\cB$ that breaks the security experiment of  $\expd{\Sigma_{\mathsf{cepk}},\cB}{cut}{choose}{cert}{ever}(\secp,b')$ defined in \cref{lem:cut_and_choose_pke}.
This contradicts the certified everlasting IND-CPA of $\Sigma_{\mathsf{cepk}}$ from \cref{lem:cut_and_choose_pke}.
Let us describe how $\cB$ works below.
\begin{enumerate}
    \item $\cB$ receives $\{\pke.\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ from the challenger of $\expd{\Sigma_{\mathsf{cepk}},\cB}{cut}{choose}{cert}{ever}(\secp,b')$ and sends $\{\pke.\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_1$.
    \item $\cA_1$ is allowed to call a key query at most one time.
    If a key query is called,
    $\cB$ receives an function $f$ from $\cA_1$, generates $L^*_{i,f[i]\oplus 1}\la \mathcal{L}$ for every $i\in[s]$, and computes $\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit}\la\mathsf{GC}.\Samp(1^\secp)$.
    If a key query is not called, $\cB$ generates $f\in\bit^s$ on the condition $f(m_0)=f(m_1)$. 
    \item $\cB$ sends $(f,L^*_{1,f[1]\oplus 1},L^*_{2,f[2]\oplus 1},\cdots, L^{*}_{s,f[s]\oplus 1},L_{1,f[1]\oplus 1},L_{2,f[2]\oplus 1},\cdots ,L_{s,f[s]\oplus 1})$ to the challenger of $\expd{\Sigma_{\mathsf{cepk}},\cB}{cut}{choose}{cert}{ever}(\secp,b')$.
    \item $\cB$ receives $(\{\pke.\sk_{i,f[i]}\}_{i\in[s]},\{\pke.\ct_{i,f[i]\oplus 1}\}_{i\in[s]})$ from the challenger.
    If a key query is called, $\cB$ sends $(f,\{\pke.\sk_{i,f[i]}\}_{i\in[s]})$ to $\cA_1$.
    \item $\cA_1$ chooses $(m_0,m_1)\in\Ms^2$ and sends $(m_0,m_1)$ to $\cB$.
    \item $\cB$ computes
    $(\widetilde{U},\mathsf{gc}.\vk)\la\mathsf{GC}.\Garble(1^\secp,U(\cdot,m_b),\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ and
    $(\pke.\vk_{i,f[i]},\pke.\ct_{i,f[i]})\la\PKE.\Enc(\pke.\pk_{i,f[i]},L_{i,f[i]})$ for every $i\in[s]$ and sends $(\widetilde{U},\{\pke.\ct_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ to $\cA_1$.
    \item $\cA_1$ sends $(\mathsf{gc}.\cert,\{\pke.\cert_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ to $\cB$ and sends its internal state to $\cA_2$.
    \item $\cB$ sends $\{\pke.\cert_{i,f[i]\oplus1}\}_{i\in[s]}$ to the challenger, and receives $\{\pke.\sk_{i,f[i]\oplus 1}\}_{i\in[s]}$ or $\bot$ from the challenger. If $\cB$ receives $\bot$ from the challenger, it outputs $\bot$ and aborts. 
    \item $\cB$ sends $\{\pke.\sk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_2$.
    \item $\cA_2$ outputs $b''$.
    \item $\cB$ computes $\mathsf{GC}.\Vrfy$ for $\gc.\cert$ and $\PKE.\Vrfy$ for all $\pke.\cert_{i,\alpha}$, and outputs $b''$ if all results are $\top$ and $f(m_0)=f(m_1)$. Otherwise, $\cB$ outputs $\bot$. 
\end{enumerate}
If $b'=1$, $\cB$ simulates $\expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, b)$.
If $b'=0$, $\cB$ simulates $\sfhyb{1}{}(b)$.
Therefore, it holds that $\Pr[1\la\cB|b'=1]=\Pr[\expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, b)=1]$ and 
$\Pr[1\la\cB|b'=0]=\Pr[\sfhyb{1}{}(b)=1]$.
By assumption, $\abs{\Pr[\expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is non-negligible, and therefore $\abs{\Pr[1\la\cB|b'=0]-\Pr[1\la\cB|b'=1]}$ is non-negligible, which contradicts the certified everlasting IND-CPA security of $\Sigma_{\mathsf{cepk}}$ from \cref{lem:cut_and_choose_pke}.
\end{proof}

\begin{proposition}\label{prop:Hyb_1_Hyb_2_non_ad_fe}
If $\Sigma_{\mathsf{cegc}}$ satisfies the certified everlasting selective security,
\begin{align}
    \abs{\Pr[\sfhyb{1}{}(b)=1]-\Pr[\sfhyb{2}{}(b)=1]}\leq\negl(\lambda)
\end{align}
for $b\in\bit$.
\end{proposition}
\begin{proof}
We assume that $\abs{\Pr[\sfhyb{1}{}(b)=1]-\Pr[\sfhyb{2}{}(b)=1]}$ is non-negligible, and construct an adversary $\cB$ that breaks the certified everlasting selective security of $\Sigma_{\mathsf{cegc}}$.
Let us describe how $\cB$ works below.
\begin{enumerate}
    \item $\cB$ generates $(\pke.\pk_{i,\alpha},\pke.\sk_{i,\alpha})\la\PKE.\keygen(1^\secp)$ for every $i\in [s]$ and $\alpha\in\bit$, and sends
    $\{\pke.\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_1$.
    \item $\cA_1$ is allowed to call a key query at most one time.
    If a key query is called, $\cB$ receives an function query $f$ from $\cA_1$, generates $L^*_{i,f[i]\oplus 1}\la \mathcal{L}$ for every $i\in[s]$, and sends $(f,\{\pke.\sk_{i,f[i]}\}_{i\in[s]})$ to $\cA_1$.
    If a key query is not called, $\cB$ generates $f\in\bit^s$ on the condition $f(m_0)=f(m_1)$.
    \item $\cA_1$ chooses $(m_0,m_1)\in\Ms^2$ and sends $(m_0,m_1)$ to $\cB$.
    \item $\cB$ sends a circuit $U(\cdot,m_b)$ and an input $f\in\bit^s$ to the challenger of $\expb{\cB,\Sigma_{\mathsf{cegc}}}{cert}{ever}{selct}(1^\secp,b')$.
    \item The challenger computes $\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit}\la\mathsf{GC}.\Samp(1^\secp)$ and does the following:
    \begin{itemize}
        \item If $b'=0$, the challenger computes $(\widetilde{U},\mathsf{gc}.\vk)\la\mathsf{GC}.\Garble(1^\secp,U(\cdot,m_b),\{L_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$, and sends $(\widetilde{U},\{L_{i,f[i]}\}_{i\in[s]})$ to $\cB$.
        \item If $b'=1$, the challenger computes $(\widetilde{U},\mathsf{gc}.\vk)\la\GC.\Sim(1^\secp,1^{|C|},U(f,m_b),\{L_{i,f[i]}\}_{i\in[s]})$, and sends $(\widetilde{U},\{L_{i,f[i]}\}_{i\in[s]})$ to $\cB$.
    \end{itemize}
    \item $\cB$ computes $(\pke.\vk_{i,f[i]},\pke.\ct_{i,f[i]})\la\PKE.\Enc(\pke.\pk_{i,f[i]},L_{i,f[i]})$ for every $i\in[s]$ 
    and $(\pke.\ct_{i,f[i]\oplus 1},\pke.\vk_{i,f[i]\oplus 1})\la\PKE.\Enc(\pke.\pk_{i,f[i]\oplus 1},L^*_{i,f[i]\oplus 1}) $ for every $i\in[s]$.
    \item $\cB$ sends $(\widetilde{U},\{\pke.\ct_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ to $\cA_1$.
    \item $\cA_1$ sends $(\mathsf{gc}.\cert,\{\pke.\cert_{i,\alpha}\}_{i\in[s],\alpha\in\bit})$ to the challenger and sends its internal state to $\cA_2$.
    \item $\cB$ sends $\mathsf{gc}.\cert$ to the challenger, and receives $\top$ or $\bot$ from the challenger.
    If $\cB$ receives $\bot$ from the challenger, it outputs $\bot$ and abort.
    \item $\cB$ sends $\top$ to $\cA_2$.
    \item $\cA_2$ outputs $b''$.
    \item $\cB$ computes $\PKE.\Vrfy$ for all $\pke.\cert_{i,\alpha}$, and outputs $b''$ if all results are $\top$ and $f(m_0)=f(m_1)$.
    Otherwise, $\cB$ outputs $\bot$.
\end{enumerate}
It is clear that $\Pr[1\la\cB|b'=0]=\Pr[\sfhyb{1}{}(b)=1]$ and $\Pr[1\la\cB|b'=1]=\Pr[\sfhyb{2}{}(b)=1]$.
By assumption, $\abs{\Pr[\sfhyb{1}{}(b)=1]-\Pr[\sfhyb{2}{}(b)=1]}$ is non-negligible, and therefore $\abs{\Pr[1\la\cB|b'=0]-\Pr[1\la\cB|b'=1]}$ is non-negligible, which contradicts the certified everlasting selective security of $\Sigma_{\mathsf{cegc}}$. 
\end{proof}
\begin{proposition}\label{prop:Hyb_2_non_ad_fe}
$
\Pr[\sfhyb{2}{}(0)=1]=\Pr[\sfhyb{2}{}(1)=1].
$
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_2_non_ad_fe}]
The experiment outputs $1$ only when $f(m_0)=f(m_1)$.
Thus, it is sufficient to consider the case with $f(m_0)=f(m_1)$.
Then, the experiment $\sfhyb{2}{}(b)$ does not depend on $b$.
This is because the experiment depends on $b$ only where $(\widetilde{U},\mathsf{gc}.\vk)\la\GC.\Sim(1^\secp,1^{|C|},U(f,m_b),\{L_{i,f[i]}\}_{i\in[s]})$ but it holds that $U(f,m_0)=U(f,m_1)$. 
Therefore, it holds that
$
\Pr[\sfhyb{2}{}(0)=1]=\Pr[\sfhyb{2}{}(1)=1].
$
\end{proof}
By \cref{prop:Exp_Hyb_1_non_ad_fe,prop:Hyb_1_Hyb_2_non_ad_fe,prop:Hyb_2_non_ad_fe}, we immediately obtain \cref{thm:func_ever_non_ad_security}.
\end{proof}



\subsection{Construction of Single-Key Certified Everlasting Functional Encryption with Adaptive Security}\label{sec:const_fe_adapt}
In this section, we present how to construct a single-key certified everlasting functional encryption scheme with adaptive security from a certified everlasting functional encryption scheme with non-adaptive security and a certified everlasting RNC scheme.

\paragraph{Our single-key certified everlasting FE scheme with adaptive security.}
In this section, we present how to construct a single-key certified everlasting functional encryption scheme with adaptive security $\Sigma_{\mathsf{cefe}}=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$ from a single-key certified everlasting functional encryption scheme with non-adaptive security
$\Sigma_{\mathsf{nad}}=\mathsf{NAD}.(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$
and a certified everlasting RNCE scheme for classical message $\Sigma_{\mathsf{cence}}=\NCE.(\Setup,\keygen,\Enc,\Dec,\Fake,\Reveal,\Delete,\Vrfy)$.
Let $\nad.\Modify$ be the algorithm such that
\begin{align}
\Pr\left[
\NAD.\Vrfy(\nad.\vk,\nad.\cert')\neq\top
\ \middle |
\begin{array}{ll}
(\nad.\MPK,\nad.\MSK)\lrun \NAD.\Setup(1^\secp)\\
(\nad.\vk,\nad.\ct) \lrun \NAD.\Enc(\nad.\MPK,m)\\
a,b\la\bit^*\\
\nad.\cert^* \lrun \NAD.\Delete(Z^bX^a\nad.\ct X^aZ^b)\\
\nad.\cert'\lrun \NAD.\Modify(a,b,\cert^*) 
\end{array}
\right] 
\leq
\negl(\secp).
\end{align}


\begin{description}
\item[$\Setup(1^\secp)$:]$ $
\begin{itemize}
    \item Generate $(\mathsf{nad}.\MPK,\mathsf{nad}.\MSK)\la\mathsf{NAD}.\Setup(1^\secp)$.
    \item Generate $(\nce.\pk,\nce.\MSK)\la\NCE.\Setup(1^{\secp})$.
    \item Output $\MPK\seteq(\nce.\pk,\mathsf{nad}.\MPK)$ and $\MSK\seteq (\nce.\MSK,\mathsf{nad}.\MSK)$.
\end{itemize}
\item[$\keygen(\MSK,f)$:]$ $
\begin{itemize}
    \item Parse $\MSK=(\nce.\MSK,\mathsf{nad}.\MSK)$.
    \item Compute $\mathsf{nad}.\sk_f\la\mathsf{NAD}.\keygen(\mathsf{nad}.\MSK,f)$.
    \item Compute $\nce.\sk\la\NCE.\keygen(\nce.\MSK)$.
    \item Output $\sk_f\seteq (\nce.\sk,\mathsf{nad}.\sk_f)$.
\end{itemize}
\item[$\Enc(\MPK,m)$:]$ $
\begin{itemize}
    \item Parse $\MPK=(\nce.\pk,\mathsf{nad}.\MPK)$.
    \item Compute $(\mathsf{nad}.\vk,\mathsf{nad}.\ct)\la\mathsf{NAD}.\Enc(\mathsf{nad}.\MPK,m)$.
    \item Generate $a,c\la\bit^n$. Let $\Psi\seteq Z^cX^a\mathsf{nad}.\ct X^aZ^c$.
    \item Compute $(\nce.\vk,\nce.\ct)\la\NCE.\Enc(\nce.\pk,(a,c))$.
    \item Output $\vk\seteq(\mathsf{nad}.\vk,\nce.\vk,a,b)$ and $\ct\seteq (\Psi,\nce.\ct)$.
\end{itemize}
\item[$\Dec(\sk_f,\ct)$:]$ $
\begin{itemize}
    \item Parse $\sk_f=(\nce.\sk,\mathsf{nad}.\sk_f)$ and $\ct=(\Psi,\nce.\ct)$.
    \item Compute $((a',c'),\widehat{\nce.\ct})\la\NCE.\Dec(\nce.\sk,\nce.\ct)$.
    \item Compute $\mathsf{nad}.\ct'\seteq X^{a'}Z^{c'}\Psi Z^{c'}X^{a'}$.
    \item Compute $(y,\widehat{\mathsf{nad}.\ct'})\la\mathsf{NAD}.\Dec(\mathsf{nad}.\sk_f,\mathsf{nad}.\ct')$.
    Let $\widehat{\Psi}\seteq Z^{c'}X^{a'}\widehat{\mathsf{nad}.\ct'}X^{a'}Z^{c'}$.
    \item Output $y$ and $\widehat{\ct}=(\widehat{\Psi},\widehat{\nce.\ct})$.
\end{itemize}
\item[$\Delete(\ct)$:]$ $
\begin{itemize}
    \item Parse $\ct=(\Psi,\nce.\ct)$.
    \item Compute $\nad.\cert^*\la \NAD.\Delete(\Psi)$.
    \item Compute $\nce.\cert\la\NCE.\Delete(\nce.\ct)$.
    \item Output $\cert\seteq(\nad.\cert,\nce.\cert)$.
\end{itemize}
\item[$\Vrfy(\vk,\cert)$:]$ $
\begin{itemize}
    \item Parse $\vk=(\mathsf{nad}.\vk,\nce.\vk,a,b)$ and $\cert_0=(\nad.\cert^*,\nce.\cert)$.
    \item Compute $\mathsf{nad}.\cert\la\NAD.\Modify (a,c,\nad.\cert^*)$.
    \item Output $\top$ if $\top\la\NCE.\Vrfy(\nce.\vk,\nce.\cert)$ and $\top\la\mathsf{NAD}.\Vrfy(\mathsf{nad}.\vk,\mathsf{nad}.\cert)$.
    Otherwise, output $\bot$.
\end{itemize}
\end{description}
\paragraph{Correctness:}
Decryption correctness easily follows from decryption correctness of $\Sigma_{\mathsf{nad}}$ and $\Sigma_{\mathsf{cence}}$.
Verification correctness easily follows from modification correctness of $\Sigma_{\mathsf{nad}}$ and verification correctness of $\Sigma_{\mathsf{cence}}$.
Rewind correctness easily follows from rewind correctness of $\Sigma_{\nad}$ and $\Sigma_{\mathsf{cence}}$.

\paragraph{Security:}
We prove the following two theorems.
\begin{theorem}\label{thm:comp_security_single_ad}
If $\Sigma_{\mathsf{nad}}$ satisfies the single-key non-adaptive security and $\Sigma_{\mathsf{cence}}$ satisfies the RNC security, 
$\Sigma_{\mathsf{cefe}}$ satisfies the single-key adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:comp_security_single_ad}]
The proof is similar to that of \cref{thm:comp_security_single_ad}.
\end{proof}

\begin{theorem}\label{thm:ever_security_single_ad}
If $\Sigma_{\mathsf{nad}}$ satisfies the single-key certified everlasting non-adaptive security and $\Sigma_{\mathsf{cence}}$ satisfies the certified everlasting RNC security, 
$\Sigma_{\mathsf{cefe}}$ satisfies the single-key certified everlasting adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:ever_security_single_ad}]
Obviously, the security holds against an adversary which makes an function query before it makes a challenge query.
This is because $\Sigma_{\mathsf{nad}}$ is single-key certified everlasting non-adaptive secure.
Hence, we consider the adversary $\cA$ which makes an function query after it makes a challenge query.
For clarity, we describe how the experiment works against the adversary $\cA\seteq(\cA_1,\cA_2)$
consisting of any QPT adversary $\cA_1$ and any unbounded time adversary $\cA_2$.
\begin{description}
\item[$\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)$:]This is the original experiment.
\begin{enumerate}
    \item The challenger generates $(\mathsf{nad}.\MPK,\mathsf{nad}.\MSK)\la\mathsf{NAD}.\Setup(1^\secp)$ and $(\nce.\pk,\nce.\MSK)\la\NCE.\Setup(1^{\secp})$, and sends $(\nce.\pk,\mathsf{nad}.\MPK)$ to $\cA_1$.
    \item $\cA_1$ submits a message pair $(m_0,m_1)\in\Ms$ to the challenger.
    The challenger generates $a,c\la\bit^n$,
    computes $(\mathsf{nad}.\vk,\mathsf{nad}.\CT)\la \mathsf{NAD}.\Enc(\mathsf{nad}.\MPK,m_b)$,
    $\Psi\seteq Z^{c}X^{a}\mathsf{nad}.\ct X^{a}Z^{c}$,
    and $(\nce.\vk,\nce.\ct)\la\NCE.\Enc(\nce.\pk,(a,c))$,
    and sends $(\Psi,\nce.\CT)$ to $\cA_1$.
    \item $\cA_1$ is allowed to make an arbitrary function query at most one time.
    For the function query, the challenger receives $f\in\mathcal{F}$,  
    computes $\nce.\sk\la\NCE.\keygen(\nce.\MSK)$
    and $\mathsf{nad}.\sk_{f}\la\mathsf{NAD}.\keygen(\mathsf{nad}.\MSK,f)$,
    and sends $(\nce.\sk,\mathsf{nad}.\sk_{f})$ to $\cA_1$.
    \item 
     $\cA_1$ sends $(\nce.\cert,\nad.\cert)$ to the challenger and its internal state to $\cA_2$.
    \item The challenger computes $\mathsf{nad}.\cert\la\NAD.\Modify(a,c,\nad.\cert^*)$.
        The challenger computes $\NCE.\Vrfy(\nce.\vk,\nce.\cert)$ and $\mathsf{NAD}.\Vrfy(\mathsf{nad}.\vk,\mathsf{nad}.\cert)$.
        If the results are $\top$, the challenger outputs $\top$ and sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
        Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item The experiment outputs $b'$ if $f(m_0)=f(m_1)$ and the challenger outputs $\top$. Otherwise, the experiment outputs $\bot$.
\end{enumerate}
What we have to prove is that 
\begin{align}
    \advc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp)
\seteq \abs{\Pr[ \expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, 0)=1] - \Pr[ \expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, 1)=1] }\leq \negl(\secp).
\end{align}
We define the following sequence of hybrids.
\item[$\sfhyb{1}{}(b)$:] $ $
This is identical to $\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, b)$ except for the following four points. 
First, the challenger computes $(\nce.\vk,\widetilde{\nce.\ct},\nce.\aux)\la\NCE.\Fake(\nce.\pk,\nce.\MSK)$ instead of computing $(\nce.\vk,\nce.\ct)\la\NCE.\Enc(\nce.\pk,(a,c))$.
Second, the challenger sends $(\Psi,\widetilde{\nce.\ct})$ to $\cA_1$ instead of sending $(\Psi,\nce.\ct)$ to $\cA_1$.
Third, the challenger computes $\widetilde{\nce.\sk}\la \NCE.\Reveal(\nce.\pk,\nce.\MSK,\nce.\aux,(a,c))$ instead of computing $\nce.\sk\la\NCE.\keygen(\nce.\MSK)$.
Fourth, the challenger sends $(\Psi,\widetilde{\nce.\sk})$ to $\cA_1$ instead of sending $(\Psi,\nce.\sk)$ to $\cA_1$.

\item[$\sfhyb{2}{}(b)$:]$ $
This is identical to $\sfhyb{1}{}(b)$ except for the following five points.
First, the challenger generates $|\widetilde{0^n0^n}\rangle$ instead of computing $\Psi\seteq Z^{c}X^{a}\mathsf{nad}.\ct X^{a}Z^{c}$.
Let $\Psi_A\seteq\Tr_B(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$ and
$\Psi_B\seteq\Tr_A(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$.
Second, the challenger sends $(\Psi_A,\widetilde{\nce.\ct})$ to $\cA_1$ instead of sending $(\Psi,\widetilde{\nce.\ct})$ to $\cA_1$.
Third, the challenger measures 
the $i$-th qubit of $\mathsf{nad}.\ct$ and $\Psi_B$ in the Bell basis and let $(x_i,z_i)$ be the measurement outcome for all $i\in[N]$.
Fourth, the challenger computes $\widetilde{\nce.\sk}\la\NCE.\Reveal(\nce.\pk,\nce.\MSK,\nce.\aux,(x,z))$ instead of computing  $\widetilde{\nce.\sk}\la\NCE.\Reveal(\nce.\pk,\nce.\MSK,\nce.\aux,(a,c))$,
and sends $\widetilde{\nce.\sk}$ to $\cA_1$ instead of sending $\nce.\sk$ to $\cA_1$.
Fifth, the challenger computes $\mathsf{nad}.\cert\la\NAD.\Modify(x,z,\nad.\cert^*)$ instead of computing $\mathsf{nad}.\cert\la\NAD.\Modify(a,c,\nad.\cert^*)$.
\end{description}

\cref{thm:ever_security_single_ad} easily follows from \cref{prop:exp_hyb_1_cefe_si_ad,prop:hyb_1_hyb_2_cefe_si_ad,prop:hyb_2_cefe_si_ad}.
(Whose proof is given later.)
\end{proof}

\begin{proposition}\label{prop:exp_hyb_1_cefe_si_ad}
If $\Sigma_{\mathsf{cence}}$ is certified everlasting RNC secure, 
it holds that
\begin{align}
\abs{\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]-\Pr[\sfhyb{1}{}(b)=1]}\leq\negl(\secp)
\end{align}
for $b\in\bit$.
\end{proposition}

\begin{proposition}\label{prop:hyb_1_hyb_2_cefe_si_ad}
$\Pr[\sfhyb{1}{}(b)]=\Pr[\sfhyb{2}{}(b)]$ for $b\in\bit$.
\end{proposition}

\begin{proposition}\label{prop:hyb_2_cefe_si_ad}
If $\Sigma_{\mathsf{nad}}$ is single-key certified everlasting non-adaptive secure,
it holds that
\begin{align}
    \abs{\Pr[\sfhyb{2}{}(0)=1]-\Pr[\sfhyb{2}{}(1)=1]}\leq\negl(\secp).
\end{align}
\end{proposition}

\begin{proof}[Proof of \cref{prop:exp_hyb_1_cefe_si_ad}]
We assume that $\abs{\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is non-negligible, and construct an adversary $\cB$ that breaks the certified everlasting RNC security of $\Sigma_{\mathsf{cence}}$.
Let us describe how $\cB$ works below.
\begin{enumerate}
    \item $\cB$ receives $\nce.\pk$ from the challenger of $\expd{\Sigma_{\mathsf{cence}},\cB}{cert}{ever}{rec}{nc}(\secp,b')$,
    generates $(\mathsf{nad}.\MPK,\mathsf{nad}.\MSK)\la \mathsf{NAD}.\keygen(1^\secp)$,
    and sends $(\nce.\pk,\mathsf{nad}.\MPK)$ to $\cA_1$.
    \item $\cB$ receives a message pair $(m_0,m_1)\in\Ms$, computes $(\mathsf{nad}.\vk,\mathsf{nad}.\ct)\la\mathsf{NAD}.\Enc(\mathsf{nad}.\MPK,m_{b'})$, generates $a,c\la\bit^n$, computes $\Psi\seteq Z^cX^a\mathsf{nad}.\ct X^aZ^c$, sends $(a,c)$ to the challenger, receives $\nce.\ct^*$ from $\cA_1$, and sends $(\Psi,\nce.\ct^*)$ to $\cA_1$.
    \item $\cA_1$ is allowed to send an function query at most one time.
    For an function query, $\cB$ receives an function query $f$, $\cB$ generates $\mathsf{nad}.\sk_f\la\mathsf{NAD}.\keygen(\mathsf{nad}.\MSK,f)$,
    call a key query to the challenger, receives $\nce.\sk^*$ from the challenger, and sends $(\nce.\sk^*,\mathsf{nad}.\sk_f)$ to $\cA_1$.
    \item $\cA_1$ sends $(\nce.\cert,\mathsf{nad}.\cert^*)$ to $\cB$ and its internal state to $\cA_2$.
    \item $\cB$ sends $\nce.\cert$ to the challenger, and receives $\nce.\MSK$ or $\bot$ from the challenger.
    $\cB$ computes $\mathsf{nad}.\cert\la\NAD.\Modify(a,c,\nad.\cert^*)$ and $\mathsf{NAD}.\Vrfy(\mathsf{nad}.\vk,\mathsf{nad}.\cert)$.
    If the result is $\top$ and $\cB$ receives $\nce.\MSK$ from the challenger,
    $\cB$ sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
    Otherwise, $\cB$ outputs $\bot$, sends $\bot$ to $\cA_2$, and aborts.
    \item $\cA_2$ outputs $b''$.
    \item $\cB$ outputs $b''$ if $f(m_0)=f(m_1)$. 
\end{enumerate}
It is clear that $\Pr[1\la\cB|b'=0]=\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]$ and $\Pr[1\la\cB|b'=1]=\Pr[\sfhyb{1}{}(b)=1]$.
By assumption, $\abs{\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is non-negligible, and therefore $\abs{\Pr[1\la\cB|b'=0]-\Pr[1\la\cB|b'=1]}$ is non-negligible, which contradicts the certified everlasting RNC security of $\Sigma_{\mathsf{cence}}$. 


\begin{proof}[Proof of \cref{prop:hyb_1_hyb_2_cefe_si_ad}]
We clarify the difference between $\sfhyb{1}{}$ and $\sfhyb{2}{}$.
First, in $\sfhyb{2}{}$, the challenger runs $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux,(x,z))$ instead of running $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux,(a,c))$ as in $\sfhyb{1}{}$.
Second, in $\sfhyb{2}{}$, the challenger sends $\Psi_A$ to $\cA_1$ instead of sending $Z^{c}X^{a}\mathsf{nad}.\ct X^{a}Z^{c}$ to $\cA_1$ as in $\sfhyb{1}{}$.
Hence,
it is sufficient to prove that $x$ and $z$ are uniformly randomly distributed and
$\Psi_A$ is identical to $Z^{z}X^{x}\mathsf{nad}.\ct X^{x}Z^{z}$.
These two things are obvious from \cref{lem:quantum_teleportation}.
\end{proof}


\begin{proof}[Proof of \cref{prop:hyb_2_cefe_si_ad}]
We assume that $\abs{\Pr[\sfhyb{2}{}(0)=1]-\Pr[\sfhyb{2}{}(1)=1]}$ is non-negligible, and construct an adversary $\cB$ that breaks the single-key certified everlasting non-adaptive security of $\Sigma_{\mathsf{nad}}$.
Let us describe how $\cB$ works below.
\begin{enumerate}
    \item $\cB$ receives $\mathsf{nad}.\MPK$ from the challenger of $\expd{\Sigma_{\mathsf{nad}},\cB}{cert}{ever}{non}{adapt}(\secp,b)$, 
    generates $(\nce.\pk,\nce.\MSK)\la\NCE.\Setup(1^\secp)$, and sends $(\nce.\pk,\mathsf{nad}.\MPK)$ to $\cA_1$.
    \item $\cB$ receives a challenge query $(m_0,m_1)\in\Ms$ from $\cA_1$,
    computes $(\nce.\vk,\widetilde{\nce.\ct},\nce.\aux)\la\NCE.\Fake(\nce.\pk,\nce.\MSK)$,
    and generates $|\widetilde{0^n0^n}\rangle$.
    Let $\Psi_A\seteq\Tr_B(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$ and
    $\Psi_B\seteq\Tr_A(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$.
    $\cB$ sends $(\Psi_A,\widetilde{\nce.\ct})$ to $\cA_1$.
    \item
    $\cA_1$ is allowed to make an function query at most one time.
    For an function query, $\cB$ receives $f$ from $\cA_1$, sends $f$ to the challenger as an function query, and receives $\mathsf{nad}.\sk_f$ from the challenger.
    \item $\cB$ sends a challenge query $(m_0,m_1)$ to the challenger, receives $\mathsf{nad}.\ct$, and measures the $i$-th qubit of $\mathsf{nad}.\ct$ and $\Psi_B$ in the Bell basis and let $(x_i,z_i)$ be the measurement outcome for all $i\in[N]$.
    \item If $\cA_1$ makes an function query, $\cB$ generates $\widetilde{\nce.\sk}\la\NCE.\Reveal(\nce.\pk,\nce.\MSK,\nce.\aux,(x,z))$, and sends $(\widetilde{\nce.\sk},\mathsf{nad}.\sk_f)$ to $\cA_1$.
    \item $\cA_1$ sends $(\nce.\cert,\mathsf{nad}.\cert^*)$ to $\cB$ and its internal state to $\cA_2$.
    \item $\cB$ computes $\mathsf{nad}.\cert\la\NAD.\Modify(x,z,\nad.\cert^*)$,
        sends $\mathsf{nad}.\cert$ to the challenger, and receives $\mathsf{nad}.\MSK$ or $\bot$ from the challenger.
        $\cB$ computes $\NCE.\Vrfy(\nce.\vk,\nce.\cert)$.
        If the result is $\top$ and $\cB$ receives $\mathsf{nad}.\MSK$ from the challenger, $\cB$ sends $(\nce.\MSK,\mathsf{nad}.\MSK)$ to $\cA_2$.
        Otherwise, $\cB$ outputs $\bot$, sends $\bot$ to $\cA_2$, and aborts.
    \item $\cA_2$ outputs $b'$.
    \item $\cB$ outputs $b'$ if $f(m_0)=f(m_1)$. 
\end{enumerate}

It is clear that $\Pr[1\la\cB|b=0]=\Pr[\sfhyb{2}{}(0)=1]$ and $\Pr[1\la\cB|b=1]=\Pr[\sfhyb{2}{}(1)=1]$.
By assumption, $\abs{\Pr[\sfhyb{}{}(0)=1]-\Pr[\sfhyb{1}{}(1)=1]}$ is non-negligible, and therefore $\abs{\Pr[1\la\cB|b=0]-\Pr[1\la\cB|b=1]}$ is non-negligible, which contradicts the single-key certified everlasting non-adaptive security of $\Sigma_{\mathsf{nad}}$. 
\end{proof}
By \cref{prop:exp_hyb_1_cefe_si_ad,prop:hyb_1_hyb_2_cefe_si_ad,prop:hyb_2_cefe_si_ad}, we immediately obtain \cref{thm:ever_security_single_ad}.
\end{proof}




{
\color{red}
\subsection{Construction of $q$-Bounded Certified Everlasting Functional Encryption for NC1 circuits}\label{sec:const_multi_fe}
In this section, we present how to construct a $q$-bounded certified everlasting functional encryption scheme for NC1 circuits from single-key certified everlasting functional encryption.
Our construction uses BGW semi-honest MPC protocol without degree reduction~\cite{}.

We construct a $q$-bounded certified everlasting FE scheme for a circuit family $\mathcal{C}\seteq NC1$.
In particular, we consider polynomial representation of circuits $C$ in the family.
The input message space $\chi=\mathbb{F}^{\ell}$ is an $\ell$ tuple of field elements, and for every circuits $C\in\mathcal{C}$, $C(\cdot)$ is an $\ell$-variate polynomial over $\mathbb{F}$ of total degree at most $D$.



\paragraph{Our bounded collusion certified everlasting FE scheme for NC1 circuits.}
Let $\mathcal{C}\seteq NC1$ be a circuit family with circuits of degree $D=D(\lambda)$ in its input, and let $q=q(\lambda)$ be a bound on the number of secret key queries. Our scheme is associated wit additional parameters $S=S(\lambda)$, $N=N(\lambda)$, $t=t(\lambda)$ and $v=v(\lambda)$.
In our construction, we set these parameters as follows:
\begin{align}
    t(\lambda)=\Theta(q^2\lambda), N(\lambda)=\Theta(D^2q^2t), v(\lambda)=\Theta(\lambda), S(\lambda)=\Theta(vq^2)
\end{align}

We start by defining a new family $\mathcal{G}$ as follows:
\begin{align}
G_{C,\Delta}(x,Z_1,Z_2,\cdots,Z_S)\seteq C(x)+\sum_{i\in\Delta}Z_i    
\end{align}
where $\Delta\subseteq[S]$ and $Z_1,\cdots,Z_S\in\mathbb{F}$.

We construct a $q$-bounded certified everlasting FE scheme for NC1 circuits  $\Sigma_{\mathsf{cefe}}=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$
from a single-key certified everlasting FE scheme $\Sigma_{\mathsf{one}}=\mathsf{ONE}.(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$.

\begin{description}
\item[$\Setup(1^\lambda)$:]$ $
\begin{itemize}
    \item For $i\in[N]$, generate $(\mathsf{one}.\MPK_i,\mathsf{one}.\MSK_i)\la\mathsf{ONE}.\Setup(1^\secp)$.
    \item Output $\MPK\seteq\{\mathsf{one}.\MPK_i\}_{i\in[N]}$ and $\MSK\seteq \{\mathsf{one}.\MSK_i\}_{i\in[N]}$.
\end{itemize}
\item[$\keygen(\MSK,C)$:]$ $
\begin{itemize}
    \item Parse $\MSK= \{\mathsf{one}.\MSK_i\}_{i\in[N]}$.
    \item Chooses a uniformly random set $\Gamma\subseteq[N]$ of size $tD+1$.
    \item Chooses a uniformly random set $\Delta\subseteq[S]$ of size $v$.
    \item For $i\in\Gamma$, compute $\mathsf{one}.\sk_{C,\Delta,i}\la\mathsf{ONE}.\keygen(\one.\MSK_i,G_{C,\Delta})$.
    \item Output $\sk_{C}\seteq (\Gamma,\Delta,\{\one.\sk_{C,\Delta,i}\}_{i\in\Gamma})$.
\end{itemize}
\item[$\Enc(\MPK,x)$:]$ $
\begin{itemize}
    \item Parse $\MPK=\{\mathsf{one}.\MPK_i\}_{i\in[N]}$.
    \item For $i\in[\ell]$, pick a random degree $t$ polynomial $\mu_i(\cdot)$ whose constant term is $x[i]$.
    \item For $i\in[S]$, pick a random degree $Dt$ polynomial $\xi_i(\cdot)$ whose constant term is $0$.
    \item For $i\in[N]$, compute $(\one.\vk_i,\one.\ct_i)\la\ONE.\Enc(\one.\MPK_i,(\mu_1(i),\cdots,\mu_{\ell}(i),\xi_1(i),\cdots,\xi_S(i) ))$.
    \item Output $\vk=\{\one.\vk_i\}_{i\in[N]}$ and $\ct\seteq\{\one.\ct_i\}_{i\in[N]}$.
    \end{itemize}
\item[$\Dec(\sk_C,\ct)$:]$ $
\begin{itemize}
    \item Parse $\sk_{C}= (\Gamma,\Delta,\{\one.\sk_{C,\Delta,i}\}_{i\in\Gamma})$ and $\ct=\{\one.\ct_i\}_{i\in[N]}$.
    \item For $i\in \Gamma$, compute $(\eta(i),\widehat{\one.\ct}_i)\la\ONE.\Dec(\one.\sk_{C,\Delta,i},\one.\ct_i)$.
    Let $\widehat{\one.\ct}_i\seteq \one.\ct_i$ for $i\in[N]/\Gamma$.
    \item Output $\eta(0)$ and $\widehat{\one.\ct}\seteq \{\widehat{\one.\ct}_i\}_{i\in[N]}$.
\end{itemize}
\item[$\Delete(\ct)$:]$ $
\begin{itemize}
    \item Parse $\ct=\{\one.\ct_i\}_{i\in[N]} $.
    \item For $i\in[N]$, compute $\one.\cert_i\la\ONE.\Delete(\one.\ct_i)$.
    \item Output $\cert\seteq \{\one.\cert_i\}_{i\in[N]}$.
\end{itemize}
\item[$\Vrfy(\vk,\cert)$:]$ $
\begin{itemize}
    \item Parse $\vk=\{\one.\vk_i\}_{i\in[N]}$ and $\cert= \{\one.\cert_i\}_{i\in[N]}$.
    \item For $i\in[N]$, compute $\top/\bot\la\ONE.\Vrfy(\one.\vk_i,\one.\cert_i)$.
    \item If all results are $\top$, output $\top$. Otherwise, output $\bot$.
\end{itemize}
\end{description}

\paragraph{Correctness:}
By decryption correctness of the $\Sigma_{\one}$, for all $i\in\Gamma$ we have 
\begin{align}
\eta(i)&=G_{C,\Delta} (\mu_1(i),\cdots,\mu_\ell(i),\xi_1(i),\cdots,\xi_S(i))\\
&=C(\mu_1(i),\cdots,\mu_\ell(i))+\Sigma_{a\in\Delta}\xi_a(i).
\end{align}
Since $|\Gamma|\geq Dt+1$, this means that $\eta$ is equal to the degree $Dt$ polynomial 
\begin{align}
    \eta(\cdot)=C(\mu_1(\cdot),\cdots,\mu_\ell(\cdot) )+\Sigma_{a\in\Delta}\xi_a(\cdot)
\end{align}
Hence $\eta(0)=C(x_1,\cdots,x_\ell)=C(x)$, which means that our construction satisfies decryption correctness.

Verification correctness easily follows from verification correctness of $\Sigma_{\one}$.




\paragraph{Security:}
We prove the following theorems.
\begin{theorem}\label{thm:compt_bounded_fe}
If $\Sigma_{\one}$ satisfies the single-key non-adaptive security, $\Sigma_{\mathsf{cefe}}$ satisfies the $q$-non-adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:compt_bounded_fe}]
The proof is very similar to that of \cref{thm:ever_bounded_fe}. Therefore, we skip the proof.
\end{proof}


\begin{theorem}\label{thm:ever_bounded_fe}
If $\Sigma_{\one}$ satisfies the single-key certified everlasting non-adaptive security,
$\Sigma_{\mathsf{cefe}}$ the $q$-certified everlasting non-adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:ever_bounded_fe}]
For clarity, we describe how the experiment works against an adversary $\cA\seteq(\cA_1,\cA_2)$ consisting of any QPT adversary $\cA_1$ and any unbouded adversary $\cA_2$.
\begin{description}
\item [$\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)$:] This is the original experiment.
\begin{enumerate}
    \item\label{step:keygen_bounded_fe} The challenger generates $(\one.\MPK_i,\one.\MSK_i)\la\ONE.\Setup(1^\secp)$ for $i\in[N]$.
    \item $\cA_1$ is allowed to call a key query at most $q$ times.
    For $j$-th key query, the challenger receives an function $C_{j}$ from $\cA_1$, generates a uniformly random set $\Gamma_{j}\in[N]$ of size $tD+1$ and $\Delta_{j}\in [S]$ of size $v$.
    For $i\in \Gamma_{j}$, the challenger generates $\mathsf{one}.\sk_{C_{j},\Delta_{j},i}\la\mathsf{ONE}.\keygen(\one.\MSK_i,G_{C_{j},\Delta_{j}})$, and sends $(\Gamma_{j},\Delta_{j},\{\one.\sk_{C_{j},\Delta_{j},i}\}_{i\in\Gamma_{j}})$ to $\cA_1$.
    Let $q^*$ be the number of times that $\cA_1$ has called key queries in this step.
    \item $\cA_1$ chooses $(x_0,x_1)\in\Ms^2$ and sends $(x_0,x_1)$ to the challenger.
    \item The challenger generates a random degree $t$ polynomial $\mu_i(\cdot)$ whose constant is $x_b[i]$ for $i\in[\ell]$
    and a random degree $Dt$ polynomial $\xi_i(\cdot)$ whose constant term is $0$.
    For $i\in[N]$, the challenger computes $(\one.\vk_i,\one.\ct_i)\la\ONE.\Enc(\one.\MPK_i,(\mu_1(i),\cdots,\mu_{\ell}(i),\xi_1(i),\cdots,\xi_S(i)))$,
    and sends $\{\one.\ct_i\}_{i\in[N]}$ to $\cA_1$.
    \item $\cA_1$ is allowed to call a key query at most $q-q^*$ times.
    For $j$-th key query, the challenger receives an function $C_{j}$ from $\cA_1$, generates a uniformly random set $\Gamma_{j}\in[N]$ of size $tD+1$ and $\Delta_{j}\in [S]$ of size $v$.
    For $i\in \Gamma_{j}$, the challenger generates $\mathsf{one}.\sk_{C_{j},\Delta_{j},i}\la\mathsf{ONE}.\keygen(\one.\MSK_i,G_{C_{j},\Delta_{j}})$, and sends $(\Gamma_{j},\Delta_{j},\{\one.\sk_{C_{j},\Delta_{j},i}\}_{i\in\Gamma_{j}})$ to $\cA_1$.
    Let $q'$ be the number of times that $\cA_1$ has called key queries in this step.
    \item $\cA_1$ sends $\{\one.\cert_i\}_{i\in[N]}$ to the challenger and its internal state to $\cA_2$.
    \item If $\top\la \ONE.\Vrfy(\one.\vk_i,\one.\cert_i)$ for all $i\in[N]$, the challenger outputs $\top$ and sends $\{\one.\MSK_i\}_{i\in[N]}$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item The experiment outputs $b'$ if $C_i(x_0)=C_i(x_1)$ for all $i\in[q^*+q']$ and the challenger outputs $\top$.
    Otherwise, the challenger outputs $\bot$.
\end{enumerate}
What we have to prove is that 
\begin{align}
    \advd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp)
\seteq \abs{\Pr[ \expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, 0)=1] - \Pr[ \expd{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{non}{adapt}(\secp, 1)=1] }\leq \negl(\secp).
\end{align}
We define the following sequence of the hybrids.
\item[$\sfhyb{1}{}(b)$:] This is identical to $\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,b)$ except that the challenger generates uniformly random set $\Gamma_i\in[N]$ of size $tD+1$ and $\Delta_{i}\in [S]$ of size $v$ for $i\in[q]$ in step \ref{step:keygen_bounded_fe} instead of generating them when a key query is called.
\item[$\sfhyb{2}{}(b)$:]To describe the difference, let us define some notations.
Let $\mathcal{L}\seteq\bigcup_{j\neq j'}(\Gamma_j\cap \Gamma_{j'})$ and let $\Delta_{0}\seteq \emptyset$.
This is identical to $\sfhyb{1}{}(b)$ except for the following points.
The challenger samples the polynomials $\xi_1,\cdots ,\xi_S$
%in \ref{step:keygen_bounded_fe}
as follows.
For $i\in [q]$:
\begin{itemize}
    \item[(a)] fix some $a^*\in\Delta_i \in(\Delta_0,\cdots \Delta_{i-1})$;
    \item[(b)] for all $a\in\left(\Delta_i \in(\Delta_0,\cdots \Delta_{i-1})\right)/\{a^*\}$, set $\xi_a$ to be uniformly random degree $Dt$ polynomial whose constant term is $0$;
    \item[(c)] if $i \leq q^*$, pick a random degree $Dt$ polynomial $\eta_i(\cdot)$ whose constant term is $C_i(x_b)$; 
    if $i>q^*$, pick random values for $\eta_i(j)$ for all $j\in \mathcal{L}$;
    \item[(d)] the evaluation of $\xi_{a^*}$ on the points in $\mathcal{L}$ is defined by the relation:
    \begin{align}
        \eta_i(\cdot)=C_i(\mu_1(\cdot),\cdots, \mu_\ell(\cdot)) +\sum_{a\in \Delta_i }\xi_a(\cdot).
    \end{align}
    \item[(e)] Finally, for all $a\notin (\Delta_1\cap\cdots \cap \Delta_q)$, set $\xi_a$ to be a uniformly random degree $Dt$ polynomial whose constant term is $0$. 
\end{itemize}
\item[$\sfhyb{3}{}(b)$:]
This is identical to $\sfhyb{2}{}(b)$ except for the following points.
For $i\notin [N]/\mathcal{L}$, the challenger samples $\mu_1(i),\cdots, \mu_\ell(i)$ as follows.
\begin{itemize}
\item In the case $i\in\Gamma_j$ for $j\in[q^*]$, the challenger pick random value for $\mu_1(i),\cdots, \mu_\ell(i)$ 
on the condition $\eta_j(i)\seteq C_j(\mu_1(i)\cdots \mu_\ell(i))+\sum_{a\in\Delta_j}\xi_a(i)$.
\item In the case if no such set exist or $j> q^*$, the challenger picks random value for $\mu_1(i),\cdots, \mu_\ell(i)$.
\end{itemize}
The challenger computes $(\one.\vk_i,\one.\ct_i)\la\ONE.\Enc(\one.\MPK_i,(\mu_1(i),\cdots ,\mu_\ell(i),\xi_1(i),\cdots,\xi_S(i)))$ for $i\in[N]/ \mathcal{L}$.

\end{description}
\end{proof}
}





==> Old_RNCE.tex <==
\paragraph{Certified Everlasting RNCE for Quantum Message.}
\begin{definition}[Certified Everlasting RNCE for Quantum Message]\label{def:cert_ever_rnce_quantum}
Let $\secp$ be the security parameter and let $p$, $q$, $r$, $s$, $t$, $u$, and $v$ be some polynomials. 
A certified everlasting receiver non-committing encryption scheme for quantum message is a tuple of algorithm $\Sigma=(\Setup,\keygen,\Enc,\Dec,\Fake,\Reveal,\Delete_0,\Delete_1,\Vrfy_0,\Vrfy_1)$
with plaintext space $\Ms\seteq\cQ^{\otimes n}$,
ciphertext space $\Cs:= \cQ^{\otimes p(\lambda)}$,
public key space $\mathcal{PK}:=\{0,1\}^{q(\lambda)}$,
secret key space $\mathcal{SK}\seteq \bit^{r(\secp)}$,
master secret key space $\mathcal{MSK}\seteq\bit^{s(\secp)}$
verification key space $\mathcal{VK}\seteq \bit^{t(\secp)}$,
deletion certificate space $\mathcal{D}:= \{0,1\}^{u(\lambda)}$,
and auxiliary space $\mathcal{AUX}\seteq\bit^{v(\lambda)}$.
\begin{description}
    \item[$\Setup(1^\secp)\ra(\pk,\MSK)$:]The setup algorithm takes the security parameter $1^\secp$ as input, and outputs a public key $\pk\in\mathcal{PK}$ and a master secret key $\MSK\in\mathcal{MSK}$.
    \item[$\keygen (\MSK) \ra \sk$:]
    The key generation algorithm takes the security parameter $1^\secp$ as input, and outputs a secret key $\sk\in\mathcal{SK}$.
    \item[$\Enc(\pk,\rho) \ra (\vk,\ct)$:]
    The encryption algorithm takes $\pk$ and a plaintext $\rho\in\Ms$ as input,
    and outputs a verification key $\vk\in\mathcal{VK}$ and a ciphertext $\ct\in \Cs$.
    \item[$\Dec(\sk,\ct) \ra \rho^\prime~or~\bot$:]
    The decryption algorithm takes $\sk$ and $\ct$ as input, and outputs a plaintext $\rho^\prime \in \Ms$ or $\bot$.
    \item[$\Fake(\pk,\MSK)\ra (\vk,\widetilde{\CT},\aux)$:]
    The fake encryption algorithm takes $\pk$ and $\MSK$ as input, and outputs a verification key $\vk\in\mathcal{VK}$, a fake ciphertext $\widetilde{\CT}\in \Cs$ and an auxiliary state $\aux\in\mathcal{AUX}$.
    \item[$\Reveal(\pk,\MSK,\aux,\rho )\ra \widetilde{\sk}$:]
    The reveal algorithm takes $\pk, \MSK$, $\aux$ and $\rho$ as input, and outputs a fake secret key $\widetilde{\sk}\in\mathcal{SK}$.
     \item[$\Delete_0(\ct) \ra \cert_0$:]
    The deletion algorithm $\Delete_0$ takes $\ct$ as input, and outputs a certification $\cert_0\in\mathcal{D}$.
    \item[$\Delete_1(\ct,\sk) \ra (\cert_1,\rho^*)$:]
    The deletion algorithm $\Delete_1$ takes $\ct$ and $\sk$ as input, and outputs a certification $\cert_1\in\mathcal{D}$ and $\rho^*$.
    \item[$\Vrfy_0(\vk,\cert_0)\ra \top~\mbox{\bf or}~\bot$:]
    The verification algorithm $\Vrfy_0$ takes $\vk$ and $\cert_0$ as input, and outputs $\top$ or $\bot$.
    \item[$\Vrfy_1(\vk,\sk,\cert_1)\ra \top~\mbox{\bf or}~\bot$:]
    The verification algorithm $\Vrfy_1$ takes $\vk$ and $\cert_1$ as input, and outputs $\top$ or $\bot$.
    \end{description}
\end{definition}
%\begin{remark}
%Note that the secret key space of the RNCE shceme must be quantum space.
%This is because if there exists the RNCE scheme with the classical secret key space,
%we can break quantum no-cloning theorem using it.
%This can be done as follows.

%Let us consider the situation we have some quantum states $\rho$.
%By running $\keygen$, we can obtain $(\pk,\sk,\aux)$.
%We can obtain multiple fake ciphertext $(\widetilde{\ct_1},\cdots,\widetilde{\ct_n})$ by running $\Fake$ multiple times.
%We can also obtain a classical secret key $\widetilde{\sk}$ by running $\Reveal$ on $\rho$.
%Since $\widetilde{\sk}$ is classical bit strings, we can copy $\widetilde{\sk}$ freely.
%Thus, we can obtain multiple $\rho$ by running $\Dec (\widetilde{\ct_j},\widetilde{\sk})$ for each $j\in[n]$
%by the correctness and the RNC security of the scheme.
%This means that we can break quantum no-cloning theorem by using the scheme.
%\end{remark}

\begin{definition}[Correctness for Certified Everlasting RNCE for Quantum Message]\label{def:correctness_cert_ever_nce_quantum}
There are two types of correctness. One is decryption correctness and the other is verification correctness.

\paragraph{Decryption Correctness:}
There exists a negligible function $\negl$ such that for any $\secp\in \N$ and $\rho\in\Ms$,
\begin{align}
\Pr\left[
\frac{1}{2}\norm{\rho-\rho^*}_{\tr}\leq\negl(\lambda)
\ \middle |
\begin{array}{ll}
(\pk,\MSK)\lrun \Setup(1^\secp)\\
(\vk,\ct) \lrun \Enc(\pk,\rho)\\
\sk\la\keygen(\MSK)\\
\rho^*\la\Dec(\sk,\ct)
\end{array}
\right] 
\leq1-\negl(\lambda),
\end{align}
and
\begin{align}
\Pr\left[
\frac{1}{2}\norm{\rho-\rho^*}_{\tr}\leq\negl(\lambda)
\ \middle |
\begin{array}{ll}
(\pk,\MSK)\lrun \Setup(1^\secp)\\
(\vk,\ct) \lrun \Enc(\pk,\rho)\\
\sk\la\keygen(\MSK)\\
(\cert_1,\rho^*)\la\Delete_1(\ct,\sk)
\end{array}
\right] 
\leq1-\negl(\lambda),
\end{align}

\paragraph{Verification Correctness:}
There exists a negligible function $\negl$ such that for any $\secp\in \N$ and $\rho\in\Ms$,
\begin{align}
\Pr\left[
\Vrfy_0(\vk,\cert_0)=\bot
\ \middle |
\begin{array}{ll}
(\pk,\MSK)\lrun \Setup(1^\secp)\\
(\vk,\ct) \lrun \Enc(\pk,\rho)\\
\cert_0 \lrun \Delete_0(\ct)
\end{array}
\right] 
\leq
\negl(\secp),
\end{align}
and
\begin{align}
\Pr\left[
\Vrfy_1(\vk,\sk,\cert_1)=\bot
\ \middle |
\begin{array}{ll}
(\pk,\MSK)\lrun \Setup(1^\secp)\\
(\vk,\ct) \lrun \Enc(\pk,\rho)\\
\sk\lrun\keygen(\MSK)\\
(\cert_1,\rho^*) \lrun \Delete_1(\ct,\sk)
\end{array}
\right] 
\leq
\negl(\secp).
\end{align}
\end{definition}


\begin{definition}[RNC Security for Quantum Message]\label{def:rec_nc_security_qunautm}
Let $\Sigma=(\Setup,\keygen,\Enc,\Dec,\Fake,\Reveal,\Delete_0,\Delete_1,\Vrfy_0,\Vrfy_1)$ be a certified everlasting RNCE scheme for quantum message.
We consider the following security experiment $\expa{\Sigma,\cA}{rec}{nc}(\secp,b)$.
\begin{enumerate}
    \item The challenger runs $(\pk,\MSK)\la\Setup(1^\lambda)$ and sends $\pk$ to $\cA$.
    \item $\cA$ sends $\rho\in\Ms$ to the challenger.
    \item The challenger does the following.
    \begin{itemize}
        \item If $b=0$, the challenger generates $(\vk,\ct)\la\Enc(\pk,\rho)$ and $\sk\la\keygen(\MSK)$, and sends $(\ct,\sk)$ to $\cA_1$.
        \item If $b=1$, the challenger generates $(\vk,\widetilde{\ct},\aux)\la \Fake(\pk,\MSK)$ and $\widetilde{\sk}\la \Reveal(\pk,\MSK,\aux,\rho)$,
        and sends $(\widetilde{\CT},\widetilde{\sk})$ to $\cA_1$.
    \end{itemize}
    \item $\cA$ outputs $b'\in\bit$.
\end{enumerate}
We say that the $\Sigma$ is RNC secure if for any QPT $\cA$, it holds that
\begin{align}
    \advb{\Sigma,\cA}{rec}{nc}(\secp) \seteq \abs{\Pr[\expa{\Sigma,\cA}{rec}{nc}(\secp,0)=1]  - \Pr[\expa{\Sigma,\cA}{rec}{nc}(\secp,1)=1]} \leq \negl(\secp).
\end{align}
\end{definition}

\begin{definition}[Certified Everlasting RNC Security for Quantum Message]\label{def:cert_ever_rec_nc_security_quantum}
Let $\Sigma=(\Setup,\keygen,\Enc,\Dec,\Fake,\Reveal,\Delete_0,\Delete_1,\Vrfy_0,\Vrfy_1)$ be a certified everlasting RNCE scheme for quantum message.
We consider the following security experiment $\expd{\Sigma,\cA}{cert}{ever}{rec}{nc}(\secp,b)$.
\begin{enumerate}
    \item The challenger runs $(\pk,\MSK)\la\Setup(1^\lambda)$ and sends $\pk$ to $\cA_1$.
    \item $\cA_1$ sends $\rho\in\Ms$ to the challenger.
    \item The challenger does the following.
    \begin{itemize}
        \item If $b=0$, the challenger generates $(\vk,\ct)\la\Enc(\pk,m)$ and $\sk\la\keygen(\MSK)$, and sends $\ct$ to $\cA_1$.
        $\cA_1$ is allowed to call a key query at most one time.
        If a key query is called, the challenger generates sends $\sk$ to $\cA_1$.
        \item If $b=1$, the challenger generates $(\vk,\widetilde{\ct},\aux)\la \Fake(\pk,\MSK)$,
        and sends $\widetilde{\CT}$ to $\cA_1$.
        $\cA_1$ is allowed to call a key query at most one time.
        If a key query is called, the challenger generates $\widetilde{\sk}\la\Reveal(\pk,\MSK,\aux,m)$ and sends $\widetilde{\sk}$ to $\cA_1$.
    \end{itemize}
    \item At some point, $\cA_1$ sends $\cert^*$ to the challenger and the internal state to $\cA_2$.
    \item The challenger does the following.
    \begin{itemize}
    \item If a key query is not called, the challenger computes $\Vrfy_0(\vk,\cert^*)$.
    If the output is $\bot$, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    If the output is $\top$, the challenger outputs $\top$ and sends $\MSK$ to $\cA_2$. 
    \item 
    If a key query is called, the challenger computes $\Vrfy_1(\vk,\widetilde{\sk},\cert^*)$.
    If the output is $\bot$, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    If the output is $\top$, the challenger outputs $\top$ and sends $\MSK$ to $\cA_2$. 
    \end{itemize}
    \item $\cA_2$ outputs $b'\in\bit$.
    \item If the challenger outputs $\top$, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
We say that the $\Sigma$ is certified everlasting RNC secure if for any QPT $\cA_1$ and any unbounded $\cA_2$,
it holds that
\begin{align}
    \advd{\Sigma,\cA}{cert}{ever}{rec}{nc}(\secp) \seteq \abs{\Pr[\expd{\Sigma,\cA}{cert}{ever}{rec}{nc}(\secp,0)=1] - \Pr[\expd{\Sigma,\cA}{cert}{ever}{rec}{nc}(\secp,1)=1]} \leq \negl(\secp).
\end{align}
\end{definition}

\subsection{Construction of RNCE for Quantum Message}\label{sec:const_rnce_quantum}
In this section, we present how to construct a certified everlasting RNCE scheme for quantum message from a certified everlasting RNCE scheme for classical message.
\paragraph{Our certified everlasting RNCE scheme for quantum message.}
We construct a certified everlasting RNCE scheme for quantum message 
$\Sigma_{\mathsf{cence}}=(\Setup,\keygen,\Enc,\Dec,\Fake,\Reveal,\Delete_0,\Delete_1,\Vrfy_0,\Vrfy_1)$
from a certified everlasting RNCE scheme for classical message $\Sigma_{\mathsf{classic}}=\mathsf{C}.(\Setup,\keygen,\Enc,\Dec,\Fake,\Reveal,\Delete_0,\Delete_1,\Vrfy_0,\Vrfy_1)$.
\begin{description}
    \item[$\Setup(1^\secp)$:]$ $
    \begin{itemize}
        \item Generate $(\mathsf{c}.\pk,\mathsf{c}.\MSK)\la\mathsf{C}.\Setup(1^\secp)$.
        \item Output $\pk\seteq\mathsf{c}.\pk$ and $\MSK\seteq\mathsf{c}.\MSK$.
    \end{itemize}
    \item[$\keygen(\MSK)$:]$ $
    \begin{itemize}
        \item Generate $\mathsf{c}.\sk\la\mathsf{C}.\keygen(\MSK)$.
        \item Output $\sk\seteq\mathsf{c}.\sk$.
    \end{itemize}
    \item[$\Enc(\pk,\rho)$:]$ $
    \begin{itemize}
        \item Parse $\pk=\mathsf{c}.\pk$.
        \item Generate $a\la\bit^{n}$ and $b\la\bit^{n}$.
        \item Generate $\Psi\seteq X^aZ^b\rho Z^bX^a$.
        \item Compute $(\mathsf{c}.\vk,\mathsf{c}.\ct)\la\mathsf{C}.\Enc(\mathsf{c}.\pk,(a,b))$.
        \item Output $\vk\seteq\mathsf{c}.\vk$ and $\ct\seteq(\Psi,\mathsf{c}.\ct)$.
    \end{itemize}
    \item[$\Dec(\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\mathsf{c}.\sk$ and $\ct=(\Psi,\mathsf{c}.\ct)$.
        \item Compute $(a',b')\la\mathsf{C}.\Dec(\mathsf{c}.\sk,\mathsf{c}.\ct)$.
         \item Output $Z^{b'}X^{a'}\Psi X^{a'}Z^{b'}$.
    \end{itemize}
    \item[$\Fake(\pk,\MSK)$:]$ $
    \begin{itemize}
        \item Parse $\pk=\mathsf{c}.\pk$ and $\MSK=\mathsf{c}.\MSK$.
        \item %Apply $X^{a^*}Z^{b^*}$ to $|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|$ and generate $|\widetilde{a^*b^*}\rangle$.
        Generate $|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|$.
        Let $\Phi_A\seteq \Tr_{B}(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$ and $\Phi_B\seteq \Tr_{A}(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$.
        \item Compute $(\mathsf{c}.\vk,\widetilde{\mathsf{c}.\ct},\mathsf{c}.\aux)\la\mathsf{C}.\Fake(\mathsf{c}.\pk,\mathsf{c}.\MSK)$.
        \item Output $\vk\seteq \mathsf{c}.\vk$, $\widetilde{\ct}\seteq (\Phi_A,\widetilde{\mathsf{c}.\ct})$ and
        $\aux\seteq (\Phi_B,\mathsf{c}.\aux)$.
    \end{itemize}
    \item[$\Reveal(\pk,\MSK,\aux,\rho)$:]$ $
    \begin{itemize}
        \item Parse $\pk=\mathsf{c}.\pk$, $\sk=\mathsf{c}.\sk$
        and $\aux\seteq (\Phi_B,\mathsf{c}.\aux)$.
        \item Measure the $i$-th qubit of $\Phi_B$ and $\rho$ in the Bell basis for all $i\in[n]$.
        Let $(x_i,z_i)$ be the measurement outcome.
        \item Compute $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux, (x,z))$.
        \item Output $\widetilde{\sk}\seteq \widetilde{\mathsf{c}.\sk}$.
    \end{itemize}
    \item[$\Delete_0(\ct):$]$ $
    \begin{itemize}
        \item Parse $\ct=(\Psi,\mathsf{c}.\ct)$.
        \item Compute $\mathsf{c}.\cert_0\la\mathsf{C}.\Delete_0(\mathsf{c}.\ct)$.
        \item Output $\cert_0\seteq\mathsf{c}.\cert_0$.
    \end{itemize}
    \item[$\Delete_1(\ct,\sk):$]$ $
    \begin{itemize}
        \item Parse $\ct=(\Psi,\mathsf{c}.\ct)$ and $\sk=\mathsf{c}.\sk$.
        \item Compute $(\mathsf{c}.\cert_1,(a',b'))\la\mathsf{C}.\Delete_1(\mathsf{c}.\ct,\mathsf{c}.\sk)$.
        \item Output $\cert_1\seteq\mathsf{c}.\cert_1$ and $Z^{b'}X^{a'}\Psi X^{a'}Z^{b'}$.
    \end{itemize}
    \item[$\Vrfy_0(\vk,\cert_0)$:]$ $
    \begin{itemize}
        \item Parse $\vk=\mathsf{c}.\vk$ and $\cert_0=\mathsf{c}.\cert_0$.
        \item Compute $\top/\bot\la\mathsf{C}.\Vrfy_0(\mathsf{c}.\vk,\mathsf{c}.\cert_0)$.
        If all results are $\top$, $\Vrfy_0(\vk,\cert_0)$ outputs $\top$. Otherwise, it outputs $\bot$.
    \end{itemize}
    \item[$\Vrfy_1(\vk,\sk,\cert_1)$:]$ $
    \begin{itemize}
        \item Parse $\vk=\mathsf{c}.\vk$ and $\cert_1=\mathsf{c}.\cert_1$.
        \item Compute $\top/\bot\la\mathsf{C}.\Vrfy_1(\mathsf{c}.\vk,\mathsf{c}.\cert_1)$.
        If all results are $\top$, $\Vrfy_1(\vk,\sk,\cert_1)$ outputs $\top$. Otherwise, it outputs $\bot$.
    \end{itemize}
\end{description}


\paragraph{Correctness:}
Correctness easily follows from correctness of $\Sigma_{\mathsf{classical}}$.


\paragraph{Security:}
We prove the following two theorems.
\begin{theorem}\label{thm:comp_security_rnce_quantum}
If $\Sigma_{\mathsf{classical}}$ is RNC secure, $\Sigma_{\mathsf{cence}}$ is RNC secure.
\end{theorem}
\begin{proof}[Proof of \cref{thm:comp_security_rnce_quantum}]
The proof is very similar to that of \cref{thm:ever_security_rnce_quantum}. Thus, we skip the proof.
\end{proof}

\begin{theorem}\label{thm:ever_security_rnce_quantum}
If $\Sigma_{\mathsf{classical}}$ is certified everlasting RNC secure, $\Sigma_{\mathsf{cence}}$ is certified everlasting RNC secure.
\end{theorem}
\begin{proof}[Proof of \cref{thm:ever_security_rnce_quantum}]
To prove the theorem let us introduce the sequence of hybrids.

\begin{description}
    \item[$\sfhyb{0}{}:$] This is the original experiment.
    \begin{enumerate}
        \item\label{step:prepare_rnce_quantum} The challenger generates $(\mathsf{c}.\pk,\mathsf{c}.\MSK)\la\mathsf{C}.\Setup(1^\secp)$.
        %and initializes the register $AB$ as follows $AB\seteq |\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|$.
        \item The challenger sends $\mathsf{c}.\pk$ to $\cA_1$.
        \item $\cA_1$ chooses $\rho\in\Ms$ and sends $\rho$ to the challenger.
        \item\label{step:enc_rnce_quantum}The challenger generates $a,b\la\bit^n$,
        computes $(\mathsf{c}.\vk,\mathsf{c}.\ct)\la\mathsf{C}.\Enc(\mathsf{c}.\pk,(a,b))$,
        and sends $(Z^bX^a\rho X^aZ^b, \mathsf{c}.\ct)$ to $\cA_1$.
        \item $\cA_1$ is allowed to call a key query at most one time.
        If a key query is called, the challenger generates $\mathsf{c}.\sk\la\mathsf{C}.\keygen(\mathsf{c}.\MSK)$ and sends $\mathsf{c}.\sk$ to $\cA_1$.
        \item $\cA_1$ does the following.
        \begin{itemize}
            \item If a key query is called, $\cA_1$ sends $\mathsf{c}.\cert_1$ to the challenger and sends its internal state to $\cA_2$.
            \item If a key query is not called, $\cA_1$ sends $\mathsf{c}.\cert_0$ to the challenger and its internal state to $\cA_2$.
        \end{itemize}
        \item The challenger does the following.
        \begin{itemize}
            \item If a key query is called, the challenger computes $\mathsf{C}.\Vrfy_1(\mathsf{c}.\vk,\mathsf{c}.\sk,\mathsf{c}.\cert_1)$.
            If the result is $\top$, the challenger outputs $\top$ and sends $\mathsf{c}.\MSK$ to $\cA_2$.
            Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$. 
            \item If a key query is not called, the challenger computes $\mathsf{C}.\Vrfy_0(\mathsf{c}.\vk,\mathsf{c}.\cert_0)$.
            If the result is $\top$, the challenger outputs $\top$ and sends $\mathsf{c}.\MSK$ to $\cA_2$.
            Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$. 
        \end{itemize}
        \item $\cA_2$ outputs $b'$.
        \item If the challenger outputs $\top$, the output of the experiment is $b'$. Otherwise, the output of the experiment is $\bot$.
    \end{enumerate}
    \item[$\sfhyb{1}{}$:]
    This is identical to $\sfhyb{0}{}$ except for the following two points.
    First, the challenger computes
    $(\mathsf{c}.\vk,\widetilde{\mathsf{c}.\ct},\mathsf{c}.\aux)\la\mathsf{C}.\Fake(\mathsf{c}.\pk,\mathsf{c}.\MSK)$ and $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux,(a,b))$.
    %instead of computing $(\mathsf{c}.\vk,\mathsf{c}.\ct)\la\mathsf{C}.\Enc(\mathsf{c}.\pk,(a,b))$.
    Second, the challenger sends $(Z^bX^a\rho X^aZ^b, \widetilde{\mathsf{c}.\ct},\widetilde{\mathsf{c}.\sk})$ to $\cA_1$
    instead of sending $(Z^bX^a\rho X^aZ^b, \mathsf{c}.\ct,\mathsf{c}.\sk)$ to $\cA_1$.
    %\item[$\sfhyb{2}{}$:]This is identical to $\sfhyb{1}{}$ except for the following two points.
    %First, the challenger generates $x,z,a^*,b^*\la\bit^n$ in the step~\ref{step:prepare_rnce_quantum}.
    %Second, in the step~\ref{step:enc_rnce_quantum}, the challenger computes $(\mathsf{c}.\vk_i,\widetilde{\mathsf{c}.\ct_i})\la\mathsf{C}.\Fake(\mathsf{c}.\pk_i,\mathsf{c}.\sk_i,\mathsf{c}.\aux_i)$ for $i\in[2n]$,
    %computes $\widetilde{\mathsf{c}.\sk_i}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk_i,\mathsf{c}.\sk_i,\mathsf{c}.\aux_i,a^*[i]\oplus x[i])$ and 
    %$\widetilde{\mathsf{c}.\sk_{n+i}}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk_{n+i},\mathsf{c}.\sk_{n+i},\mathsf{c}.\aux_{n+i},b^*[i]\oplus z[i])$ for $i\in[n]$
    %and sends $(Z^{b^{*}\oplus z}X^{a^*\oplus x}\rho X^{a^*\oplus x}Z^{b^*\oplus z}, \{\widetilde{\mathsf{c}.\ct_i}\}_{i\in[2n]},\{\widetilde{\mathsf{c}.\sk_i}\}_{i\in[2n]})$ to $\cA_1$.
    \item[$\sfhyb{2}{}$:]
    This is identical to $\sfhyb{1}{}$ except for the following three points.
    First, in the step~\ref{step:enc_rnce_quantum}, the challenger generates $|\widetilde{0^n0^n}\rangle$.
    Let
    $\Phi_A\seteq \Tr_{B}(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$ and $\Phi_B\seteq \Tr_{A}(|\widetilde{0^n0^n}\rangle\langle\widetilde{0^n0^n}|)$.
    Second, in step~\ref{step:enc_rnce_quantum},
    the challenger measures the $i$-th qubit of $\Phi_B$ and $\rho$ in the Bell basis for all $i\in[n]$.
    Let $(x_i,z_i)$ be the measurement outcome.
    Third, the challenger computes $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux,(x,z))$ instead of computing $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux,(a,b))$,
    and sends $(\Phi_A, \widetilde{\mathsf{c}.\ct},\widetilde{\mathsf{c}.\sk})$ to $\cA_1$ instead of sending $(Z^bX^a\rho X^aZ^b, \widetilde{\mathsf{c}.\ct},\widetilde{\mathsf{c}.\sk})$ to $\cA_1$.
\end{description}
It is clear that $\Pr[\expd{\Sigma_{\mathsf{cence}},\cA}{cert}{ever}{rec}{nc}(\secp,0)=1]=\Pr[\sfhyb{0}{}=1]$ and $\Pr[\sfhyb{2}{}=1]=\Pr[\expd{\Sigma_{\mathsf{cence}},\cA}{cert}{ever}{rec}{nc}(\secp,1)=1]$.
Therefore, \cref{thm:ever_security_rnce_quantum} easily follows from the following \cref{prop:hyb_0_hyb_1_rnce_quantum,prop:hyb_1_hyb_2_rnce_quantum} (whose proofs are given later.).
\end{proof}

\begin{proposition}\label{prop:hyb_0_hyb_1_rnce_quantum}
If $\Sigma_{\mathsf{classical}}$ is certified everlasting RNC secure, $\abs{\Pr[\sfhyb{0}{}=1]-\Pr[\sfhyb{1}{}=1]}\leq\negl(\lambda)$.
\end{proposition}


\begin{proposition}\label{prop:hyb_1_hyb_2_rnce_quantum}
$\Pr[\sfhyb{1}{}=1]=\Pr[\sfhyb{2}{}=1]$.
\end{proposition}



\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_rnce_quantum}]
We assume that $\abs{\Pr[\sfhyb{0}{}=1]-\Pr[\sfhyb{1}{}=1]}$ is non-negligible, and construct an adversary $\cB$ that breaks the certified everlasting RNC security of $\Sigma_{\mathsf{classical}}$. We describe how $\cB$ works below.

\begin{enumerate}
    \item $\cB$ receives $\mathsf{c}.\pk$ from the challenger of $\expd{\Sigma_{\mathsf{classical}},\cA}{cert}{ever}{rec}{nc}(\secp,b')$ and sends $\mathsf{c}.\pk$ to $\cA_1$.
    \item $\cB$ receives $\rho$ from $\cA_1$.
    \item $\cB$ generates $a,b\la\bit^n$ and sends $(a,b)$ to the challenger.
    \item $\cB$ receives $\mathsf{c}.\ct^*$ from the challenger.
    \item $\cB$ sends $(X^aZ^b\rho Z^bX^a,\mathsf{c}.\ct^*)$ to $\cA_1$.
    \item $\cA_1$ is allowed to call a key query.
    If a key query is called, $\cB$ sends a key query to the challenger and receives $\mathsf{c}.\sk$. 
    \item If a key query is called, $\cA_1$ sends $\mathsf{c}.\cert^*$ to $\cB$ and sends its internal state to $\cA_2$.
%\item The challenger does the following.
        %\begin{itemize}
            %\item If a key query is called, $\cB$ sends $\mathsf{c}.\cert_1$ to the challenger, and receives $\mathsf{c}.\MSK$ or $\bot$.
            %If $\cB$ receives $\bot$, it outputs $\bot$ and aborts.
            %\item  If a key query is called, $\cB$ sends $\mathsf{c}.\cert_1$ to the challenger, and receives $\mathsf{c}.\MSK$ or $\bot$.
            %If $\cB$ receives $\bot$, it outputs $\bot$ and aborts.
        %\end{itemize}
    \item $\cB$ sends $\mathsf{c}.\cert^*$ to the challenger, and receives $\mathsf{c}.\MSK$ or $\bot$ from the challenger.
    If $\cB$ receives $\bot$ from the challenger, it outputs $\bot$ and aborts.
    \item $\cB$ sends $\mathsf{c}.\MSK$ to $\cA_2$.
    \item $\cA_2$ outputs $b''$.
    \item $\cB$ outputs $b''$.
\end{enumerate}
\end{proof}
It is clear that $\Pr[1\la\cB|b'=0]=\Pr[\sfhyb{0}{}=1]$ and $\Pr[1\la\cB|b'=1]=\Pr[\sfhyb{1}{}=1]$.
By assumption, $\abs{\Pr[\sfhyb{0}{}=1]-\Pr[\sfhyb{1}{}=1]}$ is non-negligible, and therefore $\abs{\Pr[1\la\cB|b'=0]-\Pr[1\la\cB|b'=1]}$ is non-negligible, which contradicts the certified everlasting RNC security of $\Sigma_{\mathsf{classical}}$.

\begin{proof}[Proof of \cref{prop:hyb_1_hyb_2_rnce_quantum}]
We clarify the difference between $\sfhyb{1}{}$ and $\sfhyb{2}{}$.
First, in $\sfhyb{2}{}$, the challenger runs $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux,(x,z))$ instead of running $\widetilde{\mathsf{c}.\sk}\la\mathsf{C}.\Reveal(\mathsf{c}.\pk,\mathsf{c}.\MSK,\mathsf{c}.\aux,(a,b))$ as in $\sfhyb{1}{}$.
Second, in $\sfhyb{2}{}$, the challenger sends $\Phi_A$ to $\cA_1$ instead of sending $Z^{b}X^{a}\rho X^{a}Z^{b}$ to $\cA_1$ as in $\sfhyb{1}{}$.
Hence,
it is sufficient to prove that $x$ and $z$ are uniformly randomly distributed and
$\Phi_A$ is identical to $Z^{z}X^{x}\rho X^{x}Z^{z}$.
These two things are obvious from \cref{lem:quantum_teleportation}.

\end{proof}













==> Sec_FE_Poly.tex <==
% !TEX root = main.tex
% !TEX spellcheck = en-US


\color{red}
\subsection{Construction of $q$-Bounded Certified Everlasting Functional Encryption for Polynomial circuits}\label{sec:const_multi_fe}
In this section, we present how to construct a $q$-bounded certified everlasting functional encryption scheme for NC1 circuits from single-key certified everlasting functional encryption.
Our construction uses BGW semi-honest MPC protocol without degree reduction~\cite{}.

We construct a $q$-bounded certified everlasting FE scheme for a circuit family $\mathcal{C}\seteq NC1$.
In particular, we consider polynomial representation of circuits $C$ in the family.
The input message space $\Ms=\mathbb{F}^{\ell}$ is an $\ell$ tuple of field elements, and for every circuits $C\in\mathcal{C}$, $C(\cdot)$ is an $\ell$-variate polynomial over $\mathbb{F}$ of total degree at most $D$.



\paragraph{Our bounded collusion certified everlasting FE scheme for NC1 circuits.}
Let $\mathcal{C}\seteq NC1$ be a circuit family with circuits of degree $D=D(\lambda)$ in its input, and let $q=q(\lambda)$ be some polynomial of $\lambda$. Our scheme is associated wit additional parameters $S=S(\lambda)$, $N=N(\lambda)$, $t=t(\lambda)$ and $v=v(\lambda)$.
In our construction, we set these parameters as follows:
\begin{align}
    t(\lambda)=\Theta(q^2\lambda), N(\lambda)=\Theta(D^2q^2t), v(\lambda)=\Theta(\lambda), S(\lambda)=\Theta(vq^2)
\end{align}

We start by defining a new family $\mathcal{G}$ as follows:
\begin{align}
G_{C,\Delta}(x,Z_1,Z_2,\cdots,Z_S)\seteq C(x)+\sum_{i\in\Delta}Z_i    
\end{align}
where $\Delta\subseteq[S]$ and $Z_1,\cdots,Z_S\in\mathbb{F}$.

We construct a $q$-bounded certified everlasting FE scheme for NC1 circuits  $\Sigma_{\mathsf{cefe}}=(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$
from a single-key certified everlasting FE scheme $\Sigma_{\mathsf{one}}=\mathsf{ONE}.(\Setup,\keygen,\Enc,\Dec,\Delete,\Vrfy)$.

\begin{description}
\item[$\Setup(1^\lambda)$:]$ $
\begin{itemize}
    \item For $i\in[N]$, generate $(\mathsf{one}.\MPK_i,\mathsf{one}.\MSK_i)\la\mathsf{ONE}.\Setup(1^\secp)$.
    \item Output $\MPK\seteq\{\mathsf{one}.\MPK_i\}_{i\in[N]}$ and $\MSK\seteq \{\mathsf{one}.\MSK_i\}_{i\in[N]}$.
\end{itemize}
\item[$\keygen(\MSK,C)$:]$ $
\begin{itemize}
    \item Parse $\MSK= \{\mathsf{one}.\MSK_i\}_{i\in[N]}$.
    \item Chooses a uniformly random set $\Gamma\subseteq[N]$ of size $tD+1$.
    \item Chooses a uniformly random set $\Delta\subseteq[S]$ of size $v$.
    \item For $i\in\Gamma$, compute $\mathsf{one}.\sk_{C,\Delta,i}\la\mathsf{ONE}.\keygen(\one.\MSK_i,G_{C,\Delta})$.
    \item Output $\sk_{C}\seteq (\Gamma,\Delta,\{\one.\sk_{C,\Delta,i}\}_{i\in\Gamma})$.
\end{itemize}
\item[$\Enc(\MPK,x)$:]$ $
\begin{itemize}
    \item Parse $\MPK=\{\mathsf{one}.\MPK_i\}_{i\in[N]}$.
    \item For $i\in[\ell]$, pick a random degree $t$ polynomial $\mu_i(\cdot)$ whose constant term is $x[i]$.
    \item For $i\in[S]$, pick a random degree $Dt$ polynomial $\xi_i(\cdot)$ whose constant term is $0$.
    \item For $i\in[N]$, compute $(\one.\vk_i,\one.\ct_i)\la\ONE.\Enc(\one.\MPK_i,(\mu_1(i),\cdots,\mu_{\ell}(i),\xi_1(i),\cdots,\xi_S(i) ))$.
    \item Output $\vk=\{\one.\vk_i\}_{i\in[N]}$ and $\ct\seteq\{\one.\ct_i\}_{i\in[N]}$.
    \end{itemize}
\item[$\Dec(\sk_C,\ct)$:]$ $
\begin{itemize}
    \item Parse $\sk_{C}= (\Gamma,\Delta,\{\one.\sk_{C,\Delta,i}\}_{i\in\Gamma})$ and $\ct=\{\one.\ct_i\}_{i\in[N]}$.
    \item For $i\in \Gamma$, compute $(\eta(i),\widehat{\one.\ct}_i)\la\ONE.\Dec(\one.\sk_{C,\Delta,i},\one.\ct_i)$.
    Let $\widehat{\one.\ct}_i\seteq \one.\ct_i$ for $i\in[N]\backslash\Gamma$.
    \item Output $\eta(0)$ and $\widehat{\one.\ct}\seteq \{\widehat{\one.\ct}_i\}_{i\in[N]}$.
\end{itemize}
\item[$\Delete(\ct)$:]$ $
\begin{itemize}
    \item Parse $\ct=\{\one.\ct_i\}_{i\in[N]} $.
    \item For $i\in[N]$, compute $\one.\cert_i\la\ONE.\Delete(\one.\ct_i)$.
    \item Output $\cert\seteq \{\one.\cert_i\}_{i\in[N]}$.
\end{itemize}
\item[$\Vrfy(\vk,\cert)$:]$ $
\begin{itemize}
    \item Parse $\vk=\{\one.\vk_i\}_{i\in[N]}$ and $\cert= \{\one.\cert_i\}_{i\in[N]}$.
    \item For $i\in[N]$, compute $\top\backslash\bot\la\ONE.\Vrfy(\one.\vk_i,\one.\cert_i)$.
    If all results are $\top$, output $\top$. Otherwise, output $\bot$.
\end{itemize}
\end{description}

\paragraph{Correctness:}
By decryption correctness of the $\Sigma_{\one}$, for all $i\in\Gamma$ we have 
\begin{align}
\eta(i)&=G_{C,\Delta} (\mu_1(i),\cdots,\mu_\ell(i),\xi_1(i),\cdots,\xi_S(i))\\
&=C(\mu_1(i),\cdots,\mu_\ell(i))+\Sigma_{a\in\Delta}\xi_a(i).
\end{align}
Since $|\Gamma|\geq Dt+1$, this means that $\eta$ is equal to the degree $Dt$ polynomial 
\begin{align}
    \eta(\cdot)=C(\mu_1(\cdot),\cdots,\mu_\ell(\cdot) )+\Sigma_{a\in\Delta}\xi_a(\cdot)
\end{align}
Hence $\eta(0)=C(x_1,\cdots,x_\ell)=C(x)$, which means that our construction satisfies decryption correctness.

Verification correctness easily follows from verification correctness of $\Sigma_{\one}$.
Rewind correctness easily follows from rewind correctness of $\Sigma_{\one}$.



\paragraph{Security:}
We prove the following theorems.
\begin{theorem}\label{thm:compt_bounded_fe}
If $\Sigma_{\one}$ satisfies the single-key adaptive security, $\Sigma_{\mathsf{cefe}}$ satisfies the $q$-bounded adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:compt_bounded_fe}]
The proof is very similar to that of \cref{thm:ever_bounded_fe}. Therefore, we skip the proof.
\end{proof}


\begin{theorem}\label{thm:ever_bounded_fe}
If $\Sigma_{\one}$ satisfies the single-key certified everlasting adaptive security,
$\Sigma_{\mathsf{cefe}}$ the $q$-bounded certified everlasting adaptive security.
\end{theorem}
\begin{proof}[Proof of \cref{thm:ever_bounded_fe}]
Let us denote the simulating algorithm of $\Sigma_{\one}$ as $\ONE.\Sim=\ONE.(\Sim_1,\Sim_2,\Sim_3)$.
Let us describe how the simulator $\Sim=(\Sim_1,\Sim_2,\Sim_3)$ works below.
\begin{description}
\item[$\Sim_1(\MPK,\mathcal{V},1^{|m|})$:] Let $q^*$ be the number of times that $\cA_1$ has made key queries before it sends a challenge query. 
\begin{enumerate}
    \item Parse $\MPK\seteq \{\one.\MPK_{i}\}_{i\in[N]}$ and $\mathcal{V}\seteq \{C_j,C_j(x),(\Gamma_j,\Delta_j,\{\one.\sk_{C_j,\Delta_j,i}\}_{i\in[\Gamma_j]})\}_{j\in[q^*]}$.
    \item Generate a uniformly random set $\Gamma_i\subseteq[N]$ of size $tD+1$ and a uniformly random set $\Delta_i\subseteq[S]$ of size $v$ for all $i\in\{q^*+1,\cdots, q\}$.
    Let $\Delta_0\seteq \emptyset$. Let $\mathcal{L}\seteq \bigcup_{i\neq i'}(\Gamma_i\cap \Gamma_{i'})$.
    $\Sim_1$ aborts if $\left|\mathcal{L}\right|> t$ or
    there exists some $i\in[q]$ such that $\Delta_i\backslash(\bigcup_{j\neq i}\Delta_j)=\emptyset$.
    \item $\Sim_1$ uniformly and independently samples $\ell$ random degree $t$ polynomials $\mu_1,\cdots, \mu_\ell$ whose constant terms are all $0$. 
    \item $\Sim_1$ samples the polynomials $\xi_1,\cdots, \xi_S$ as follows for $j\in[q]$:
    \begin{itemize}
        \item fix $a^*\in\Delta_j\backslash(\Delta_0\cup\cdots\cup\Delta_{j-1})$;
        \item for all $a\in(\Delta_j\backslash(\Delta_0\cup\cdots\cup \Delta_{j-1}))\backslash\{a^*\}$, set $\xi_a$ to be a uniformly random degree $Dt$ polynomial whose constant term is $0$;
        \item if $j\leq q^*$, pick a random degree $Dt$ polynomial $\eta_j(\cdot)$ whose constant term is $C_j(x)$; if $j>q^*$, pick random values for $\eta_j(i)$ for all $i\in\mathcal{L}$;
        \item the evaluation of $\xi_{a^*}$ on the points in $\mathcal{L}$ is defined by the relation:
        \begin{align}
            \eta_j(\cdot)=C_j(\mu_1(\cdot),\cdots, \mu_\ell(\cdot))+\sum_{a\in\Delta_j}\xi_a(\cdot).
        \end{align}
        \item Finally, for all $a\notin (\Delta_1\cup\cdots \cup \Delta_q)$, set $\xi_a$ to be a uniformly random degree $Dt$ polynomial whose constant term is $0$.
    \end{itemize}
    \item For each $i\in\mathcal{L}$, $\Sim_1$ computes 
    \begin{align}
        (\one.\vk_i,\one.\ct_i)\la\ONE.\Enc(\one.\MPK_i,(\mu_1(i),\cdots,\mu_\ell(i),\xi_1(i),\cdots, \xi_S(i) )).
    \end{align}
    \item For each $i\notin \mathcal{L}$, $\Sim_1$ does the following:
    \begin{itemize}
        \item If $i\in \Gamma_j$ for some $j\in[q^*]$
        \footnote
        { Note that $j$ is unique since $i\notin \mathcal{L}$ .
        },
        computes
        \begin{align}
        (\one.\ct_i,\one.\state_i)\la\ONE.\Sim_1(\one.\MPK_i,(G_{C_j,\Delta_j,i},\eta_j(i),\one.\sk_{C_j,\Delta_j,i}),1^{|m|}).
        \end{align}
        \item If $i\notin\Gamma_j$ for all $j\in[q^*]$, 
        computes 
        \begin{align}
            (\one.\ct_i,\one.\state_i)\la\ONE.\Sim_1(\one.\MPK_i,\emptyset,1^{|m|}).
        \end{align}
    \end{itemize}
    \item Output $\ct\seteq \{\one.\ct_i\}_{i\in[N]}$ and $\state\seteq (\{\Gamma_i\}_{i\in[q]},\{\Delta_i\}_{i\in[q]},\{\eta_j(i)\}_{j\in\{q^*+1,\cdots,q\},i\in\mathcal{L}},\{\one.\state_i\}_{i\in[N]\backslash\mathcal{L}},\{\one.\vk_i\}_{i\in\mathcal{L}})$.
\end{enumerate}
\item[$\Sim_2(\MSK,C_j,C_j(x),\state)$:]The simulator simulates the $j$-th key query for $j>q^*$.
\begin{enumerate}
    \item Parse $\MSK\seteq\{\one.\MSK_i\}_{i\in[N]}$ and $\state_{j-1} \seteq  (\{\Gamma_i\}_{i\in[q]},\{\Delta_i\}_{i\in[q]},\{\eta_s(i)\}_{s\in\{q^*+1,\cdots,q\},i\in\mathcal{L}},\{\one.\state_i\}_{i\in[N]\backslash\mathcal{L}},\{\one.\vk_i\}_{i\in\mathcal{L}})$.
    \item For each $i\in\Gamma_j\cap \mathcal{L}$, generate $\one.\sk_{C_j,\Delta_j,i}\la\ONE.\keygen(\one.\MSK_i,G_{C_j,\Delta_j})$.
    \item For each $i\in\Gamma_j\backslash \mathcal{L}$, 
    generate a random degree $Dt$ polynomial $\eta_j(\cdot)$ whose constant term is $C_j(x)$ and subject to the constraints on the values in $\mathcal{L}$ chosen earlier,
    and generate 
    \begin{align}
    (\one.\sk_{C_j,\Delta_j,i},\one.\state_i^*)\la\ONE.\Sim_2(\one.\MSK_i,\eta_j(i),G_{C_j,\Delta_j},\one.\state_i).
    \end{align}
    For simplicity, let us denote $\one.\state_i^*$ as $\one.\state_i$ for $i\in\Gamma_j\backslash \mathcal{L}$.
    \item Output $\sk_{C_j}\seteq(\Gamma_j,\Delta_j,\{\one.\sk_{C_j,\Delta_j,i}\}_{i\in\Gamma_j})$ and
    $\state_j\seteq (\{\Gamma_i\}_{i\in[q]},\{\Delta_i\}_{i\in[q]},\{\eta_j(i)\}_{j\in\{q^*+1,\cdots,q\},i\in\mathcal{L}},\\ \{\one.\state_i\}_{i\in[N]\backslash\mathcal{L}},\{\one.\vk_i\}_{i\in\mathcal{L}})$.
\end{enumerate}
\item[$\Sim_3(\state^*)$:]The simulator simulates a verification key.
\begin{enumerate}
    \item Parse $\state^*\seteq (\{\Gamma_i\}_{i\in[q]},\{\Delta_i\}_{i\in[q]},\{\eta_j(i)\}_{j\in\{q^*+1,\cdots,q\},i\in\mathcal{L}}, \{\one.\state_i\}_{i\in[N]\backslash\mathcal{L}},\{\one.\vk_i\}_{i\in\mathcal{L}})$.
    \item For each $i\in [N]\backslash\mathcal{L}$, computes $\one.\vk_i\la\ONE.\Sim_3(\one.\state_i)$.
    \item Output $\vk\seteq\{\one.\vk_i\}_{i\in[N]}$.
\end{enumerate}
Let us define the sequence of hybrids as follows.

\item [$\sfhyb{0}{}$:] This is identical to $\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, 0)$.
\begin{enumerate}
    \item\label{step:keygen_bounded_fe} The challenger generates $(\one.\MPK_i,\one.\MSK_i)\la\ONE.\Setup(1^\secp)$ for $i\in[N]$.
    \item $\cA_1$ is allowed to call a key query at most $q$ times.
    For the $j$-th key query, the challenger receives an function $C_{j}$ from $\cA_1$, generates a uniformly random set $\Gamma_{j}\in[N]$ of size $tD+1$ and $\Delta_{j}\in [S]$ of size $v$.
    For $i\in \Gamma_{j}$, the challenger generates $\mathsf{one}.\sk_{C_{j},\Delta_{j},i}\la\mathsf{ONE}.\keygen(\one.\MSK_i,G_{C_{j},\Delta_{j}})$, and sends $(\Gamma_{j},\Delta_{j},\{\one.\sk_{C_{j},\Delta_{j},i}\}_{i\in\Gamma_{j}})$ to $\cA_1$.
    Let $q^*$ be the number of times that $\cA_1$ has called key queries in this step.
    \item $\cA_1$ chooses $x\in\Ms$ and sends $x$ to the challenger.
    \item\label{step:enc_bounded_fe} The challenger generates a random degree $t$ polynomial $\mu_i(\cdot)$ whose constant term is $x[i]$ for $i\in[\ell]$
    and a random degree $Dt$ polynomial $\xi_i(\cdot)$ whose constant term is $0$.
    For $i\in[N]$, the challenger computes $(\one.\vk_i,\one.\ct_i)\la\ONE.\Enc(\one.\MPK_i,(\mu_1(i),\cdots,\mu_{\ell}(i),\xi_1(i),\cdots,\xi_S(i)))$,
    and sends $\{\one.\ct_i\}_{i\in[N]}$ to $\cA_1$.
    \item\label{step:key_bounded_fe_2} $\cA_1$ is allowed to call a key query at most $q-q^*$ times.
    For the $j$-th key query, the challenger receives an function $C_{j}$ from $\cA_1$, generates a uniformly random set $\Gamma_{j}\in[N]$ of size $tD+1$ and $\Delta_{j}\in [S]$ of size $v$.
    For $i\in \Gamma_{j}$, the challenger generates $\mathsf{one}.\sk_{C_{j},\Delta_{j},i}\la\mathsf{ONE}.\keygen(\one.\MSK_i,G_{C_{j},\Delta_{j}})$, and sends $(\Gamma_{j},\Delta_{j},\{\one.\sk_{C_{j},\Delta_{j},i}\}_{i\in\Gamma_{j}})$ to $\cA_1$.
    %Let $q'$ be the number of times that $\cA_1$ has called key queries in this step.
    \item $\cA_1$ sends $\{\one.\cert_i\}_{i\in[N]}$ to the challenger and its internal state to $\cA_2$.
    \item If $\top\la \ONE.\Vrfy(\one.\vk_i,\one.\cert_i)$ for all $i\in[N]$, the challenger outputs $\top$ and sends $\{\one.\MSK_i\}_{i\in[N]}$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b$.
    \item The experiment outputs $b$ if the challenger outputs $\top$.
    Otherwise, the experiment outputs $\bot$.
\end{enumerate}
\item[$\sfhyb{1}{}$:] This is identical to $\sfhyb{0}{}$ except for the following three points.
First, the challenger generates uniformly random set $\Gamma_i\in[N]$ of size $tD+1$ and $\Delta_{i}\in [S]$ of size $v$ for $i\in\{q^*+1,\cdots,q\}$ in step \ref{step:enc_bounded_fe} instead of generating them when a key query is called.
Second, if $\left|\mathcal{L}\right|> t$, the challenger aborts and the experiment outputs $\bot$.
Third, if there exists some $i\in[q]$ such that $\Delta_i\backslash(\bigcup_{j\neq i}\Delta_j)=\emptyset$, the challenger aborts and the experiment outputs $\bot$.

\item[$\sfhyb{2}{}$:]This is identical to $\sfhyb{1}{}$ except that the challenger samples $\xi_1,\cdots,\xi_S, \eta_1,\cdots,\eta_q$ as in the simulator $\Sim_1$ described above.

\item[$\sfhyb{3}{}$:]
This is identical to $\sfhyb{2}{}$ except that the challenger generates $\{\one.\ct_i\}_{i\in[N]\backslash\{\mathcal{L}\}}$,
$\{\one.\sk_{C_j,\Delta_j,i}\}_{i\in\Gamma_j}$ for $j\in\{q^*+1,\cdots ,q'\}$,
and $\vk\seteq\{\one.\vk_i\}_{i\in[N]\backslash\{\mathcal{L}\}}$ as in the simulator $\Sim=(\Sim_1,\Sim_2,\Sim_3)$ described above,
where $q'$ is the number of key queries that the adversary makes in total.

\item[$\sfhyb{4}{}$:]
This is identical to $\sfhyb{3}{}$ except that the challenger generates $\mu_1,\cdots, \mu_\ell$ as in the simulator $\Sim_1$ described above.
\end{description}

From the definition of $\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp, b)$ and $\Sim=(\Sim_1,\Sim_2,\Sim_3)$,
it is clear that $\Pr[\sfhyb{0}{}=1]=\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,0)=1]$ and
$\Pr[\sfhyb{4}{}=1]=\Pr[\expc{\Sigma_{\mathsf{cefe}},\cA}{cert}{ever}{adapt}(\secp,1)=1]$.
Therefore, \cref{thm:ever_bounded_fe} easily follows from \cref{prop:hyb_0_hyb_1_bounded_fe,prop:hyb_1_hyb_2_bounded_fe,prop:hyb_2_hyb_3_bounded_fe,prop:hyb_3_hyb_4_bounded_fe}.
\end{proof}

\begin{proposition}\label{prop:hyb_0_hyb_1_bounded_fe}
\begin{align}
    \abs{\Pr[\sfhyb{0}{}=1]-\Pr[\sfhyb{1}{}=1]}\leq \negl(\lambda).
\end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_hyb_2_bounded_fe}
\begin{align}
    \Pr[\sfhyb{1}{}=1]=\Pr[\sfhyb{2}{}=1].
\end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_2_hyb_3_bounded_fe}
If $\Sigma_{\one}$ is single-key certified everlasting adaptive secure,
\begin{align}
    \abs{\Pr[\sfhyb{2}{}=1]-\Pr[\sfhyb{3}{}=1]}\leq \negl(\lambda).
\end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_3_hyb_4_bounded_fe}
\begin{align}
    \Pr[\sfhyb{3}{}=1]=\Pr[\sfhyb{4}{}=1].
\end{align}
\end{proposition}

\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_bounded_fe}]
Let $\sfhyb{0}{'}$ be the experiment identical to $\sfhyb{0}{}$ except that the challenger generates a set $\Gamma_i\in[N]$ and $\Delta_{i}\in [S]$ for $i\in\{q^*+1,\cdots ,q\}$
in step~\ref{step:enc_bounded_fe}.
Generating uniformly random set $\Gamma_i\in[N]$ of size $tD+1$ and $\Delta_{i}\in [S]$ of size $v$ for $i\in\{q^*+1,\cdots,q\}$ commutes with all operations in step~\ref{step:enc_bounded_fe}.
Hence, it holds that $\Pr[\sfhyb{0}{}=1]=\Pr[\sfhyb{0}{'}=1]$. 

Let $\sfhyb{0}{*}$ be the experiment identical to $\sfhyb{0}{'}$ except that the challenger aborts and the experiment outputs $\bot$ if $|\mathcal{L}|>t$.
It is clear that $\Pr[\sfhyb{0}{'}=1\wedge (|\mathcal{L}|\leq t)]=\Pr[\sfhyb{0}{*}=1\wedge (|\mathcal{L}|\leq t)]$.
Hence, it holds that
\begin{align}
    \abs{\Pr[\sfhyb{0}{'}=1]-\Pr[\sfhyb{0}{*}=1]}\leq \Pr[|\mathcal{L}|>t]
\end{align}
from \cref{lem:defference}.

Let $\mathsf{Collide}$ be the event that
there exists some $i\in[q]$ such that $\Delta_i\backslash(\bigcup_{j\neq i}\Delta_j)=\emptyset$.
By definition, $\sfhyb{0}{*}$ is identical to $\sfhyb{1}{}$ when $\mathsf{Collide}$ does not occur.
Hence, it is clear that $\Pr[\sfhyb{0}{*}=1\wedge\overline{\mathsf{Collide}}]=\Pr[\sfhyb{1}{}=1\wedge \overline{\mathsf{Collide}}]$.
Therefore, it holds that 
\begin{align}
    \abs{\Pr[\sfhyb{0}{*}=1]-\Pr[\sfhyb{1}{}=1]}\leq \Pr[\mathsf{Collide}]
\end{align}
from \cref{lem:defference}.

From the all discussion above, we have 
\begin{align}
    \abs{\Pr[\sfhyb{0}{}=1]-\Pr[\sfhyb{1}{}=1]}\leq \Pr[|\mathcal{L}|>t]+\Pr[\mathsf{Collide}].
\end{align}
A simple probabilistic argument shows that 
$\Pr[|\mathcal{L}|>t]\leq 2^{-\Omega(\lambda)}$
and $\Pr[\mathsf{Collide}]\leq 2^{-\Omega(\lambda)}$, which completes the proof
\footnote{The formal proof of $\Pr[|\mathcal{L}|>t]\leq 2^{-\Omega(\lambda)}$ is given in \cref{sec:prob_1} and that of $\Pr[\mathsf{Collide}]\leq q2^{-\Omega(\lambda)}$ is given in \cref{sec:prob_2}.}.


\end{proof}

\begin{proof}[Proof of \cref{prop:hyb_1_hyb_2_bounded_fe}]
In the encryption in $\sfhyb{1}{}$, $\xi_{a^*}$ is chosen at random and $\eta_j(\cdot)$ is defined by the relation.
$\Sim$ essentially chooses $\eta_j(\cdot)$ at random which defines $\xi_{a^*}$.
It is easy to see that reversing the order of how the polynomials chosen produces the same distribution.
\end{proof}

\begin{proof}[Proof of \cref{prop:hyb_2_hyb_3_bounded_fe}]
To prove the proposition, let us define the sequence of hybrids $\sfhyb{2}{s}$ for each $s\in[N]$ as follows.
\begin{description}
\item[$\sfhyb{2}{s}$:] This is identical to $\sfhyb{2}{}$ except for the following points.
First, the challenger generates $\{\one.\ct_i\}_{i\in[s]\backslash\mathcal{L}}$ as in the simulator $\Sim_1$.
Second, the challenger generates $\{\one.\sk_{C_j,\Delta_j,i}\}_{i\in\Gamma_j\cap[s]}$ for $j\in\{q^*+1,\cdots ,q'\}$ as in the simulator $\Sim_2$,
where $q'$ is the number of key queries that the adversary makes in total.
Third, the challenger generates $\{\one.\vk_i\}_{i\in[s]\backslash\mathcal{L}}$ as in the simulator $\Sim_3$.
\end{description}
Let us denote $\sfhyb{2}{}$ as $\sfhyb{2}{0}$.
It is clear that $\Pr[\sfhyb{2}{N}=1]=\Pr[\sfhyb{3}{}=1]$.
Furthermore, we can show that
\begin{align}
    \abs{\Pr[\sfhyb{2}{s-1}=1]-\Pr[\sfhyb{2}{s}=1]}\leq \negl(\lambda)
\end{align}
for $s\in[N]$. (Its proof is given later.)
From these facts, we obtain \cref{prop:hyb_2_hyb_3_bounded_fe}.


Let us show the remaining one.
In the case $s\in\mathcal{L}$, it is clear that $\sfhyb{2}{s-1}$ is identical to $\sfhyb{2}{s}$.
Hence, we consider the case $s\notin\mathcal{L}$.
To show the inequality above, let us assume that $\abs{\Pr[\sfhyb{2}{s-1}=1]-\Pr[\sfhyb{2}{s}=1]}$ is non-negligible.
Then, we can construct an adversary $\cB$ that can break the single-key certified everlasting adaptive security of $\Sigma_{\one}$ as follows.

\begin{enumerate}
    \item $\cB$ receives $\one.\MPK$ from the challenger of $\expc{\Sigma_{\mathsf{one}},\cA}{cert}{ever}{adapt}(\secp,b)$.
    $\cB$ sets $\one.\MPK_s\seteq \one.\MPK$.
    \item $\cB$ generates $(\one.\MPK_i,\one.\MSK_i)\la\ONE.\Setup(1^\secp)$ for all $i\in[N]\backslash s$, and sends $\{\one.\MPK_i\}_{i\in[N]}$ to $\cA_1$.
    \item $\cA_1$ is allowed to call a key query at most $q$ times.
    For the $j$-th key query, $\cB$ receives an function $C_{j}$ from $\cA_1$, generates a uniformly random set $\Gamma_{j}\in[N]$ of size $tD+1$ and $\Delta_{j}\in [S]$ of size $v$.
    For $i\in \Gamma_{j}\backslash s$, $\cB$ generates $\mathsf{one}.\sk_{C_{j},\Delta_{j},i}\la\mathsf{ONE}.\keygen(\one.\MSK_i,G_{C_{j},\Delta_{j}})$.
    If $s\in\Gamma_j$, $\cB$ sends $G_{C_j,\Delta_j}$ to the challenger, and receives $\one.\sk_{C_j,\Delta_j,s}$ from the challenger
    and sends $(\Gamma_{j},\Delta_{j},\{\one.\sk_{C_{j},\Delta_{j},i}\}_{i\in\Gamma_{j}})$ to $\cA_1$.
    Let $q^*$ be the number of times that $\cA_1$ has called key queries in this step.
    \item $\cA_1$ chooses $x\in\Ms$ and sends $x$ to $\cB$.
    \item\label{step:enc_bounded_fe_hyb_2} $\cB$ generates uniformly random set $\Gamma_i\in[N]$ of size $tD+1$ and $\Delta_{i}\in [S]$ of size $v$ for $i\in\{q^*+1,\cdots,q\}$.
    $\cB$ generates a random degree $t$ polynomial $\mu_i(\cdot)$ whose constant term is $x[i]$ for $i\in[\ell]$, and $\xi_1,\cdots,\xi_S, \eta_1,\cdots,\eta_q$ as in the simulator $\Sim_1$.
    For $i\in[s-1]\backslash\mathcal{L}$, $\cB$ generates $\one.\ct_i$ as in the simulator $\Sim_1$.
    For $i\in\{s+1,\cdots N\}\cup \mathcal{L}$, $\cB$ generates $(\one.\vk_i,\one.\ct_i)\la \ONE.\Enc(\one.\MPK_i, (\mu_1(i),\cdots,\mu_\ell(i),\xi_1(i),\cdots, \xi_S(i)))$.
    $\cB$ sends $\mu_1(s),\cdots,\mu_\ell(s),\xi_1(s),\cdots ,\xi_S(s)$ to the challenger, and receives $\one.\ct_s$ from the challenger. 
    $\cB$ sends $\{\one.\ct_i\}_{i\in[N]}$ to $\cA_1$.
    \item $\cA_1$ is allowed to call a key query at most $q-q^*$ times.
    For the $j$-th key query, $\cB$ receives an function $C_j$ from $\cA_1$.
    For $i\in\Gamma_j\backslash [s]$, $\cB$ generates $\one.\sk_{C_j,\Delta_j,i}\la\ONE.\keygen(\one.\MSK_i,G_{C_j,\Delta_j})$.
    For $i\in \Gamma_j\wedge[s-1]$, $\cB$ generates $\one.\sk_{C_j,\Delta_j,i}$ as in the simulator $\Sim_2$.
    If $s\in\Gamma_j$, $\cB$ sends $G_{C_j,\Delta_j}$ to the challenger, and receives $\one.\sk_{C_j,\Delta_j,s}$ from the challenger.
    $\cB$ sends $(\Gamma_j,\Delta_j,\{\one.\sk_{C_j,\Delta_j,i}\}_{i\in \Gamma_j})$ to $\cA_1$.
    \item For $i\in[s-1]\backslash\mathcal{L}$, $\cB$ generates $\one.\vk_i$ as in the simulator $\Sim_3$
    \footnote{
    For $i\in\{s+1,\cdots N\}\cup \mathcal{L}$, $\cB$ generated $\one.\vk_i$ in step~\ref{step:enc_bounded_fe_hyb_2}.
    }.
    \item $\cA_1$ sends $\{\one.\cert_i\}_{i\in[N]}$ to $\cB$ and its internal state to $\cA_2$.
    \item $\cB$ sends $\one.\cert_s$ to the challenger, and receives $\one.\MSK_s$ or $\bot$ from the challenger.
    $\cB$ computes $\ONE.\Vrfy(\one.\vk_i,\one.\cert_i)$ for all $i\in[N]\backslash s$.
    If the results are $\top$ and $\cB$ receives $\one.\MSK_s$ from the challenger, $\cB$ sends $\{\one.\MSK_i\}_{i\in[N]}$ to $\cA_2$.
    Otherwise, $\cB$ aborts.
    \item $\cA_2$ outputs $b'$.
    \item $\cB$ outputs $b'$.
\end{enumerate}
If $b=0$, $\cB$ simulates $\sfhyb{2}{s-1}$.
If $b=1$, $\cB$ simulates $\sfhyb{2}{s}$.
Therefore, it is clear that $\Pr[1\la\cB|b=0]=\Pr[\sfhyb{2}{s-1}=1]$ and $\Pr[1\la\cB|b=1]=\Pr[\sfhyb{2}{s}=1]$.
By assumption, $\abs{\Pr[\sfhyb{2}{s-1}=1]-\Pr[\sfhyb{2}{s}=1]}$ is non-negligible, and therefore $\abs{\Pr[1\la\cB|b=0]-\Pr[1\la\cB|b=1]}$ is non-negligible, which contradicts the single-key certified everlasting adaptive security of $\Sigma_{\one}$.
\end{proof}

\begin{proof}[Proof of \cref{prop:hyb_3_hyb_4_bounded_fe}]
In $\sfhyb{3}{}$, the polynomials $\mu_1,\cdots ,\mu_\ell$ are chosen with constant terms $x_1,\cdots ,x_\ell$, respectively.
In $\sfhyb{4}{}$, these polynomials are now chosen with $0$ constant terms.
This only affects the distribution of $\mu_1,\cdots, \mu_\ell$ themselves and polynomials $\xi_1,\cdots,\xi_S$.
Moreover, only the evaluations of these polynomials on the points in $\mathcal{L}$ affect the outputs of the experiments.
Now observe that:
\begin{itemize}
    \item The distribution of the values $\{\mu_1(i),\cdots, \mu_\ell(i)\}_{i\in\mathcal{L}}$ are identical to both $\sfhyb{3}{}$ and $\sfhyb{4}{}$.
    This is because in both experiments, we choose these polynomials to be random degree $t$ polynomials (with different constraints in the constant term),
    so their evaluation on the points in $\mathcal{L}$ are identically distributed, since $\mathcal{L}$.
    \item The values $\{\xi_1(i),\cdots ,\xi_S(i)\}_{i\in\mathcal{L}}$ depend only on the values $\{\mu_1(i),\cdots,\mu_{\ell}(i)\}_{i\in\mathcal{L}}$.
\end{itemize}
\cref{prop:hyb_3_hyb_4_bounded_fe} follows from these observations.
\end{proof}

\color{black}

==> Sec_OT.tex <==
\section{Certified Everlasting Oblivious Transfer}\label{sec:ot}

\subsection{Definition}\label{sec:ot_def}
\begin{definition}[$k$-out-of-$n$ Certified Everlasting Oblivious Transfer]\label{def:cert_ever_ot}
Let $p$, $q$, $r$, $s$, and $t$ be some polynomial.
A $k$-out-of-$n$ certified everlasting oblivious transfer scheme is a tuple of algorithm $\Sigma=(\mathsf{CRSGen},\mathsf{Receiver},\mathsf{Sender},\mathsf{Derive},\Delete,\Vrfy)$
with plaintext space $\Ms:=\{0,1\}^n$, common reference string space $\mathcal{CRS}\seteq \bit^{p(\secp)}$, first message space $\mathcal{OT}_1:= \bit^{ q(\lambda)}$,
second message space $\mathcal{OT}_2\seteq\cQ^{\otimes r(\secp)}$,
verification key space $\mathcal{VK}:=\{0,1\}^{s(\lambda)}$,
and certificate space $\cD\seteq \cQ^{\otimes t(\lambda)}$.
\begin{description}
    \item[$\mathsf{CRSGen}(1^\secp)\ra \crs$:] 
    This is an algorithm supposed to run by a trusted third party that takes as input the security parameter $1^\secp$, and outputs a common reference string $\crs\in\mathcal{CRS}$.
    \item[$\mathsf{Receiver}(\crs,J)\ra (\mathsf{ot}_1,\state)$:] 
    This is an algorithm supposed to run by a receiver that takes as input $\crs$ and $J\in[n]_k$, and outputs a first message $\mathsf{ot}_1\in\mathcal{OT}_1$ and an internal state $\state$.
    \item[$\mathsf{Sender}(\crs,\mathsf{ot}_1,\bm{\mu}) \ra (\mathsf{ot}_2,\vk)$:]
    This is an algorithm supposed to run by a sender that takes as input takes as input $\crs$, $\mathsf{ot}_1$ and $\bm{\mu}\in\Ms^n$, and outputs a second message $\mathsf{ot}_2\in\mathcal{OT}_2$ and a verification key $\vk\in\mathcal{VK}$.
    \item[$\mathsf{Derive}(\state,\mathsf{ot}_2)\ra (\bm{\mu}',\widehat{\mathsf{ot}_2})$:]
    This is an algorithm supposed to run by a receiver that takes as input $\state$ and $\mathsf{ot}_2$, and outputs $\bm{\mu}'\in\Ms^k$.
    \item[$\Delete(\mathsf{ot}_2)\ra\cert$:]
    This is an algorithm supposed to run by a receiver that takes as input $\mathsf{ot}_2$, and outputs $\cert\in\cD$.
    \item[$\Vrfy(\vk,\cert)\ra \top \,\,{\bf or}\,\, \bot$:]
    This is an algorithm supposed to run by a sender that takes as input $\vk$ and $\cert$, and outputs $\top$ or $\bot$
\end{description}
\end{definition}

We require that a certified everlasting oblivious transfer satisfies correctness defined below.
\begin{definition}[Correctness for Certified Everlasting Oblivious Transfer]\label{def:correct_ever_ot}
There are two types correctness.
The first is decryption correctness,
and the second is verification correctness.

\paragraph{Decryption Correctness:}
There exists a negligible function such that for any $\secp\in \N$, $J=(j_1,\cdots ,j_k)\in[n]_k$ and $\bm{\mu} \in\Ms^n$, 
\begin{align}
\Pr\left[
\bm{\mu}'\neq (\mu_{j_1},\cdots, \mu_{j_k}) 
\ \middle |
\begin{array}{ll}
\crs\la\mathsf{CRSGen}(1^\secp)\\
(\mathsf{ot}_1,\state)\la\mathsf{Receiver}(\crs,J) \\
(\mathsf{ot}_2,\vk)\la\mathsf{Sender}(\crs,\mathsf{ot}_1,\bm{\mu})\\
\bm{\mu}'\la\mathsf{Derive}(\state,\mathsf{ot}_2)
\end{array}
\right] 
\leq\negl(\secp).
\end{align}

\paragraph{Verification Correctness:}
There exists a negligible function such that for any $\secp\in \N$, $J=(j_1,\cdots ,j_k)\in[n]_k$ and $\bm{\mu} \in\Ms^n$, 
\begin{align}
\Pr\left[
\Vrfy(\vk,\cert)= \bot
\ \middle |
\begin{array}{ll}
\crs\la\mathsf{CRSGen}(1^\secp)\\
(\mathsf{ot}_1,\state)\la\mathsf{Receiver}(\crs,J) \\
(\mathsf{ot}_2,\vk)\la\mathsf{Sender}(\crs,\mathsf{ot}_1,\bm{\mu})\\
\cert\la\Delete(\mathsf{ot}_2)
\end{array}
\right] 
\leq\negl(\secp).
\end{align}
\end{definition}



We require that certified everlasting oblivious transfer satisfies the securities defined below.
\begin{definition}[Security for Certified Everlasting Oblivious Transfer]
There are three types of security.
The first is statistical receiver's security,
the second is computational sender's security,
and the third is certified everlasting sender's security.

\paragraph{Statistical Receiver's Security:}
There exists a PPT simulator $\Sim$ such that for any $\secp\in\N$,
and any unbounded distinguisher $\cD$,

\begin{align}
\left|
\Pr\left[
1\la\cD(\crs,\mathsf{ot}_1)
\ \middle |
\begin{array}{ll}
\crs\la\mathsf{CRSGen}(1^\secp)\\
(\mathsf{ot}_1,\state)\la\mathsf{Receiver}(\crs,J) 
\end{array}
\right]
-
\Pr\left[
1\la\cD(\crs,\mathsf{ot}_1)
\ \middle |
\begin{array}{ll}
\crs\la\mathsf{CRSGen}(1^\secp)\\
\mathsf{ot}_1\la\Sim(\crs)
\end{array}
\right] 
\right|
\leq\negl(\secp).
\end{align}



\paragraph{Computational Sender's Security:}
There are PPT algorithm $\Sim_{\mathsf{CRS}}$ and QPT algorithm $\Sim_{\mathsf{sen}}$ and a deterministic classical polynomial-time algorithm $\Open_{\mathsf{rec}}$ such that the following two properties are satisfied.

\begin{itemize}
    \item For any QPT distinguisher $\cD$, we have 
    \begin{align}
        \abs{\Pr[1\la\cD(\crs)|\crs\la\mathsf{CRSGen}(1^\secp)]-\Pr[1\la\cD(\crs)|(\crs,\td)\la\Sim_{\mathsf{CRS}}(1^\secp)]}\leq \negl(\secp).
    \end{align}
    \item For any QPT adversary $\cA=(\cA_0,\cA_1)$ and $\bm{\mu}=(\mu_1,\cdots ,\mu_n)$, we have
    \begin{align}
        &\Bigg|
        \Pr\left[
        1\la\cA_1(\state_\cA, \mathsf{ot}_2)
        \ \middle |
        \begin{array}{ll}
        (\crs,\td)\la\Sim_{\mathsf{CRS}}(1^\secp)\\
        (\mathsf{ot}_1,\state_\cA)\la\cA_0(\crs,\td)\\
        (\mathsf{ot}_2,\vk)\la\mathsf{Sender}(\crs,\mathsf{ot}_1,\bm{\mu})
        \end{array}
        \right]
        -\\
        & \Pr\left[
        1\la\cA_1(\state_\cA,\mathsf{ot}_2)
        \ \middle |
        \begin{array}{ll}
        (\crs,\td)\la\Sim_{\mathsf{CRS}}(1^\secp)\\
        (\mathsf{ot}_1,\state_\cA)\la\cA_0(\crs,\td)\\
        J\seteq \Open_{\mathsf{rec}}(\td,\mathsf{ot}_1)\\
        \mathsf{ot}_2\la\Sim_{\mathsf{Sen}}(\crs,\mathsf{ot}_1,J,\bm{\mu})
        \end{array}
        \right] 
        \Bigg |
        \leq\negl(\secp).
    \end{align}
\end{itemize}


\paragraph{Certified Everlasting Sender's Security:}
There are PPT algorithm $\Sim_{\mathsf{CRS}}$ and QPT algorithm $\Sim_{\mathsf{sen}}$ and a deterministic classical polynomial-time algorithm $\Open_{\mathsf{rec}}$ such that the following two properties are satisfied.

\begin{itemize}
    \item For any QPT distinguisher $\cD$, we have 
    \begin{align}
        \abs{\Pr[1\la\cD(\crs)|\crs\la\mathsf{CRSGen}(1^\secp)]-\Pr[1\la\cD(\crs)|(\crs,\td)\la\Sim_{\mathsf{CRS}}(1^\secp)]}\leq \negl(\secp).
    \end{align}
    \item For any adversary $\cA=(\cA_0,\cA_1,\cA_2)$, where $\cA_0$ and $\cA_1$ are QPT adversaries and $\cA_2$ is an unbounded adversary, and $\bm{\mu}=(\mu_1,\cdots ,\mu_n)$, we have
    \begin{align}
        &\Bigg|
        \Pr\left[
        1\la\cA_2(\state_{\cA}^*)\wedge \top\la\Vrfy(\vk,\cert)
        \ \middle |
        \begin{array}{ll}
        (\crs,\td)\la\Sim_{\mathsf{CRS}}(1^\secp)\\
        (\mathsf{ot}_1,\state_\cA)\la\cA_0(\crs,\td)\\
        (\mathsf{ot}_2,\vk)\la\mathsf{Sender}(\crs,\mathsf{ot}_1,\bm{\mu})\\
        (\cert,\state_\cA^*)\la\cA_1(\mathsf{ot}_2,\state_\cA)
        \end{array}
        \right]
        -\\
        & \Pr\left[
        1\la\cA_2(\state_{\cA}^*)\wedge \top\la\Vrfy(\vk,\cert)
        \ \middle |
        \begin{array}{ll}
        (\crs,\td)\la\Sim_{\mathsf{CRS}}(1^\secp)\\
        (\mathsf{ot}_1,\state_\cA)\la\cA_0(\crs,\td)\\
        J\seteq \Open_{\mathsf{rec}}(\td,\mathsf{ot}_1)\\
        (\mathsf{ot}_2,\vk)\la\Sim_{\mathsf{Sen}}(\crs,\mathsf{ot}_1,J,\bm{\mu})\\
        (\cert,\state_{\cA}^*)\la\cA_1(\mathsf{ot}_2,\state_\cA)
        \end{array}
        \right] 
        \Bigg |
        \leq\negl(\secp).
    \end{align}
\end{itemize}
%\begin{align}
%\left|
%\Pr\left[
%1\la\cD(\state)
%\ \middle |
%\begin{array}{ll}
%\crs\la\mathsf{CRSGen}(1^\secp)\\
% (\mathsf{ot}_1,r_1)\la\cA_1(\crs)\\
%\mathsf{ot}_2\la\mathsf{Send}(\mathsf{ot}_1,(m_0,m_1),\crs)\\
%\state\la\cA_2(r_1,\mathsf{ot}_2)
%\end{array}
%\right]
%-
%\Pr\left[
%1\la\cD(\state)
%\ \middle |
%\begin{array}{ll}
%\crs\la\mathsf{CRSGen}(1^\secp)\\
%\state\la\Sim^{\mathcal{I}[m_0,m_1](\cdot)}(\crs)\\
%\end{array}
%\right] 
%\right|
%\leq\negl(\secp).
%\end{align}
\end{definition}

In \cref{sec:const_ot_wo_rom}, we construct a certified everlasting OT scheme with constant plaintext space.
We can extend it to a certified everlasting OT scheme with polynomial plaintext space by using following \cref{lem:ot_poly}.
\begin{lemma}\label{lem:ot_poly}
If there exists a certified everlasting OT scheme with constant plaintext space, then there exists a certified everlasting OT scheme with polynomial plaintext space.
\end{lemma}



\subsection{Construction with QROM}\label{sec:const_ot}
In this section, we present how to construct a certified everlasting oblivious transfer scheme from one-time SKE with certified deletion (\cref{def:sk_cert_del}), oblivious transfer (\cref{def:ot}), and hash function modeled as a quantum random oracle.
Our construction in this section is similar to the certified everlasting commitment scheme presented in \cite{EPRINT:HMNY21_2}.
The difference is that we use OT instead of commitment as in \cite{EPRINT:HMNY21_2}.

\paragraph{Our certified everlasting oblivious transfer scheme.}
We construct a certified everlasting oblivious transfer scheme $\Sigma_{\mathsf{ceot}}=(\mathsf{CRSGen},\mathsf{Receiver},\mathsf{Sender},\mathsf{Derive},\Delete,\Vrfy)$
from a one-time SKE with certified deletion scheme $\Sigma_{\mathsf{skcd}}=\SKE.(\keygen,\Enc,\Dec,\Delete,\Vrfy)$~(\cref{def:sk_cert_del}),
a OT scheme $\Sigma_{\comp}=\COMP.(\mathsf{CRSGen},\mathsf{Receiver},\mathsf{Sender},\mathsf{Derive},\Delete,\Vrfy)$~(\cref{def:pke}),
and a hash function $H$ modeled as quantum random oracle.
Each space is defined similarly to the construction of certified everlasting SKE in \cref{sec:const_ske_rom}.

\begin{description}
\item[$\mathsf{CRSGen}(1^\secp)$:] $ $
\begin{itemize}
    \item Generate $\mathsf{comp}.\crs\la\mathsf{COMP}.\mathsf{CRSGen}(1^\secp)$.
    \item Output $\crs\seteq \mathsf{comp}.\crs$.
\end{itemize}
\item[$\mathsf{Receiver}(\crs,J)$:] $ $
\begin{itemize}
    \item Parse $\crs=\mathsf{comp}.\crs$ and $J\seteq (j_1,\cdots,j_k)\in[n]_k$.
    \item Compute
    $(\comp.\mathsf{ot}_1,\comp.\state)\la\mathsf{COMP}.\mathsf{Receiver}(\mathsf{comp}.\crs,J)$.
    \item Output $\mathsf{ot}_1\seteq \comp.\mathsf{ot}_1$ and $\state\seteq (\comp.\state,J)$.
\end{itemize}
\item[$\mathsf{Sender}(\crs,\mathsf{ot}_1,\bm{\mu})$:]$ $
\begin{itemize}
    \item Parse $\crs =\comp.\crs$, $\mathsf{ot}_1=\comp.\mathsf{ot}_1$ and $\bm{\mu} \seteq (\mu_1,\cdots,\mu_n)$.
    \item For $i\in[n]$, generate $\ske.\sk_i\la\SKE.\keygen(1^\secp)$ and $R_i\la\bit^{\secp}$.
    Let $\bm{R}\seteq (R_1,\cdots,R_n)$.
    \item For $i\in[n]$, compute $\ske.\ct_i\la\SKE.\Enc(\ske.\sk_i,\mu_i)$.
    \item For $i\in[n]$, compute $h_i\seteq H(R_i)\oplus \ske.\sk_i$.
    \item For $i\in[n]$, compute $\comp.\mathsf{ot}_2\la\COMP.\mathsf{Sender}(\comp.\crs,\comp.\mathsf{ot}_1,\bm{R})$.
    \item Output $\mathsf{ot}_2\seteq (\{\ske.\ct_i\}_{i\in[n]},\{h_i\}_{i\in[n]},\comp.\mathsf{ot}_2)$ and $\vk\seteq \{\ske.\sk_i\}_{i\in[n]}$.
\end{itemize}
\item[$\mathsf{Derive}(\state,\mathsf{ot}_2)$:] $ $
\begin{itemize}
    \item Parse $\state=\comp.\state$ and $\mathsf{ot}_2=(\{\ske.\ct_i\}_{i\in[n]},\{h_i\}_{i\in[n]},\comp.\mathsf{ot}_2)$.
    \item Compute $\bm{R}'\la\COMP.\mathsf{Derive}(\comp.\state,\comp.\mathsf{ot}_2)$, where $\bm{R}'=(R'_{j_1},\cdots,R'_{j_k})$ with $R'_{j_i}\in\Ms$ for all $i\in[k]$.
    \item For $i\in[k]$, compute $\ske.\sk'_{j_i}=h_{j_i}\oplus R'_{j_i}$.
    \item For $i\in[k]$, compute $\mu'_{j_i}\la\SKE.\Dec(\ske.\sk'_{j_i},\ske.\ct_{j_i})$.
    \item Output $\bm{\mu}'\seteq (\mu'_{j_1},\cdots,\mu'_{j_k})$.
\end{itemize}
\item[$\Delete(\mathsf{ot}_2)$:] $ $
\begin{itemize}
    \item Parse $\mathsf{ot}_2=(\{\ske.\ct_i\}_{i\in[n]},\{h_i\}_{i\in[n]},\comp.\mathsf{ot}_2)$.
    \item For $i\in[n]$, compute $\ske.\cert_i\la\SKE.\Delete(\ske.\ct_i)$.
    \item Output $\cert\seteq \{\ske.\cert_i\}_{i\in[n]}$.
\end{itemize}
\item[$\Vrfy(\vk,\cert)$:]$ $
\begin{itemize}
    \item Parse $\vk\seteq\{\ske.\sk_i\}_{i\in[n]}$ and $\cert =\{\ske.\cert_i\}_{i\in[n]}$.
    \item For $i\in[n]$, compute $\top/\bot\la\Vrfy(\ske.\sk_i,\ske.\cert_i)$.
    If all results are $\top$, output $\top$.
\end{itemize}
\end{description}
\paragraph{Correctness:}
Decryption correctness easily follows from the decryption correctness of $\Sigma_{\comp}$ and $\Sigma_{\mathsf{skcd}}$.
Verification correctness easily follows from the verification correctness of $\Sigma_{\mathsf{skcd}}$.

\paragraph{Security:}
The following three theorem holds.
\begin{theorem}\label{thm:stat_sec_ot_rom}
If $\Sigma_{\comp}$ satisfies the statistical receiver's security, $\Sigma_{\mathsf{ceot}}$ satisfies the statistical receiver's security.
\end{theorem}
The statistical receiver's security of $\Sigma_{\mathsf{ceot}}$ easily follows from the statistical receiver's security of $\Sigma_{\comp}$.


\begin{theorem}\label{thm:comp_sec_ot_rom}
If $\Sigma_{\mathsf{skcd}}$ satisfies the OT-CD security and $\Sigma_{\comp}$ satisfies the computational sender's security, $\Sigma_{\mathsf{ceot}}$ satisfies the computational sender's security.
\end{theorem}
The computational sender's security of $\Sigma_{\mathsf{ceot}}$ easily follows from the computational sender's security of $\Sigma_{\comp}$ and the OT-CD security of $\Sigma_{\mathsf{skcd}}$.

\begin{theorem}\label{thm:ever_sec_ot_rom}
If $\Sigma_{\mathsf{skcd}}$ satisfies the OT-CD security and $\Sigma_{\comp}$ satisfies the computational sender's security, $\Sigma_{\mathsf{ceot}}$ satisfies the certified everlasting sender's security.
\end{theorem}
The proof is very similar to that of \cref{thm:sk_ever_security}. Therefore, we skip the proof.



\subsection{Construction without QROM}\label{sec:const_ot_wo_rom}
In this section, we present how to construct a certified everlasting OT scheme with constant plaintext space
from OT without QROM.
We note that we can extend a certified everlasting OT scheme with constant plaintext space to a certified everlasting OT scheme with polynomial plaintext space by using \cref{lem:ot_poly}.
Our construction in this section is similar to that of quantum timed-release encryption presented in \cite{JACM:Unruh15}.
The difference is that we use OT instead of timed-release encryption as in \cite{JACM:Unruh15}.

\paragraph{Our certified everlasting OT scheme without QROM.}
Let $k_1$ and $k_2$ be some constant such that $k_1>k_2$.
Let $p$, $q$, $r$, $s$, $t$ and $u$ be some polynomials.
Let $C_1$ and $C_2$ be a CSS code with parameters $q,k_1,k_2,t$.
We construct a certified everlasting OT scheme
$\Sigma_{\mathsf{ceot}}=(\mathsf{CRSGen},\mathsf{Receiver},\mathsf{Sender},\mathsf{Derive},\Delete,\Vrfy)$, with plaintext space $\Ms=C_1/C_2$ (isomorphic $\bit^{(k_1-k_2)}$), 
common reference string space $\mathcal{CRS}\seteq\bit^{u(\secp)}$,
first message space $\mathcal{OT}_1\seteq \bit^{s(\lambda)}$,
second message space $\Cs=\cQ^{\otimes n\cdot\left(p(\lambda)+q(\lambda)\right)}\times \{0,1\}^{r(\lambda)}\times (\bit^{q(\lambda)}/C_1)^n\times (C_1/C_2)^n$,
verification key space $\mathcal{VK}=\{0,1\}^{np(\lambda)}\times ([p(\lambda)+q(\lambda)]_{p(\lambda)})^n\times \bit^{np(\lambda)}$ 
and deletion certificate space $\mathcal{D}=\mathcal{Q}^{\otimes n\cdot\left(p(\lambda)+q(\lambda)\right)}$
from the following primitive.
\begin{itemize}
    \item A OT scheme $\Sigma_{\comp}=\COMP.(\mathsf{CRSGen},\mathsf{Receiver},\mathsf{Sender},\mathsf{Derive},\Delete,\Vrfy)$ with
    plaintext space $\Ms=\{0,1\}^{p(\lambda)}\times[p(\lambda)+q(\lambda)]_{p(\lambda)}\times \bit^{p(\lambda)} \times C_1/C_2$,
    common reference string space $\mathcal{CRS}=\bit^{u(\lambda)}$,
    first message space $\mathcal{OT}_1=\{0,1\}^{s(\secp)}$
    and second message space $\mathcal{OT}_2=\bit^{r(\lambda)}$.
\end{itemize}
The construction is as follows. (We will omit the security parameter below.)

\begin{description}
\item[$\mathsf{CRSGen}(1^\secp)$:]$ $
\begin{itemize}
    \item Compute $\comp.\crs\la\COMP.\mathsf{CRSGen}(1^\secp)$.
    \item Output $\crs\seteq \comp.\crs$.
\end{itemize}
\item[$\mathsf{Receiver}(\crs,J)$:]$ $
\begin{itemize}
    \item Parse $\crs=\comp.\crs$ and $J=(j_1,\cdots,j_k)\in[n]_k$.
    \item Compute $(\comp.\mathsf{ot}_1,\comp.\state)\la\COMP.\mathsf{Sender}(\comp.\crs,J)$.
    \item Output $\mathsf{ot}_1\seteq\comp.\mathsf{ot}$ and $\state\seteq (\comp.\state,J)$.
\end{itemize}
\item[$\mathsf{Sender}(\crs,\mathsf{ot}_1,\bm{\mu})$:]$ $
\begin{itemize}
    \item Parse $\crs=\comp.\crs$, $\mathsf{ot}_1=\comp.\mathsf{ot}_1$ and $\bm{\mu}=(\mu_1,\cdots,\mu_n)$.
    \item For $i\in[n]$, generate $B_i\la\bit^{p}$, $Q_i\la[p+q]_{p}$, $y_i\la C_1/C_2$, $u_i\la\bit^q/C_1$, $r_i\la\bit^p$, $x_i\la C_1/C_2$, $w_i\la C_2$.
    \item Let $\bm{B}=(B_1,\cdots,B_n)$, $\bm{Q}=(Q_1,\cdots,Q_n)$, $\bm{r}=(r_1,\cdots,r_n)$ and $\bm{y}=(y_1,\cdots, y_n)$.
    \item Compute
    $\comp.\mathsf{ot}_2\la\COMP.\mathsf{Sender}(\comp.\crs,\comp.\mathsf{ot}_1,(\bm{B},\bm{Q},\bm{r},\bm{y}))$.
    \item Let $U_Q$ be the unitary that permutes the qubits in $Q$ into the first half of the system.
    (I.e., $U_Q|x_1x_2\cdots x_{p+q}\rangle=|x_{a_1}x_{a_2}\cdots x_{a_p}x_{b_1}x_{b_2}\cdots x_{b_q}\rangle$ with $Q\seteq \{a_1,a_2,\cdots, a_p\}$ and $\{1,2,\cdots, p+q\}/Q\seteq \{b_1,b_2,\cdots,b_q\}$.)
    \item For $i\in[n]$, construct a quantum state $|\Psi_i\rangle \seteq U_{Q_i}^{\dagger}(H^{B_i}\otimes I^{\otimes q})(|r_i\rangle\otimes |x_i\oplus w_i\oplus u_i\rangle)$.
    \item For $i\in[n]$, compute $h_i\seteq \mu_i\oplus x_i\oplus y_i$.
    \item Output $\mathsf{ot}_2\seteq (\{|\Psi_i\rangle\}_{i\in[n]},\comp.\mathsf{ot}_2,\{u_i\}_{i\in[n]},\{h_i\}_{i\in[n]})$ and $\vk\seteq (\bm{B},\bm{Q},\bm{r})$.
\end{itemize}
\item[$\mathsf{Derive}(\state,\mathsf{ot}_2)$:]$ $
\begin{itemize}
    \item Parse $\state =(\comp.\state,J)$ and $\mathsf{ot}_2=(\{|\Psi_i\rangle\}_{i\in[n]},\comp.\mathsf{ot}_2,\{u_i\}_{i\in[n]},\{h_i\}_{i\in[n]})$.
    \item Compute $(\bm{B}',\bm{Q}',\bm{r}',\bm{y}')\la \COMP.\mathsf{Derive}(\comp.\state,\comp.\mathsf{ot}_2)$, where $\bm{B}'=(B'_{j_1},\cdots,B'_{j_k})$, $\bm{Q}'=(Q'_{j_1},\cdots,Q'_{j_k})$, $\bm{r}'=(r'_{j_1},\cdots, r'_{j_k})$ and $\bm{y}'=(y'_{j_1},\cdots, y'_{j_k})$.
    \item For $i\in[k]$, apply $U_{Q_{j_i}}$ to $|\Psi_{j_i}\rangle$, measure the last $q$-qubits of $|\Psi_i\rangle$ in the computational basis, and obtain measurement outcome $\gamma_{j_i}$.
    \item For $i\in[k]$, compute $x_{j_i}\seteq \gamma_{j_i}\oplus u_{j_i}$.
    \item For $i\in[k]$, compute $\mu_{j_i}=h_{j_i}\oplus x_{j_i}\oplus y_{j_i}$.
    \item Output $\bm{\mu}'=(\mu_{j_1},\cdots ,\mu_{j_k})$.
\end{itemize}
\item[$\Delete(\mathsf{ot}_2)$:]$ $
\begin{itemize}
    \item Parse $\mathsf{ot}_2=(\{|\Psi_i\rangle\}_{i\in[n]},\comp.\mathsf{ot}_2,\{u_i\}_{i\in[n]},\{h_i\}_{i\in[n]})$.
    \item Output $\cert\seteq\{|\Psi_i\rangle\}_{i\in[n]}$.
\end{itemize}
\item[$\Vrfy(\vk,\cert)$:]$ $
\begin{itemize}
    \item Parse $\vk=(\bm{B},\bm{Q},\bm{r})$ and $\cert=\{|\Psi_i\rangle\}_{i\in[n]}$.
    \item For $i\in[n]$, apply $(H^{B_{i}}\otimes I^{\otimes q})U_{Q_i}$ to $|\Psi_i\rangle$, measure the first $p$-qubits in the computational basis and obtain the measurement outcome $r'_i$.
    \item Output $\top$ if $r_i=r'_i$ for all $i\in[n]$ , and output $\bot$ otherwise.
\end{itemize}
\end{description}

\paragraph{Correctness:}
Decryption correctness and verification easily follows from the decryption correctness of $\Sigma_{\comp}$.


\paragraph{Security:}
The following three theorem holds.
\begin{theorem}\label{thm:stat_sec_ot_wo_rom}
If $\Sigma_{\comp}$ satisfies the statistical receiver's security, $\Sigma_{\mathsf{ceot}}$ satisfies the statistical receiver's security.
\end{theorem}
The statistical receiver's security of $\Sigma_{\mathsf{ceot}}$ easily follows from the statistical receiver's security of $\Sigma_{\comp}$.

\begin{theorem}\label{thm:comp_sec_ot_wo_rom}
If $\Sigma_{\comp}$ satisfies the computational sender's security, $\Sigma_{\mathsf{ceot}}$ satisfies the computational sender's security.
\end{theorem}
The computational sender's security of $\Sigma_{\mathsf{ceot}}$ easily follows from the computational sender's security of $\Sigma_{\comp}$.


\begin{theorem}\label{thm:ever_sec_ot_wo_rom}
If $\Sigma_{\comp}$ satisfies the computational sender's security and $tp/(p+q)-4(k_1-k_2){\rm ln}2$ is superlogarithmic, $\Sigma_{\mathsf{ceot}}$ satisfies the certified everlasting sender's security.
\end{theorem}
The proof is very similar to that of \cref{thm:sk_ever_security_wo_rom}. Therefore, we skip the proof.




==> Sec_Proof_rom.tex <==
% !TEX root = main.tex
% !TEX spellcheck = en-US


\section{Proof of \cref{thm:sk_ever_security}}\label{sec:proof_rom}
In this section, we prove \cref{thm:sk_ever_security}.
We note that the proof is similar to that of \cite[Theorem3.9]{EPRINT:HMNY21_2}.
For the convenience of readers, we describe the proof.
(Note that a large part of the proof is directly taken from \cite{EPRINT:HMNY21_2}.)
\begin{proof}[Proof of \cref{thm:sk_ever_security}]

We describe how the experiment $\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)$ works against an adversary $\cA\coloneqq (\cA_1,\cA_2)$ consisting of any QPT adversary $\cA_1$ and any quantum unbounded time adversary $\cA_2$.
For notational simplicity, let $u$ be the number of times that $\cA$ query encryption oracle in the experiment.
(We note that $\cA$ can query encryption oracle polynomially arbitrary times.)
\begin{description}
    \item[$\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)$:] This is the original experiment.


\begin{enumerate}
    \item A uniformly random function $H$ from $\{0,1\}^{\lambda}$ to $\{0,1\}^{q(\lambda)}$ is chosen.
    $\cA_1$ and $\cA_2$ can make arbitrarily many quantum queries to $H$ at any time in the experiment. 
    \item The challenger generates $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item $\cA_1$ sends an encryption query $m_i\in\Ms$ to the challenger. The challenger samples $R_i\la\bit^{\secp}$,
    computes $\ske.\CT_i\la \SKE.\Enc(\ske.\sk,R_i)$,
    $\mathsf{cd}.\sk_i\la\mathsf{CD}.\keygen(1^\secp)$,
    $\mathsf{cd}.\ct_i\la\mathsf{CD}.\Enc(\mathsf{cd}.\sk_i,m_i)$ and $h_i\seteq H(R_i)\oplus \mathsf{cd}.\sk_i$,
    and sends $(\mathsf{cd}.\sk_i,h_i,\ske.\ct_i,\mathsf{cd}.\ct_i)$ to the challenger.
    %\footnote{Note that, 
    %in $\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)$, the challenger also sends $\vk$ in addition to $\ct$ against an encryption query
    %and that $\mathsf{cd}.\sk$ is $\vk$ of $\Sigma_{\mathsf{cesk}}$.}.
    $\cA_1$ repeats this process for $i\in[\ell]$.
    \item $\cA_1$ chooses $(M_0,M_1)\in\cM^2$, and sends $(M_0,M_1)$ to the challenger.
    \item The challenger samples $R\la\bit^{\secp}$,
    computes $\ske.\CT\la \SKE.\Enc(\ske.\sk,R)$,
    $\mathsf{cd}.\sk\la\mathsf{CD}.\keygen(1^\secp)$,
    $\mathsf{cd}.\ct\la\mathsf{CD}.\Enc(\mathsf{cd}.\sk,M_b)$ and $h\seteq H(R)\oplus \mathsf{cd}.\sk$,
    and sends $(h,\ske.\ct,\mathsf{cd}.\ct)$ to the challenger.
    \item $\cA_1$ sends an encryption query $m_i\in\Ms$ to the challenger.
    The challenger samples $R_i\la\bit^{\secp}$,
    computes $\ske.\CT_i\la \SKE.\Enc(\ske.\sk,R_i)$,
    $\mathsf{cd}.\sk_i\la\mathsf{CD}.\keygen(1^\secp)$,
    $\mathsf{cd}.\ct_i\la\mathsf{CD}.\Enc(\mathsf{cd}.\sk_i,m_i)$ and $h_i\seteq H(R_i)\oplus \mathsf{cd}.\sk_i$,
    and sends $(\mathsf{cd}.\sk_i,h_i,\ske.\ct_i,\mathsf{cd}.\ct_i)$ to the challenger.
    $\cA_1$ repeats this process for $i\in\{\ell+1,\cdots,u\}$.
    \item $\cA_1$ sends $\mathsf{cd}.\cert$ to the challenger, and sends its internal state to $\cA_2$.
    \item If $\top\lrun\mathsf{CD}.\Vrfy(\mathsf{cd}.\sk,\mathsf{cd}.\cert)$,
    the challenger outputs $\top$, and sends $\ske.\sk$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$, and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
What we have to prove is that 
\begin{align}
\advd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\secp)
\seteq \abs{\Pr[ \expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\secp, 0)=1] - \Pr[ \expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\secp, 1)=1] }\leq \negl(\secp).
\end{align}
To describe the sequence of hybrid experiments,
let us denote $\mathcal{R}\seteq \{R,\{R_i\}_{i\in[u]}\}$.
%Let us define $\Lambda \subseteq[u]$ such that $j\in \Lambda$ whe $R=R^j$ for every $j\in[u]$.
%Let us assume that $R^i\neq R$ and $R^i\neq R^j$ for all $j\in[i-1]$.
%Then, let us define $\Lambda^i\subseteq [u]$ such that $j\in\Lambda^i$ when $R^i=R^j$ and $i<j\leq u$.
We define the following sequence of hybrids.
    \item [$\sfhyb{1}{}(b)$:]This is identical to $\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\secp, b)$ except that the oracle given to $\cA_1$ is replaced with $H_{R\ra H'}$ which is $H$ reprogrammed according to $H'$ on an input $R^*\in \mathcal{R}$ where $H'$ is another independent uniformly random function.
    More formally, $H_{R\ra H'}$ is defined by 
    \begin{align}
    H_{R\rightarrow H'}(R^*) \coloneqq
    \begin{cases}
    H(R^*)~~~&(R^*\notin \mathcal{R})\\
    H'(R^*)~~~&(R^*\in \mathcal{R}).
    \end{cases}
    \end{align}
    We note that the challenger still uses $H$ to generate $h$ and $h_i$ for each $i\in[u]$
    and the oracle
    which $\cA_2$ uses is still $H$ similarly to the original experiment.
    \item [$\sfhyb{2}{}(b)$:]
    This experiment is identical to $\sfhyb{1}{}(b)$ except for the following four points.
    First, the challenger aborts the protocol if $R=R_i$ for some $i\in[u]$ or $R_i= R_j$ for some $i,j\in[u]$ with $i\neq j$.
    In that case, the experiment outputs $\bot$.
    Second, the challenger generates $h$ and $h_i$ for $i\in[u]$ uniformly at random.
    Third, the oracle given to $\cA_1$ is replaced with $H'$ which is an independent uniformly random function.
    Fourth, the oracle given to $\cA_2$ is replaced with $H'_{R\ra h\oplus \mathsf{cd}.\sk}$ which is $H'$ reprogrammed to $h_i\oplus \mathsf{cd}.\sk_i$ on an input $R_i$ for each $i\in[u]$ and reprogrammed to $h\oplus \mathsf{cd}.\sk$ on an input $R$.
    More formally, $H'_{R\ra h\oplus \mathsf{cd}.\sk}$ is defined by 
    \begin{align}
    H'_{R\rightarrow h\oplus \mathsf{cd}.\sk}(R^*)\seteq
    \begin{cases}
    H'(R^*)~~~&(R^*\notin \mathcal{R})\\
    h_i\oplus \mathsf{cd}.\sk_i ~~~&(R^*=R_i)\\
    h\oplus \mathsf{cd}.\sk~~~&(R^*=R).
    \end{cases}
\end{align}
\end{description}

\begin{proposition}\label{prop:Exp_Hyb_1_cert_sk}
If $\Sigma_{\mathsf{sk}}$ satisfies the OW-CPA security, then
\begin{align}
    \abs{\Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\secp, b)=1]-\Pr[\sfhyb{1}{}(b)=1]}\leq\negl(\lambda).
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:Exp_Hyb_1_cert_sk}]
We assume that $\abs{\Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\secp, b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is non-negligible,
and construct an adversary $\cB$ that breaks the OW-CPA security of $\Sigma_{\mathsf{sk}}$.
For notational simplicity, we denote $\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\secp, b)$ as $\sfhyb{0}{}(b)$.
We consider an algorithm $\widetilde{\cA}$ that works as follows.
$\widetilde{\cA}$ is given an oracle $\mathcal{O}$, which is either $H$ or $H_{R\ra H'}$, and an input $z$ that consists of $\mathcal{R}= \{R,\{R_i\}_{i\in[u]}\}$ and the whole truth table of $H$, where $R\la \bit^{\lambda}$, $R_i\la\bit^{\lambda}$ for all $i\in[u]$, and $H$ and $H'$ are uniformly random functions.
$\widetilde{\cA}$ runs $\sfhyb{0}{}(b)$ except that it uses its own oracle $\mathcal{O}$ to simulate $\cA_1$'s random oracle queries.
On the other hand, $\widetilde{\cA}$ uses $H$ to simulate $h$, $h_i$ for all $i\in[u]$ and $\cA_2$'s random oracle queries regardless of $\mathcal{O}$,
which is possible because the truth table of $H$ is included in the input $z$.
By definition, we have
\begin{align}
    \Pr[\sfhyb{0}{}(b)=1]=\Pr[\widetilde{\cA}^H(\mathcal{R},H)=1]
\end{align}
and
\begin{align}
    \Pr[\sfhyb{1}{}(b)=1]=\Pr[\widetilde{\cA}^{H_{R\ra H'}}(\mathcal{R},H)=1]
\end{align}
where $H$ in the input means the truth table of $H$.
We apply the one-way to hiding lemma (\cref{lem:one-way_to_hiding}) to the above $\widetilde{\cA}$.
Note that $\widetilde{\cA}$ is inefficient, but the one-way to hiding lemma is applicable to inefficient algorithms.
Then if we let $\widetilde{\cB}$ be the algorithm that measures uniformly chosen query of $\widetilde{\cA}$, we have
\begin{align}
    \abs{\Pr[\widetilde{\cA}^H(\mathcal{R},H)=1]-\Pr[\widetilde{\cA}^{H_{R\ra H'}}(\mathcal{R},H)=1]}\leq 2q\sqrt{\Pr[\widetilde{\cB}^{H_{R\ra H'}}(\mathcal{R},H)\in \mathcal{R}]}.
\end{align}
By the assumption, the LHS is non-negligible, and thus $\Pr[\widetilde{\cB}^{H_{R\ra H'}}(\mathcal{R},H)\in \mathcal{R}]$ is non-negligible.

Let $\widetilde{\cB'}$ be the algorithm that is the same as $\widetilde{\cB}$ except for the following three points.
First, it does not take the truth table of $H$ as input.
Second, it sets $h$ to be uniformly random string instead of setting $h\seteq H(R)\oplus \mathsf{cd}.\sk$.
Third, it sets $h_i$ to be uniformly random string instead of setting $h_i\seteq H(R_i)\oplus \mathsf{cd}.\sk_i$ for $i\in [u]$.
Then we have
\begin{align}
    \Pr[\widetilde{\cB}^{H_{R\ra H'}}(\mathcal{R},H)\in \mathcal{R}]=\Pr[\widetilde{\cB'}^{H_{R\ra H'}}(\mathcal{R})\in \mathcal{R}].
\end{align}
The reason is as follows:
First, $\widetilde{\cB}$ uses the truth table of $H$ only for generating $h\seteq H(R)\oplus \mathsf{cd}.\sk$ and $h_i\seteq H(R_i)\oplus \mathsf{cd}.\sk_i$ for $i\in[u]$,
because it halts before $\widetilde{\cB}$ simulates $\cA_2$.
Second, the oracle $H_{R\ra H'}$ reveals no information about $H(R^*)$ for $R^*\in \mathcal{R}$,
and thus $h$ and $h_i$ for $i\in [u]$ can be independently and uniformly random.

Moreover, for any fixed $\mathcal{R}$, when $H$ and $H'$ are uniformly random, $H_{R\ra H'}$ is also a uniformly random function, and therefore we have
\begin{align}
     \Pr[\widetilde{\cB'}^{H_{R\ra H'}}(\mathcal{R})\in \mathcal{R}]=\Pr[\widetilde{\cB'}^{H}(\mathcal{R})\in \mathcal{R}].
\end{align}
Since $\Pr[\widetilde{\cB}^{H_{R\ra H'}}(\mathcal{R},H)\in \mathcal{R}]$ is non-negligible, $\Pr[\widetilde{\cB'}^{H}(\mathcal{R})\in \mathcal{R}]$ is also non-negligible.
Recall that $\widetilde{\cB'}^H$ is an algorithm that simulates $\sfhyb{0}{}(b)$ with the modification that $h$ and $h_i$ for all $i\in[u]$ are set to be uniformly random and measures random chosen $\cA_1$'s query. Then it is straightforward to construct an adversary $\cB$ that breaks the OW-CPA security of $\Sigma_{\mathsf{sk}}$ by using $\widetilde{\cB'}$. For clarity, we give the description of $\cB$ below.


$\cB$ receives $(\ske.\ct,\{\ske.\ct_i\}_{i\in[u]})$ from the challenger of $\expa{\Sigma_{\mathsf{sk}},\cB}{ow}{cpa}(\secp)$.
$\cB$ chooses $j\la[q]$ and runs $\sfhyb{1}{}(b)$
until $\cA_1$ makes $j$-th random oracle query or $\cA_1$ sends the internal state to $\cA_2$.
For the $i$-th encryption query, $\cB$ does the following.
$\cB$ receives $m_i$ from $\cA_1$.
$\cB$ simulates $(\mathsf{cd}.\sk_i,h_i,\ske.\ct_i,\mathsf{cd}.\ct_i)$,
where $\cB$ embeds the problem instance $\ske.\ct_i$ into those sent to $\cA_1$ instead of generating it by itself.
$\cB$ repeats this process for $i\in[\ell]$.
$\cB$ receives $(M_0,M_1)$ from $\cA_1$.
$\cB$ simulates $(h,\ske.\ct,\mathsf{cd}.\ct)$,
where $\cB$ embeds the problem instance $\ske.\ct$ into those sent to $\cA_1$ instead of generating it by itself.
For the $i$-th encryption query, $\cB$ does the following.
$\cB$ receives an encryption query $m_i$ from $\cA_1$.
$\cB$ simulates $(\mathsf{cd}.\sk_i,h_i,\ske.\ct_i,\mathsf{cd}.\ct_i)$,
where $\cB$ embeds the problem instance $\ske.\ct_i$ into those sent to $\cA_1$ instead of generating it by itself.
$\cB$ repeats this process for $i\in\{\ell+1,\cdots,u\}$.
In this process, $\cB$ stops the simulation when $\cA_1$ makes $j$-th random oracle query, measures $j$-th random oracle query by $\cA_1$, and outputs the measurement outcome.
Note that $\cB$ can efficiently simulate the random oracle $H$ by Zhandry's compressed oracle technique.
It is clear that the probability that $\cB$ obtains $R^*$ such that $R^*\in \mathcal{R}$ is exactly
$\Pr[\widetilde{\cB'}^H(\mathcal{R})\in \mathcal{R}]$, which is non-negligible.
This contradicts the OW-CPA security of $\Sigma_{\mathsf{sk}}$.
Therefore, $\abs{\Pr[\sfhyb{0}{}(b)=1]-\Pr[\sfhyb{1}{}(b)=1]}$ is negligible.
\end{proof}


\begin{proposition}\label{prop:hyb_1_hyb_2_cert_sk}
$\abs{\Pr[\sfhyb{1}{}(b)=1]-\Pr[\sfhyb{2}{}(b)=1]}\leq\negl(\lambda)$.
\end{proposition}
\begin{proof}[Proof of \cref{prop:hyb_1_hyb_2_cert_sk}]
Let $\mathsf{Collide}$ be the event that $R=R_i$ for some $i\in[u]$, or $R_i=R_j$ for some $i,j\in[u]$ with $i\neq j$.
Then, it holds that 
\begin{align}
    \Pr[\sfhyb{1}{}(b)=1\wedge \overline{\mathsf{Collide}}]=\Pr[\sfhyb{2}{}(b)=1\wedge \overline{\mathsf{Collide}}].
\end{align}
This is because when $\mathsf{Collide}$ does not occur,
the joint probability distribution of the bit string and the oracle given to the adversary $\cA=(\cA_1,\cA_2)$ in $\sfhyb{1}{}(b)$ is equivalent to that of $\sfhyb{2}{}(b)$. 
Thus, from difference lemma (\cref{lem:defference}), it holds that
\begin{align}
    \abs{ \Pr[\sfhyb{1}{}(b)=1]-\Pr[\sfhyb{2}{}(b)=1]}\leq \Pr[\mathsf{Collide}].
\end{align}
From the definition of $\mathsf{Collide}$, $\Pr[\mathsf{Collide}]$ is negligible. 
Thus, it holds that
\begin{align}
    \abs{\Pr[\sfhyb{1}{}(b)=1]-\Pr[\sfhyb{2}{}(b)=1]}\leq\negl(\lambda).
\end{align}
\end{proof}

\begin{proposition}\label{prop:hyb_2_cert_sk}
If $\Sigma_{\mathsf{skcd}}$ is OT-CD secure, then 
\begin{align}
\abs{\Pr[\sfhyb{2}{}(1)=1]-\Pr[\sfhyb{2}{}(0)=1]}\leq\negl(\lambda).
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:hyb_2_cert_sk}]
We construct an adversary $\cB$ that breaks the OT-CD security of $\Sigma_{\mathsf{skcd}}$ assuming that $\cA$ can distinguish these two experiments while $\cA$ can make the challenger accept.
$\cB$ plays the experiment $\expb{\Sigma_{\mathsf{skcd}},\cB}{otsk}{cert}{del}(\secp,b')$ for some $b'\in\bit$.
First, $\cB$ simulates $\sfhyb{2}{}(b)$ by itself until $\cA_1$ makes an encryption query $\ell$ times.
Second, $\cB$ receives a challenge query $(M_0,M_1)$ from $\cA_1$, and sends the message $(M_0,M_1)$ to the challenger of $\expb{\Sigma_{\mathsf{skcd}},\cB}{otsk}{cert}{del}(\secp,b')$. 
Then, $\cB$ receives $\mathsf{cd}.\ct$ from the challenger, generates $R\la\bit^{\secp}$,
computes $\ske.\ct\la\SKE.\Enc(\ske.\sk,R)$ and generates $h$ uniformly at random.
$\cB$ sends $(h,\ske.\ct,\mathsf{cd}.\ct)$ to $\cA_1$.
Next, $\cB$ simulates $\sfhyb{2}{}(b)$ by itself until $\cA_1$ makes encryption query $u-\ell$ times.
While $\cB$ simulates $\sfhyb{2}{}(b)$, if $R=R_i$ for some $i\in[u]$ or $R_i=R_j$ for some $i,j\in[u]$ with $i\neq j$, $\cB$ aborts the experiment.
This event occurs only with negligible probability.

At some point, $\cB$ receives $\mathsf{cd}.\cert$ from $\cA_1$, and sends $\mathsf{cd}.\cert$ to the challenger.
The challenger runs $\mathsf{CD}.\Vrfy(\mathsf{cd}.\sk,\mathsf{cd}.\cert)\ra\top/\bot$.
If $\mathsf{CD}.\Vrfy(\mathsf{cd}.\sk,\mathsf{cd}.\cert)\ra\bot$, then the challenger sends $\bot$ to $\cB$.
In that case, $\cB$ aborts the experiment and outputs $\bot$.
If it is $\top$, the challenger sends $\mathsf{cd}.\sk$ to $\cB$.
In that case, $\cB$ sends $\mathsf{cd}.\sk$ to $\cA_2$,
simulates $\cA_2$, and outputs the output of $\cA_2$.
Note that $\cB$ can simulate the random oracle $H'_{R\ra \oplus \mathsf{cd}.\sk}$ given to $\cA_2$ when $\cB$ outputs $\top$.
This is because $\cB$ receives $\mathsf{cd}.\sk$ from the challenger when $\cB$ outputs $\top$.

\begin{itemize}
    \item If $b'=0$, and $\cB$ outputs $\top$, $\cB$ perfectly simulates $\sfhyb{2}{}(0)$.
    \item If $b'=1$, and $\cB$ outputs $\top$, $\cB$ perfectly simulates $\sfhyb{2}{}(1)$.
\end{itemize}
Thus, if $\cA$ can distinguish the two experiments while $\cA$ can make the challenger accept, $\cB$ breaks the OT-CD security. This completes the proof.
\end{proof}

From \cref{prop:Exp_Hyb_1_cert_sk,prop:hyb_1_hyb_2_cert_sk,prop:hyb_2_cert_sk}, \cref{thm:sk_ever_security} follows.
\end{proof}

==> Sec_Proof_wo_rom.tex <==
% !TEX root = main.tex
% !TEX spellcheck = en-US
\newcommand{\isEPR}{\algo{isEPR}}
\newcommand{\EPR}{\algo{EPR}}
\section{Proof of \cref{thm:sk_ever_security_wo_rom}}\label{sec:proof_wo_rom}

In this section, we prove \cref{thm:sk_ever_security_wo_rom}.
We note that the proof is similar to that of \cite[Theorem 3]{JACM:Unruh15}, but there are several important differences:
First, we have to consider the adversary's encryption queries since an adversary can call encryption queries unlike \cite{JACM:Unruh15}.
Second, we have to take it into account that the challenger needs to send the secret key to the adversary.
For the convenience of readers, we describe the proof. (Note that a large part of the proof is directly taken from \cite{JACM:Unruh15}.)
In order to prove \cref{thm:sk_ever_security_wo_rom}, let us introduce the property of CSS code and auxiliary propositions as follows.

\paragraph{Property of CSS code.}
%We use a CSS code to construct certified everlasting SKE and certified everlasting PKE in \cref{sec:const_ske_wo_rom,sec:const_pke_wo_rom}, respectively.

%A CSS code with parameters $q,k_1,k_2, t$ consists of two classical linear binary codes, namely a $[q,k_1]$ code $C_1$
%\footnote{A $[q,k]$ code is a code consisting of $2^k$ codewords, each of lengths $q$.
%That is, a $k$-dimensional subspace of $\bit^q={\rm GF}(2)^q$.
%}
%and a $[q,k_2]$ code such that $C_2\subseteq C_1$
%and both $C_1$ and $C_2^\bot$ can correct up to $t$ errors. We require that the parity check matrices of $C_1,C_2$ are computable in polynomial time, and that error correction can be performed in polynomial time. (Here we assume an asymptotic setting in which $C_1,C_2$ are defined for every security parameter.)

%Given two binary codes $C\subseteq D$, with a slight abuse of notation, $D/C$ denotes a representative system of the quotient $D/C$.
%{\color{red}More precisely, we assume an idempotent linear polynomial-time computable operation ``mod $C$'' on $\bit^q$ such that we have that $x$ mod $C=x'$ mod $C$ iff $x-x'\in C$ and for all codes $C\subseteq D$ that $x\in D\Rightarrow x$ mod $C\in D$ and that $x$ mod $D$ mod $C$ = $x$ mod $D$. }
%Let $D/C\seteq\{x \mbox{ mod } C:x\in D\}$.
%Let $C_1$ and $C_2$ be a CSS code with parameters $q,k_1,k_2,t$.
%Let $|\xi_{xuv}\rangle \seteq \frac{1}{\sqrt{|C_2|}}\sum_{w\in C_2}(-1)^{v\cdot w}|x\oplus w\oplus u\rangle \in \mathbb{C}^{2^q}$.
%For any $u\in\bit^q/ C_1$ and $v\in\bit^q/C_2^{\bot}$, the set of states $\{|\xi_{xuv}\rangle\}_{x\in C_1/C_2}$ defines a different quantum code (with similar properties) where $|\xi_{xuv}\rangle$ is the encoding of a word $x\in C_1/C_2$.
See~\cref{sec:quantum_computation} for CSS code. Let $\ket{\xi_{xuv}} \seteq \frac{1}{\sqrt{|C_2|}}\sum_{w\in C_2}(-1)^{v\cdot w}\ket{x\oplus w\oplus u}$.
Unruh proved several useful properties below.
\begin{proposition}[\cite{JACM:Unruh15}]\label{prop:character_sum}
$ $
\begin{itemize}
    \item [(a)] For a linear binary code $C$, if $x\in C^{\bot}$ then $\sum_{y\in C}(-1)^{x\cdot y}=|C|$,
    and if $x\notin C^{\bot}$, then $\sum_{y\in C}(-1)^{x\cdot y}=0$.\label{prop:character_sum_a}
    \item [(b)] For a linear binary code $C$ and $x\in C$, if $x=0$ then $\sum_{y\in\bit^q /C^{\bot}}(-1)^{x\cdot y}=|C|$, and if $x\neq 0$,
    then $\sum_{y\in \bit^q/C^{\bot}}(-1)^{x\cdot y}=0$.\label{prop:character_sum_b}
\end{itemize}
\end{proposition}

\begin{proposition}[\cite{JACM:Unruh15}]\label{prop:orthonormal_basis}
$\{|\xi_{xuv}\rangle \}_{x\in C_1/C_2, u\in \bit^q/C_1,v\in \bit^q/C_2^{\bot} }$ is an orthonormal basis of $\mathbb{C}^{2^q}$.
\end{proposition}

\begin{proposition}[\cite{JACM:Unruh15}]\label{prop:EPR_state}
$\frac{1}{2^{q/2}}\sum_{x,u,v}|\xi_{xuv}\rangle\otimes |\xi_{xuv}\rangle =|\widetilde{0^q0^q}\rangle$ where summation is taken over $x \in C_1/C_2$, $u\in\bit^q/C_1$ and $v\in\bit^q/C_2^{\bot}$.
\end{proposition}

%\paragraph{Error-correction and decoding operations.}
We need to define some operations related to CSS codes to describe propositions.
For $u\in\bit^q/C_1$, $v\in \bit^{q}/C_2^{\bot}$, let $U_{uv}^{EC}$ be an isometry describing error correction and decoding for the CSS code $\{|\xi_{xuv}\rangle\}_x$.
More precisely, we require that for any $u,v$ and any $f\in\bit^q$, $e\in \bit^q$ with $w(f),w(e)\leq t$ there exists a state $|\Psi\rangle$ such that for all $x$ we have $U_{uv}^{EC}X^eZ^f|\xi_{xuv}\rangle =|x\rangle\otimes |\Psi\rangle$.

Let $U_{uv}^{dec}$ be an isometry describing decoding (without error correction) for the CSS code $\{|\xi_{xuv}\rangle\}_{x}$.
More precisely, we require that for any $u\in\bit^q/C_1$, $v\in \bit^q/C_2^{\bot}$
there is a state $|\Psi\rangle$ such that for all $x\in C_1/C_2$ we have $U_{uv}^{dec}|\xi_{xuv}\rangle=|x\rangle \otimes |\Psi\rangle$.
In addition, for any $u\in \bit^q/C_1$, $v\in \bit^q/C_2^{\bot}$ and any $|\xi\rangle$ orthogonal to span $\{|\xi_{xuv}\rangle :x\in C_1/C_2\}$,
there is a $|\Psi\rangle$ such that $U_{uv}^{dec}|\xi\rangle=|\bot\rangle \otimes |\Psi\rangle$.

Now, we introduce more propositions proved by Unruh.
\begin{proposition}[\cite{JACM:Unruh15}]\label{prop:error_correcting}
Polynomial-time operations $U_{uv}^{dec}$ and $U_{uv}^{EC}$ with the properties above exists.
\end{proposition}

\begin{proposition}[\cite{JACM:Unruh15}]\label{prop:Gate_teleport}
For any $A$, we have $(A\otimes I^{\otimes q})|\widetilde{0^{q}0^{q}}\rangle=(I^{\otimes q}\otimes A^T)|\widetilde{0^q0^q}\rangle$,
where $A^T$ denotes the transpose of $A$.
\end{proposition}

\begin{proposition}[\cite{JACM:Unruh15}]\label{prop:ideal_state}
Let $\rho$ be a mixed state, and let $P$ be a projector.
Let $1-\epsilon\seteq\Tr(P\rho)$.
Then there exists a mixed state $\rho^{ideal}$ such that 
\begin{itemize}
    \item $\frac{1}{2}\parallel\rho -\rho^{ideal} \parallel_{\tr}\leq \sqrt{\epsilon}$.
    \item $\rho^{ideal}$ is a mixture over ${\rm im}P$.
    (I.e., $\rho=\sum_i p_i|\Psi_i\rangle\langle \Psi_i|$ for quantum states $|\Psi_i\rangle\in$ ${\rm im}P$
    and $p_i\geq 0$ and $\sum p_i =1$.)
\end{itemize}
\end{proposition}

\begin{proposition}[\cite{JACM:Unruh15}]\label{prop:Detect_error}
Fix integers $p,q,t\geq 1$.
Let $x^0,x^1\in \bit^{p+q}$ such that $w(x^0)\geq t+1$ or $w(x^1)\geq t+1$.
Consider the following process: Select uniformly $Q=\{Q_1,Q_2,\cdots ,Q_p\}\in [p+q]_p$.
Select uniformly $B=B_1B_2\cdots B_p\in\bit^p$.
Let $P(x)\seteq \Pr[\nexists i\in\{1,2,\cdots,p\}|x_{Q_i}^{B_i}=1]$.

Then $P(x)\leq 3\sqrt{p}(1-\frac{p}{2(p+q)})^{t+1}$.
\end{proposition}

We use propositions above in the proof below.
\begin{proof}[Proof of \cref{thm:sk_ever_security_wo_rom}]
To prove \cref{thm:sk_ever_security_wo_rom}, we define the following measurements.

\begin{itemize}
\item The measurement $M_R\seteq \{P_r\}_{r\in\bit^{p}}$, where $P_r\seteq |r\rangle\langle r|\otimes I^{\otimes q}$, measures the first $p$-qubits of a $(p+q)$-qubit register in the computational basis.

\item The measurement $M_{UV} \seteq \{P_{uv}\}_{u,v}$, where $P_{uv}\seteq \sum_{x\in C_1/C_2}I^{\otimes p}\otimes |\xi_{xuv}\rangle \langle \xi_{xuv}|$, measures the value $u,v$ in a $(p+q)$-qubit state of the form $|r\rangle\otimes |\xi_{xuv}\rangle$.

\item The measurement $M_{X}^{uv} \seteq \{P_{x}^{uv}\}_{x\in C_1/C_2\cup \{\bot\}}$, where $P_{x}^{uv}\seteq I^{\otimes p}\otimes |\xi_{xuv}\rangle\langle\xi_{xuv}|$ and $P_{\bot}^{uv}=1-\sum_{x\in C_1/C_2} P_x^{uv}$, measures the value $x$ in a $(p+q)$-qubit state of the form $|r\rangle \otimes |\xi_{xuv}\rangle$.
$M_{X}^{uv}$ is parameterized by $u$ and $v$ and if the parameters $u,v$ do not match, the outcome is $\bot$.

\item The measurements $M_{UV}$ and $M_X^{uv}$ are projective measurements since the $|\xi_{xuv}\rangle$ forms an orthogonal basis by~\cref{prop:orthonormal_basis}.
\end{itemize}

We also define
$
P_t^{\EPR}\seteq \sum_{f,e\in\bit^q\\,w(f),w(e)\leq t}|\widetilde{fe}\rangle\langle \widetilde{fe}|
$ and $P_{C_1/C_2}^{\EPR}\seteq \frac{1}{|C_1/C_2|}\left(\sum_{x\in C_1/C_2}|xx\rangle\right)\allowbreak \left(\sum_{x'\in C_1/C_2}\langle x'x'|\right)$.
%\taiga{Note that, in Unruh's paper, $P_{C_1/C_2}^{\EPR}$ is defined by $\sum_{x\in C_1/C_2}|x\rangle\langle x|\otimes |x\rangle\langle x|$. But, I think that he should define $P_{C_1/C_2}^{\EPR}$ as $\frac{1}{|C_1/C_2|}\left(\sum_{x\in C_1/C_2}|xx\rangle\right)\left(\sum_{x'\in C_1/C_2}\langle x'x'|\right)$. In his definition, \cref{prop:Hyb_4_Hyb_5_revoc} fails.}
%\ryo{I edited this measurement part.}\taiga{Thank you. This looks OK}

For clarity, we describe how the experiment works against an adversary $\cA\coloneqq (\cA_1,\cA_2)$ consisting of any QPT adversary $\cA_1$ and any unbounded adversary $\cA_2$.

\begin{description}
\item[$\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)$:] This is the original experiment.

\begin{enumerate}   
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.\label{step:message_generation}
    \item The challenger generates $u\la\bit^{q}/C_1$ and $r\la\bit^{p}$.
    \item The challenger generates $x\la C_1/C_2$.
    \item The challenger generates $w\la C_2$.
    \item The challenger initializes a register $X\seteq U_Q^\dagger (H^B\otimes I^{\otimes q})(|r\rangle \otimes |x\oplus w\oplus u\rangle)$.
    \item The challenger computes $h\seteq m_b\oplus x\oplus y$. 
    \item The challenger computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(B,Q,r,y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$ and sends $\ske.\sk$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
What we have to prove is that  
\begin{align}
    \advd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda)\seteq
\left|\Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,0)=1]-
\Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,1)=1]\right|\leq \negl(\lambda).
\end{align}
We define the following sequence of hybrids.
We highlight changes between games in blue.
\end{description}
\begin{description}
\item[$\sfhyb{1}{}(b)$:] $ $
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item The challenger generates $u\la\bit^{q}/C_1$ and $r\la\bit^{p}$.
    \item The challenger generates $x\la C_1/C_2$ {\color{blue}and $\hat{x}\la C_1/C_2$.}
    \item The challenger generates $w\la C_2$.
    \item The challenger initializes a register $X\seteq U_Q^\dagger (H^B\otimes I^{\otimes q})(|r\rangle \otimes |x\oplus w\oplus u\rangle)$.
    \item The challenger computes $h\seteq {\color{blue}\hat{x}}\oplus y$.
    \item The challenger generates computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(B,Q,r,y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$,
    measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$ and sends $\ske.\sk$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$ {\color{blue}and $m_b\oplus x= \hat{x}$}, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\item[$\sfhyb{2}{}(b)$:] $ $
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item The challenger generates $u\la\bit^{q}/C_1$ and $r\la\bit^{p}$.
    \item The challenger generates $x\la C_1/C_2$ and $\hat{x}\la C_1/C_2$.
    \item The challenger generates {\color{blue}\sout{$w\la C_2$}} {\color{blue}$v\la \bit^{q}/C_2^\bot$}.
    \item The challenger initializes a register
    $X\seteq U_Q^\dagger (H^B\otimes I^{\otimes q})(|r\rangle \otimes {\color{blue}|\xi_{xuv}\rangle})$.
    \item The challenger computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(B,Q,r,y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$ and sends $\ske.\sk$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$ and $m_b\oplus x= \hat{x}$, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\item [$\sfhyb{3}{}(b)$:]$ $\label{game:Hyb_3_revoc}
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item {\color{blue}\sout{The challenger generates $u\la\bit^{q}/C_1$ and $r\la\bit^{p}$.}}
    \item {\color{blue}\sout{The challenger generates $x\la C_1/C_2$ and $\hat{x}\la C_1/C_2$.}}
    \item {\color{blue}\sout{The challenger generates $v\la \bit^{q}/C_2^\bot$.}}
    \item {\color{blue}\sout{The challenger initializes a register
    $X\seteq U_Q^\dagger (H^B\otimes I^{\otimes q})(|r\rangle \otimes {\color{blue}|\xi_{xuv}\rangle})$.}}
    \item {\color{blue} The challenger initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.}
    \item {\color{blue} The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.}
    \item {\color{blue} The challenger measures $Y$ using $M_{UV}$, and obtains the outcomes $(u,v)$.}
    \item {\color{blue} The challenger measures $Y$ using $M_X^{uv}$, and obtains the outcome $x$.}
    \item {\color{blue} The challenger measures $Y$ using $M_R$, and obtains the outcome $r$.}
    \item The challenger {\color{blue} generates $\hat{x}\la C_1/C_2$} and computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(B,Q,r,y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$ and sends $\ske.\sk$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$ and $m_b\oplus x= \hat{x}$, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\item[$\sfhyb{4}{}(b)$:] $ $\label{game:Hyb_4_revoc}
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item The challenger initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.
    \item The challenger measures $Y$ using $M_{UV}$, and obtains the outcomes $(u,v)$.
    \item {\color{blue}\sout{The challenger measures $Y$ using $M_X^{uv}$, and obtains the outcome $x$.}}
    \item The challenger measures $Y$ using $M_R$, and obtains the outcome $r$.
    \item \label{step:8_Hyb_4_revoc}The challenger generates $\hat{x}\la C_1/C_2$ and computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(B,Q,r,y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item \label{step:12_Hyb_4_revoc} The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$ and sends $\ske.\sk$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item {\color{blue} The challenger measures $Y$ using $M_X^{uv}$, and obtains the outcome $x$.}
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$ and $m_b\oplus x= \hat{x}$, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}

\item[$\sfhyb{5}{}$:] $ $
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item The challenger initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.
    \item The challenger measures $Y$ using $M_{UV}$, and obtains the outcomes $(u,v)$.
    \item The challenger measures $Y$ using $M_R$, and obtains the outcome $r$.
    \item The challenger generates $\hat{x}\la C_1/C_2$ and computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(B,Q,r,y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item \label{step:11_Hyb_5_revoc}The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$ and sends $\ske.\sk$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$ and sends $\bot$ to $\cA_2$.
    \item {\color{blue} The challenger operates $I^{\otimes p}\otimes U_{uv}^{EC}$ on $X$ and $I^{\otimes p}\otimes U_{uv}^{dec}$ on $Y$.
    The challenger measures $X'Y'$ using $P_{C_1/C_2}^{\EPR}$, and obtains the outcome $\isEPR$.
    (Here $X',Y'$ refer to the last $q$ qubits of $X,Y$, respectively.)}
    %\taiga{Note that, in Unruh's paper, he writes ``the challenger measures $XY$ using $P_{C_1/C_2}^{\EPR}$'' instead of $X'Y'$. But, I think this is his mistake.}
    \item {\color{blue} If the challenger outputs $\top$, then the output of the experiment is $\isEPR$.
    Otherwise, the output of the experiment is $\bot$.}
    \item {\color{blue} \sout{The challenger measures $Y$ using $M_X^{uv}$, and obtains the outcome $x$.}}
    \item {\color{blue}\sout{$\cA_2$ outputs $b'$.}}
    \item {\color{blue}\sout{If the challenger outputs $\top$ and $m_b\oplus x= \hat{x}$, then the output of the experiment is $b'$.
    Otherwise, the output of the experiment is $\bot$.}}
    \end{enumerate}
\item[$\sfhyb{6}{}$:] $ $
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item The challenger initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.
    \item The challenger measures $Y$ using $M_{UV}$, and obtains the outcomes $(u,v)$.
    \item The challenger measures $Y$ using $M_R$, and obtains the outcome $r$.
    \item The challenger generates $\hat{x}\la C_1/C_2$ and computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(B,Q,r,y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item \label{step:11_Hyb_6_revoc}The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$ \sout{{\color{blue} and sends $\ske.\sk$ to $\cA_2$}}.
    Otherwise, the challenger outputs $\bot$ \sout{{\color{blue} and sends $\bot$ to $\cA_2$}}.
    \item The challenger operates $I^{\otimes p}\otimes U_{uv}^{EC}$ on $X$ and $I^{\otimes p}\otimes U_{uv}^{dec}$ on $Y$.
    The challenger measures $X'Y'$ using $P_{C_1/C_2}^{\EPR}$, and obtains the outcome $\isEPR$.
    (Here $X',Y'$ refer to the last $q$ qubits of $X,Y$, respectively.)
    \item If the challenger outputs $\top$, then the output of the experiment is $\isEPR$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\item[$\sfhyb{7}{}$:] $ $
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item The challenger initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.
    \item The challenger measures $Y$ using $M_{UV}$, and obtains the outcomes $(u,v)$.
    \item The challenger measures $Y$ using $M_R$, and obtains the outcome $r$.
    \item The challenger generates $\hat{x}\la C_1/C_2$ and computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger generates {\color{blue} $\hat{B}\la \bit^{p}$, $\hat{Q}\leftarrow[p+q]_{p}$ and $\hat{r}\la\bit^{p}$}, and computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,({\color{blue}\hat{B},\hat{Q},\hat{r},y}))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item \label{step:11_Hyb_7_revoc}The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$.
    Otherwise, the challenger outputs $\bot$.
    \item The challenger operates $I^{\otimes p}\otimes U_{uv}^{EC}$ on $X$ and $I^{\otimes p}\otimes U_{uv}^{dec}$ on $Y$.
    The challenger measures $X'Y'$ using $P_{C_1/C_2}^{\EPR}$, and obtains the outcome $\isEPR$.
    (Here $X',Y'$ refer to the last $q$ qubits of $X,Y$, respectively.)
    \item If the challenger outputs $\top$, then the output of the experiment is $\isEPR$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\item[$\sfhyb{8}{}$:] $ $
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates {\color{blue}\sout{$B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$,}} $y\la C_1/C_2$.
    \item The challenger initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.
    \item {\color{blue}\sout{The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.}}
    \item {\color{blue}\sout{The challenger measures $Y$ using $M_{UV}$, and obtains the outcomes $(u,v)$.}}
    \item {\color{blue}\sout{The challenger measures $Y$ using $M_R$, and obtains the outcome $r$.}}
    \item The challenger generates $\hat{x}\la C_1/C_2$ and computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger generates $\hat{B}\la \bit^{p}$, $\hat{Q}\leftarrow[p+q]_{p}$ and $\hat{r}\la\bit^{p}$, and computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(\hat{B},\hat{Q},\hat{r},y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item {\color{blue}The challenger generates $B\la \bit^{p}$ and $Q\la[p+q]_{p}$.}
    \item {\color{blue}The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.}
    \item \label{step:11_Hyb_8_revoc}The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$.
    {\color{blue}The challenger measures the register $Y$ using $M_R$, obtains the outcome $r$,}
    measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$.
    Otherwise, the challenger outputs $\bot$.
    \item \label{step:Hyb_8}{\color{blue}The challenger measures $Y$ using $M_{UV}$ and obtains the outcomes $u,v$.}
    \item The challenger operates $I^{\otimes p}\otimes U_{uv}^{EC}$ on $X$ and $I^{\otimes p}\otimes U_{uv}^{dec}$ on $Y$.
    The challenger measures $X'Y'$ using $P_{C_1/C_2}^{\EPR}$, and obtains the outcome $\isEPR$.
    (Here $X',Y'$ refer to the last $q$ qubits of $X,Y$, respectively.)
    \item If the challenger outputs $\top$, then the output of the experiment is $\isEPR$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\item[$\sfhyb{9}{}$:] $ $
\begin{enumerate}
    \item The challenger computes $\ske.\sk\la\SKE.\keygen(1^\secp)$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ chooses $(m_0,m_1)\leftarrow \cM^2$, and sends $(m_0,m_1)$ to the challenger.
    \item The challenger generates $y\la C_1/C_2$.
    \item The challenger initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.
    \item The challenger generates $\hat{x}\la C_1/C_2$ and computes $h\seteq \hat{x}\oplus y$. 
    \item The challenger generates $\hat{B}\la \bit^{p}$, $\hat{Q}\leftarrow[p+q]_{p}$ and $\hat{r}\la\bit^{p}$, and computes $\ske.\ct\la \SKE.\Enc(\ske.\sk,(\hat{B},\hat{Q},\hat{r},y))$.
    \item The challenger sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item The challenger receives an encryption query $m$ from $\cA_1$, computes $(\vk,\ct)\la\Enc(\sk,m)$, and sends $(\vk,\ct)$ to $\cA_1$. This process can be repeated polynomially many times.
    \item $\cA_1$ sends back the register $X$ to the challenger and sends its internal state to $\cA_2$.
    \item The challenger generates $B\la \bit^{p}$ and $Q\la[p+q]_{p}$.
    \item The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.
    \item \label{step:11_Hyb_9_revoc}The challenger operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$.
    The challenger measures the register $Y$ using $M_R$, obtains the outcome $r$,
    measures the register $X$ using $M_R$ and obtains the outcome $r'$.
    If $r=r'$, the challenger outputs $\top$.
    Otherwise, the challenger outputs $\bot$.
    \item {\color{blue}\sout{The challenger measures $Y$ using $M_{UV}$ and obtains the outcomes $u,v$.}}
    \item {\color{blue}\sout{The challenger operates $I^{\otimes p}\otimes U_{uv}^{EC}$ on $X$ and $I^{\otimes p}\otimes U_{uv}^{dec}$ on $Y$.
    The challenger measures $X'Y'$ using $P_{C_1/C_2}^{\EPR}$, and obtains the outcome $\isEPR$.
    (Here $X',Y'$ refer to the last $q$ qubits of $X,Y$, respectively.)}}
    \item {\color{blue} The challenger measures $X'Y'$ using $P_t^{\EPR}$, and obtains the outcome $\isEPR$.}
    \item If the challenger outputs $\top$, then the output of the experiment is $\isEPR$.
    Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\end{description}

\paragraph{Notation.} In the following,
let us denote the event as $ok=1$ that the challenger outputs $\top$
and 
let us denote the event as $ok=0$ that the challenger outputs $\bot$ in the security experiment.
$\Pr[X|Y:Z]$ is the probability that the event $X$ occurs conditioned on that the event $Y$ occurs in the experiment $Z$.
\begin{proposition}\label{prop:Exp_Hyb_1_revoc}
For $b\in\bit$, it holds that
\begin{align}
\Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)=1]=|C_1/C_2|\Pr[\sfhyb{1}{}(b)=1].
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:Exp_Hyb_1_revoc}]
For all $\underline{x},\underline{\hat{x}},\underline{m_0},\underline{m_1}$, it holds that
\begin{align}
&\Pr[\sfhyb{1}{}(b)=1|(x,\hat{x},m_0,m_1)=(\underline{x},\underline{\hat{x}},\underline{m_0},\underline{m_1}):\sfhyb{1}{}(b)]\\
&=
\begin{cases}
    \Pr[1\la\cA_2\wedge ok=1|(x,m_0,m_1)=(\underline{x},\underline{m_0},\underline{m_1}):
    \expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)]~~~&(m_b\oplus x=\underline{\hat{x}})\\
    0~~~&(m_b\oplus x\neq\underline{\hat{x}}).
    \end{cases}
\end{align}
%\ryo{In probabilities, both $:$ and $|$ are used for conditional probability? Or using $:$ to denote ``in the Game XX''? It is confusing.}
%\taiga{I use : to denote ``in the Game XX''.}
%\ryo{Then, please explicitly explain the notations at some point since $:$ is sometimes used as conditional probability in cryptography.}
Since $\sfhyb{1}{}(b)$ and $\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)$ are identical before step \ref{step:message_generation}, it holds that
\begin{align}
\Pr[(m_0,m_1)=(\underline{m_0},\underline{m_1}):\sfhyb{1}{}(b)]=\Pr[(m_0,m_1)=(\underline{m_0},\underline{m_1}):\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)].
\end{align}
Thus, we have
\begin{align}
    &|C_1/C_2|\Pr[\sfhyb{1}{}(b)=1]\\
    &=\sum_{\underline{x},\underline{\hat{x}},\underline{m_0},\underline{m_1}\in C_1/C_2}\frac{1}{|C_1/C_2|}\Pr[\sfhyb{1}{}(b)=1|(x,\hat{x},m_0,m_1)=(\underline{x},\underline{\hat{x}},\underline{m_0},\underline{m_1}):\sfhyb{1}{}(b)]\\
    &\hspace{4cm}\cdot\Pr[(m_0,m_1)=(\underline{m_0},\underline{m_1}):\sfhyb{1}{}(b)]\\
    &=\sum_{\underline{x},\underline{m_0},\underline{m_1}\in C_1/C_2}\frac{1}{|C_1/C_2|}\Pr[1\la \cA_2\wedge ok=1 |(x,m_0,m_1)=(\underline{x},\underline{m_0},\underline{m_1}):\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)]\\
    &\hspace{4cm}\cdot\Pr[(m_0,m_1)=(\underline{m_0},\underline{m_1}):\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)]\\
    &=\Pr[1\la\cA_2\wedge ok=1:\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,b)]\\
    &=\Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cp}(\lambda,b)=1].
\end{align}
\end{proof}

\begin{proposition}\label{prop:Hyb_1_Hyb_2_revoc}
For $b\in\bit$, it holds that
\begin{align}
    \Pr[\sfhyb{1}{}(b)=1]=\Pr[\sfhyb{2}{}(b)=1].
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_1_Hyb_2_revoc}]
In $\sfhyb{1}{}$ and $\sfhyb{2}{}$, $w$ and $v$ are never used except in the construction of the state $|x\oplus w\oplus u\rangle$ and $|\xi_{xuv}\rangle$, respectively.
We will prove that for all $x$ and $u$, $\ket{x\oplus w\oplus u}$ and $\ket{\xi_{xuv}}$ are indistinguishable by any quantum circuit for random $v,w$ to prove \cref{prop:Hyb_1_Hyb_2_revoc}.
More formally, we will prove that $\rho_{1}^{xu}=\rho_2^{xu}$ where $\rho_1^{xu}=\sum_{w\in C_2}\frac{1}{|C_2|}|x\oplus w\oplus u\rangle \langle x\oplus w\oplus u|$
and $\rho_2^{xu}=\sum_{v\in\bit^q/C_2^{\bot}}\frac{1}{|\bit^q/C_2^{\bot}|}|\xi_{x,u,v}\rangle\langle \xi_{x,u,v}|$.
We can show this equation as follows.
\begin{align}
    \rho_{2}^{xu}&=\sum_{w_1,w_2\in C_2}\frac{1}{|C_2|}\left(\sum_{v\in \bit^q/C_2^{\bot}}\frac{1}{|\bit^q/C_2^{\bot}|}(-1)^{v\cdot(w_1\oplus w_2)}\right) |x\oplus w_1\oplus u\rangle\langle x\oplus w_2\oplus u|\\
                 &= \sum_{w\in C_2}\frac{1}{|C_2|} |x\oplus w\oplus u\rangle\langle x\oplus w\oplus u|=\rho_1^{xu}. 
\end{align}
In the first equation, we have used the definition of $|\xi_{xuv}\rangle$.
In the second equation, we have used \cref{prop:character_sum_b} of $(b)$.
\end{proof}

\begin{proposition}\label{prop:Hyb_2_Hyb_3_revoc}
For $b\in\bit$, it holds that
\begin{align}
\Pr[\sfhyb{2}{}(b)=1]=\Pr[\sfhyb{3}{}(b)=1].
\end{align}
\end{proposition}

\begin{proof}[Proof of \cref{prop:Hyb_2_Hyb_3_revoc}]
We show two facts to prove \cref{prop:Hyb_2_Hyb_3_revoc}.
The first is that when initializing $XY$ with $|\widetilde{0^{p+q}0^{p+q}}\rangle$, applying $(H_B\otimes I^{\otimes q})U_Q$ on $Y$, and performing the measurements $M_{UV}$, $M^{uv}_X$, and $M_R$ on $Y$,
then the outcomes $u,v,x,r$ will be uniformly distributed over their respective domains.
The second is that the post-measurement state in $X$ is $U_Q(H^B\otimes I^{\otimes q})(|r\rangle\otimes |\xi_{xuv}\rangle)$.

We define $\ket{\Psi_{xruv}}\seteq (I^{\otimes p+q}\otimes P_rP^{uv}_xP_{uv}(H^B\otimes I^{\otimes q})U_Q)|\widetilde{0^{p+q}0^{p+q}}\rangle$.
By this definition, the probability of obtaining the measurement outcomes $x,r,u,v$ in $\sfhyb{3}{}(b)$ is $\||\Psi_{xruv}\rangle\|^2$. 
The post measurement state is $|\Psi_{xruv}\rangle/\| |\Psi_{xruv}\rangle \|$.

It holds that
\begin{align}
    |\Psi_{xruv}\rangle &=(I^{\otimes p+q}\otimes P_rP_x^{uv}P_{uv})(I^{\otimes p+q}\otimes (H^B\otimes I^{\otimes q})U_Q)|\widetilde{0^{p+q}0^{p+q}}\rangle\\
                        &=(I^{\otimes p+q}\otimes P_rP_{x}^{uv}P_{uv})(U_Q^{\dagger}(H^B\otimes I^{\otimes q})\otimes I^{\otimes p+q})|\widetilde{0^{p+q}0^{p+q}}\rangle\\
                        &=(U_{Q}^{\dagger}(H^B\otimes I^{\otimes q})\otimes I^{\otimes p+q})(I^{\otimes p+q}\otimes P_rP_x^{uv}P_{uv})|\widetilde{0^{p+q}0^{p+q}}\rangle\\
                        &=(U_Q^{\dagger}(H^B\otimes I^{\otimes q})\otimes I^{\otimes p+q})(P_rP_x^{uv}P_{uv}\otimes I^{\otimes p+q})|\widetilde{0^{p+q}0^{p+q}}\rangle\\
                        &=(U_Q^{\dagger}(H^B\otimes I^{\otimes q})\otimes I^{\otimes p+q})(P_rP_x^{uv}P_{uv}\otimes I^{\otimes p+q})2^{-p/2-q/2}\sum_{r,x,u,v}|r\rangle|\xi_{xuv}\rangle|r\rangle |\xi_{xuv}\rangle\\
                        &=2^{-p/2-q/2}U_Q^{\dagger}(H^B\otimes I^{\otimes q})|r\rangle |\xi_{xuv}\rangle \otimes |r\rangle |\xi_{xuv}\rangle,
\end{align}
where the summation in the fifth equation is taken over $r\in\bit^p$, $x \in C_1/C_2$, $u\in\bit^q/C_1$ and $v\in\bit^q/C_2^{\bot}$.
In the second equation and in the fourth equation, we have used \cref{prop:Gate_teleport}.
In the fifth equation, we have used \cref{prop:EPR_state}.
In the sixth equation, we have used that $|r\rangle |\xi_{xuv}\rangle$ are orthogonal, and that  $P_rP_x^{uv}P_{uv}$ is a projector onto $|r\rangle|\xi_{xuv}\rangle$.

By the equation above, $\||\Psi_{xruv}\rangle\|$ is $2^{-p-q}$.
Therefore, the probability distribution of the measurement outcomes $x,r,u,v$ is uniformly distributed.
The post-measurement state in $X$ is $U_Q^{\dagger}(H^B\otimes I^{\otimes q})|r\rangle |\xi_{xuv}\rangle$.
\end{proof}



\begin{proposition}\label{prop:Hyb_3_Hyb_4_revoc}
For $b\in\bit$, it holds that
\begin{align}
    \Pr[\sfhyb{3}{}(b)=1]=\Pr[\sfhyb{4}{}(b)=1].
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_3_Hyb_4_revoc}]
The measurement $M_X^{uv}$ on $Y$ is deferred in $\mathsf{Hyb}_4(b)$. However, $M_X^{uv}$ commutes with $M_R$ because it operates on a different part of the register $Y$.
It also commutes with steps \ref{step:8_Hyb_4_revoc}-\ref{step:12_Hyb_4_revoc} in $\mathsf{Hyb}_4 (b)$ because the latter do not operate on $Y$.
\end{proof}

\begin{proposition}\label{prop:Hyb_4_Hyb_5_revoc}
Let $\epsilon\seteq \Pr[\sfhyb{5}{}=0]$.
Then it holds that
\begin{align}
    \abs{\Pr[\sfhyb{4}{}(0)=1]-\Pr[\sfhyb{4}{}(1)=1]}\leq \sqrt{\epsilon}.
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_4_Hyb_5_revoc}]
For any $\hat{x}$, $u$, $v$, let $\rho_{\hat{x}uv}$ be the state in $\sfhyb{5}{}$ after step~\ref{step:11_Hyb_5_revoc}
conditioned on the variables $\hat{x},u,v,ok$ in the game taking the values $\hat{x},u,v,1$.
Let $\Pr_{\hat{x}uv}$ be the probability of $\hat{x},u,v, ok$ in the game taking the values $\hat{x},u,v,1$.

Hybrid games $\sfhyb{4}{}$ and $\sfhyb{5}{}$ are identical until step~\ref{step:11_Hyb_5_revoc}, and $\rho_{\hat{x}uv}$ and $\Pr_{\hat{x}uv}$ also refer to $\mathsf{Hyb}_4$.
Thus, for $b\in\bit$ it holds that 
\begin{align}
    &\Pr[\sfhyb{4}{}(b)=1]\\
    &=\sum_{\substack{\hat{x}\in C_1/C_2,u\in \bit^q/C_1\\ v\in\bit^q/C_2^{\bot}} }{\rm Pr}_{\hat{x}uv}\cdot \Pr[b'=1|\mbox{start with $\rho_{\hat{x}uv}$, $x\la $measure $Y$ with $M_X^{uv}$, $b'\la \cB(x\oplus m_b\oplus \hat{x})$}],
\end{align}
where $\cB(x')$ runs the following procedure: ``If $x'=0$, runs $b'\la\cA_2$. Else, $\cB(x')$ outputs $\bot$.''

To define a measurement $M_X$ for the result of decoding with $U_{uv}^{dec}$ in the computational basis, we define $P_x$ to be the projector upon span$\{|r\rangle |x\rangle |\Psi\rangle:r\in\bit^p,|\Psi\rangle\mbox{ arbitrary}\}$.
We also define $P_{\bot}\seteq I-\sum_{x\in C_1/C_2}P_x$. 
Then, we set $M_X \seteq \{P_x\}_{x\in C_1/C_2 \cup \{\bot\}}$.

We can verify that for all $r,x,u,v,x',u',v'$, and suitable $\ket{\Psi}$,
\begin{align}
    &P_x(I^{\otimes p}\otimes U_{uv}^{dec})|r\rangle |\xi_{xuv}\rangle =|r\rangle|x\rangle \otimes |\Psi\rangle=(I^{\otimes p}\otimes U_{uv}^{dec})|r\rangle |\xi_{xuv}\rangle
    =(I^{\otimes p}\otimes U_{uv}^{dec})P_{x}^{uv}|r\rangle |\xi_{xuv}\rangle\\
    &P_x(I^{\otimes p}\otimes U_{uv}^{dec})|r\rangle |\xi_{x'u'v'}\rangle=0=(I^{\otimes p}\otimes U_{uv}^{dec})P_{x}^{uv}|r\rangle |\xi_{x'u'v'}\rangle\hspace{1.5cm}(x,u,v)\neq(x',u',v')\\
    &P_{\bot}(I^{\otimes p}\otimes U_{uv}^{dec}) |r\rangle |\xi_{xuv}\rangle=0=(I^{\otimes p}\otimes U_{uv}^{dec})P_{\bot}^{uv}|r\rangle |\xi_{xuv}\rangle\\
    &P_{\bot}(I^{\otimes p}\otimes U_{uv}^{dec})|r\rangle |\xi_{x'u'v'}\rangle =|r\rangle |\bot\rangle \otimes |\Psi\rangle =(I^{\otimes p}\otimes U_{uv}^{dec})P_{\bot}^{uv}|r\rangle |\xi_{x'u'v'}\rangle\hspace{1.5cm} (u,v)\neq (u',v')
\end{align}
We can derive $P_x(I^{\otimes p}\otimes U_{uv}^{dec})=(I^{\otimes p}\otimes U_{uv}^{dec})P_x^{uv}$
for any $u,v$ and $x\in C_1/C_2\cup\{\bot\}$ from the equations above since the $\ket{\xi_{xuv}}$ form a basis.
This means that applying $I^{\otimes p}\otimes U_{uv}^{dec}$ and then measuring with $M_X$ is equivalent to measuring with $M_X^{uv}$ and then applying $(I^{\otimes p}\otimes U_{uv}^{dec})$.
To conisder the difference between two games, we let $\rho_{\hat{x}uv}^*$ be the state resulting from applying $I^{\otimes p}\otimes U_{uv}^{EC}\otimes I^{\otimes p}\otimes U_{uv}^{dec}$ to $\rho_{\hat{x}uv}$ in $XY$.
Then, the following four variations of games have the same probability of $b'=1$:
\begin{itemize}
    \item Start with $\rho_{\hat{x}uv}$, obtaining $x$ by measuring $Y$ with $M_X^{uv}$, $b'\la\cB(x\oplus m_i\oplus \hat{x})$.
    \item Start with $\rho_{\hat{x}uv}$, {\color{blue} operate $(I^{\otimes p}\otimes U_{uv}^{EC})$ on $X$,} obtaining $x$ by measuring $Y$ with $M_{X}^{uv}$, {\color{blue} operate $(I^{\otimes p}\otimes U_{uv}^{dec})$ on $Y$,}
    $b'\la\cB(x\oplus m_i\oplus\hat{x})$. \,\,\,\,\,\,\,(Use that $\cB$ does not access $X$ and $Y$. )
    \item Start with $\rho_{\hat{x}uv}$, operate $(I^{\otimes p}\otimes U_{uv}^{EC})$ on $X$, {\color{blue}operate $(I^{\otimes p}\otimes U_{uv}^{dec})$ on $Y$, obtaining $x$ by measuring $Y$ with $M_X$,} $b'\la\cB(x\oplus m_i\oplus \hat{x})$.\,\,\,\,\,\,\,(Use that $(I^{\otimes p}\otimes U_{u,v}^{dec})M_X$ is equivalent to $M_X^{uv}(I^{\otimes p}\otimes U_{u,v}^{dec})$.)
    \item Start with {\color{blue}$\rho^*_{\hat{x}uv}$, \sout{operate $(I^{\otimes p}\otimes U_{uv}^{EC})$ on $X$,} \sout{operate $(I^{\otimes p}\otimes U_{uv}^{dec})$ on $Y$,}} obtaining $x$ by measuring $Y$ with $M_X$, $b'\la\cB(x\oplus m_i\oplus \hat{x})$.
\end{itemize}

Thus, for $b\in\bit$ it holds that
\begin{align}
    &\Pr[\sfhyb{4}{}(b)=1]\\
    &=\sum_{\substack{\hat{x}\in C_1/C_2,u\in\bit^q/C_1 \\v\in\bit^q/C_2^{\bot}}}{\rm Pr}_{\hat{x}uv}\cdot \Pr[b'=1|\mbox{start with $\rho_{\hat{x}uv}^*$, $x\la $measure $Y$ with $M_X$, $b'\la \cB(x\oplus m_b\oplus \hat{x})$}].
\end{align}
\ryo{In this case, not $|$ but $:$? It seems the contents after $|$ desctibe a game.}
\taiga{I should use $:$ instead of $:$.}
\ryo{What does ``$x\la$ measure'' means? This notation appears in many places.}
\taiga{``$x\la$ measure Y with $M_X$'' means that $x$ is obtained by measuring register $Y$ with $M_X$. }
\ryo{Where is the definition?}
For simplicity, let us define 
$
\mathsf{Succ}_{\hat{x}uv}^b\seteq  \Pr[b'=1|\mbox{start with $\rho_{\hat{x}uv}^*$, $x\la$ measure $Y$ with $M_X$, $b'\la \cB(x\oplus m_b\oplus \hat{x})$}]
$. 


Furthermore, it holds that
\begin{align}
    \epsilon\seteq\Pr[\sfhyb{5}{}=0]=\sum_{\substack{\hat{x}\in C_1/C_2,u\in\bit^q/C_1 \\v\in\bit^q/C_2^{\bot}}}{\rm Pr}_{\hat{x}uv}\cdot\Tr[\left((1-P_{C_1/C_2}^{\EPR})\otimes I\right)\rho_{\hat{x}uv}^*]
\end{align}
where $I$ is the identity on all registers except for $X',Y'$.
For simplicity, let us define
$
\epsilon_{\hat{x}uv}\seteq \Tr[\left((1-P_{C_1/C_2}^{\EPR})\otimes I\right)\rho_{\hat{x}uv}^*].
$
Since 
$
\Tr[(P_{C_1/C_2}^{\EPR}\otimes I)\rho_{\hat{x}uv}^{*}]=1-\epsilon_{\hat{x}uv}
$
by definition of $\epsilon_{\hat{x}uv}$, \cref{prop:ideal_state} implies there exists a state $\rho_{\hat{x}uv}^{ideal}$ such that
\begin{align}
    \frac{1}{2}\parallel \rho_{\hat{x}uv}^*-\rho_{\hat{x}uv}^{ideal}\parallel_{\tr}\leq \sqrt{\epsilon_{\hat{x}uv}}
\end{align}
and
\begin{align}
    \rho^{ideal}_{\hat{x}uv} \mbox{ is a mixture over im}(P_{C_1/C_2}^{\EPR}\otimes I).
\end{align}
\ryo{What is ``im''?}\taiga{imM is the image of an operator $M$.}
\ryo{Where is the definition?}
The above equation\ryo{Where is an equation? ``$ \rho^{ideal}_{\hat{x}uv}$ is a mixture over $im(P_{C_1/C_2}^{\EPR}\otimes I)$'' is a sentence.}\taiga{the above fact} implies that $\rho_{\hat{x}uv}^{ideal}$ is of the form
$
\frac{1}{|C_1/C_2|}\left(\sum_{x\in C_1/C_2}|xx\rangle\right)\left(\sum_{x'\in C_1/C_2}\langle x'x'|\right)\otimes \rho_{rest}
$.
Note also that in the game, `` start with $\rho_{\hat{x}uv}^{ideal}$, $x\la$ measure $Y$ with $M_X$, $b'\la \cB(x\oplus m_b\oplus \hat{x})$'', the adversary $\cB(x\oplus m_b\oplus \hat{x})$ operates only on $\rho_{rest}$.\ryo{What is $\rho_{rest}$?}\taiga{$\rho_{rest}$ is the quantum state $\rho_{\hat{x}uv}^{ideal}$ without the register $X$ and $Y$.}
This means that $x$ is uniformly distributed on $C_1/C_2$ and independent of the initial state of $\cB(x\oplus m_b\oplus \hat{x})$. 
Thus, the output $b'$ by $\cB(x\oplus m_b\oplus \hat{x})$ is independent of $m_i$, and we have
\begin{align}
    &\Pr[b'=1|\mbox{start with $\rho_{\hat{x}uv}^{ideal}$, $x\la$ measure $Y$ with $M_X$, $b'\la \cB(x\oplus m_0\oplus \hat{x})$} ]\\
    &=\Pr[b'=1|\mbox{start with $\rho_{\hat{x}uv}^{ideal}$, $x\la$ measure $Y$ with $M_X$, $b'\la \cB(x\oplus m_1\oplus \hat{x})$} ].
\end{align}
From $\frac{1}{2}\parallel \rho_{\hat{x}uv}^*-\rho_{\hat{x}uv}^{ideal}\parallel\leq \sqrt{\epsilon_{\hat{x}uv}}$, it follows that
\begin{align}
    &|\Pr[b'=1|\mbox{start with {\color{blue}$\rho_{\hat{x}uv}^{*}$}, $x\la$ measure $Y$ with $M_X$, $b'\la \cB(x\oplus m_0\oplus \hat{x})$} ]\\
    &-\Pr[b'=1|\mbox{start with {\color{blue}$\rho_{\hat{x}uv}^{*}$}, $x\la$ measure $Y$ with $M_X$, $b'\la \cB(x\oplus m_1\oplus \hat{x})$} ]|\leq \sqrt{\epsilon_{\hat{x}uv}}.
\end{align}
From the definition of $\mathsf{Succ}_{\hat{x}uv}^b$,
it follows that
$
\abs{\mathsf{Succ}_{\hat{x}uv}^0-\mathsf{Succ}_{\hat{x}uv}^1}\leq\sqrt{\epsilon_{\hat{x}uv}}
$. 
Therefore, we have
\begin{align}
    &\abs{\Pr[\sfhyb{4}{}(0)=1]-\Pr[\sfhyb{4}{}(1)=1]}\\
    &\leq \sum_{\substack{\hat{x}\in C_1/C_2,u\in\bit^q/C_1 \\v\in\bit^q/C_2^{\bot}}}{\rm Pr}_{\hat{x}uv}\abs{\mathsf{Succ}_{\hat{x}uv}^0-\mathsf{Succ}_{\hat{x}uv}^1}\\
    &\leq\sum_{\substack{\hat{x}\in C_1/C_2,u\in\bit^q/C_1 \\v\in\bit^q/C_2^{\bot}}}{\rm Pr}_{\hat{x}uv}\sqrt{\epsilon_{\hat{x}uv}}\\
    &\leq \sqrt{\sum_{\substack{\hat{x}\in C_1/C_2,u\in\bit^q/C_1 \\v\in\bit^q/C_2^{\bot}}}
    {\rm Pr}_{\hat{x}uv}\epsilon_{\hat{x}uv}}=\sqrt{\epsilon}.
\end{align}
In the third inequality, we have used Jensen's inequality and the fact that $\sum_{\substack{\hat{x}\in C_1/C_2,u\in\bit^q/C_1 \\v\in\bit^q/C_2^{\bot}}}{\rm Pr}_{\hat{x}uv}\leq 1$.
\end{proof}
\begin{proposition}\label{prop:Hyb_5_Hyb_6_revoc}
It holds that
\begin{align}
\Pr[\sfhyb{5}{}=0]= \Pr[\sfhyb{6}{}=0].
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_5_Hyb_6_revoc}]
The output of the two experiments do not depend on $\cA_2$.
Therefore, 
the output of the two experiments do not depend on
whether the challenger sends $\ske.\sk$ or $\bot$ to $\cA_2$, or not.
Therefore, it holds that
\begin{align}
    \Pr[\sfhyb{5}{}=0]= \Pr[\sfhyb{6}{}=0].
\end{align}
\end{proof}


\begin{proposition}\label{prop:Hyb_6_Hyb_7_revoc}
Let $\mu$ be the advantage of $\Sigma_{\mathsf{sk}}$.
It holds that
\begin{align}
    \Pr[\sfhyb{6}{}=0]\leq \Pr[\sfhyb{7}{}=0]+\mu.
\end{align}
\end{proposition}
\begin{proof}
To show \cref{prop:Hyb_6_Hyb_7_revoc}, let us assume that $\Pr[\sfhyb{6}{}=0]>\Pr[\sfhyb{7}{}=0]+\mu$.
Then, we can construct an adversary $\cB$ that can break the IND-CPA security of $\Sigma_{\sk}$ as follows.
\begin{enumerate}
    \item $\cB$ receives an encryption query $m^*$ from $\cA_1$.
    \item $\cB$ generates $B^*\la \bit^{p}$, $Q^*\leftarrow[p+q]_{p}$, $y^*\la C_1/C_2$, $u^*\la\bit^{q}/C_1$, $r^*\la\bit^{p}$, $x^*\la C_1/C_2$ and $w^*\la C_2$, sends an encryption query $(B^*,Q^*,r^*,y^*)$ to the challenger of $\expa{\Sigma_{\sk},\cB}{ind}{cpa}(\secp,b)$, and receives $\ske.\ct^*$ from the challenger.
    $\cB$ initializes a register $X^*\seteq U_{Q^*}^\dagger (H^{B^*}\otimes I^{\otimes q})(|r^*\rangle \otimes |x^*\oplus w^*\oplus u^*\rangle)$, computes $h^*\seteq m^*\oplus x^*\oplus y^*$, and sends $(X^*,\ske.\ct^*,u^*,h^*)$ to $\cA_1$.
    This process can be repeated polynomially many times.
    \item $\cB$ receives $(m_0,m_1)$ from $\cA_1$.
    \item $\cB$ generates $B\la \bit^{p}$, $Q\leftarrow[p+q]_{p}$, $y\la C_1/C_2$.
    \item $\cB$ initializes $XY\seteq |\widetilde{0^{p+q}0^{p+q}}\rangle$.
    \item $\cB$ operates $(H^B\otimes I^{\otimes q})U_Q$ on $Y$.
    \item $\cB$ measures $Y$ using $M_{UV}$, and obtains the outcomes $(u,v)$.
    \item $\cB$ measures $Y$ using $M_R$, and obtains the outcome $r$.
    \item $\cB$ generates $\hat{x}\la C_1/C_2$ and computes $h\seteq \hat{x}\oplus y$.
    \item $\cB$ generates $\hat{B}\la \bit^{p}$, $\hat{Q}\leftarrow[p+q]_{p}$ and $\hat{r}\la\bit^{p}$,
    sends $M_0\seteq (B,Q,r,y)$ and $M_1\seteq (\hat{B},\hat{Q},\hat{r},y)$ to the challenger of $\expa{\Sigma_{\sk},\cB}{ind}{cpa}(\secp,b)$,
    and receives $\ske.\ct$ from the challenger.
    \item $\cB$ sends $(X,\ske.\ct,u,h)$ to $\cA_1$.
    \item $\cB$ receives an encryption query $m^*$ from $\cA_1$.
    \item $\cB$ generates $B^*\la \bit^{p}$, $Q^*\leftarrow[p+q]_{p}$, $y^*\la C_1/C_2$, $u^*\la\bit^{q}/C_1$, $r^*\la\bit^{p}$, $x^*\la C_1/C_2$ and $w^*\la C_2$, sends an encryption query $(B^*,Q^*,r^*,y^*)$ to the challenger of $\expa{\Sigma_{\sk},\cB}{ind}{cpa}(\secp,b)$, and receives $\ske.\ct^*$ from the challenger.
    $\cB$ initializes a register $X^*\seteq U_{Q^*}^\dagger (H^{B^*}\otimes I^{\otimes q})(|r^*\rangle \otimes |x^*\oplus w^*\oplus u^*\rangle)$, computes $h^*\seteq m^*\oplus x^*\oplus y^*$, and sends $(X^*,\ske.\ct^*,u^*,h^*)$ to $\cA_1$.
    This process can be repeated polynomially many times.
    \item $\cB$ receives the register $X$ from $\cA_1$.
    \item $\cB$ operates $(H^B\otimes I^{\otimes q})U_Q$ on the register $X$, measures the register $X$ using $M_R$, and obtains the measurement outcome $r'$.
    If $r=r'$, $\cB$ outputs $\mathsf{flag}=\top$.
    Otherwise, $\cB$ outputs $\mathsf{flag}=\bot$.
    \item $\cB$ operates $I^{\otimes p}\otimes U_{uv}^{EC}$ on $X$ and $I^{\otimes p}\otimes U_{uv}^{dec}$ on $Y$.
    $\cB$ measures $X'Y'$ using $P_{C_1/C_2}^{\EPR}$, and obtains the outcome $\isEPR$.
    \item If $\mathsf{flag}=\top$ and $\isEPR=0$, then $\cB$ outputs $1$.
    Otherwise, $\cB$ outputs $\bot$.
\end{enumerate}
It is clear that 
$\Pr[1\la\cB|b=0]=\Pr[\sfhyb{6}{}=0]$ and $\Pr[1\la\cB|b=1]=\Pr[\sfhyb{7}{}=0]$.
By assumption of $\Pr[\sfhyb{6}{}=0]>\Pr[\sfhyb{7}{}=0]+\mu$, we have $\abs{\Pr[1\la\cB|b=0]-\Pr[1\la\cB|b=1]}\geq \mu$, which contradicts the IND-CPA security of $\Sigma_{\sk}$. 
\end{proof}

\begin{proposition}\label{prop:Hyb_7_Hyb_8_revoc}
It holds that
\begin{align}
    \Pr[\sfhyb{7}{}=0]= \Pr[\sfhyb{8}{}=0].
\end{align}
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_7_Hyb_8_revoc}]
The difference between the two experiments is that we change the order of procedures.
All involved quantum operations and measurements are on different registers $X,Y$, except for the measurements $M_R$ and $M_{UV}$ on $Y$. However those measurements commute by definition of $M_R, M_{UV}$. Thus, there is no difference between the two games.
\end{proof}
\begin{proposition}\label{prop:Decode_EPR_state}
For any state $\rho$ of $X'Y'$ and with 
\begin{align}
    &pr_1\seteq \Pr[\isEPR=1|\mbox{start with $\rho$, \isEPR$\la$ measure using $P_t^{\EPR}$}]\\
    &pr_2\seteq {\rm Pr}[\isEPR=1|\mbox{start with $\rho$, $(u,v)\la$ measure using $I^{\otimes q}\otimes M_{UV}$,}\\
    &\hspace{1cm}\mbox{apply $U_{uv}^{EC}\otimes U_{uv}^{dec}$, \isEPR$\la$ measure using $P_{C_1/C_2}^{\EPR}$}]
\end{align}
we have $pr_1\leq pr_2$.
(Here we write in a slight abuse of notation $M_{UV}$ for the restriction of $M_{UV}$ to $X'Y'$.
Since $M_{UV}$ ignores the first $p$ qubits if $X,Y$ anyway, this restriction is well-defined.
And by ``measure using $P_{C_1/C_2}^{\EPR}$'', we mean applying $P_{C_1/C_2}^{\EPR}$ to the first $q$ qubits of the outputs of $U_{uv}^{EC}$ and $U_{uv}^{dec}$.)
\end{proposition}
\begin{proof}[Proof of \cref{prop:Decode_EPR_state}]
We can assume $\rho$ is a pure state $\dyad{\Psi}$ since all other density operators are convex combinations of pure states and the probabilities $pr_1,pr_2$ are then the corresponding convex combinations of the probabilities for the pure states.


Let $U$ be the purification of the steps 
``$(u,v)\la$ measure using $I^{\otimes q}\otimes M_{UV}$, apply $U_{uv}^{EC}\otimes U_{uv}^{dec}$''.
By applying these steps to an initial state $\dyad{\psi}$, we obtain $\Tr_H(U\ket{\psi}\ket{0^m}\bra{ \psi}\bra{0^m}U^{\dagger})$, where $H$ refers to some auxiliary system of dimension $m$.

We obtain
\begin{align}
    &pr_1= \parallel (P_t^{\EPR}\otimes |0^m\rangle\langle 0^m|)|\Psi\rangle|0^m\rangle\parallel^2\\
    &pr_2= \parallel (P_{C_1/C_2}^{\EPR}\otimes I^{\otimes m})U|\Psi\rangle|0^m\rangle\parallel^2
    =\parallel U^\dagger(P_{C_1/C_2}^{\EPR}\otimes I^{\otimes m})U|\Psi\rangle|0^m\rangle \parallel^2.
\end{align}
For simplicity, let us define 
$P_1\seteq P_t^{\EPR}\otimes |0^m\rangle\langle 0^m|$
and
$P_2\seteq U^\dagger(P_{C_1/C_2}^{\EPR}\otimes I^{\otimes m})U$.
Our goal is to prove $pr_1\leq pr_2$.
It is sufficient to show ${\rm im}P_1\subseteq {\rm im}P_2$ for the purpose since $P_1$ and $P_2$ are orthogonal projectors.\ryo{Again, the definition of $\mathrm{im}$.}
By definition of $P_t^{\EPR}$, we have ${\rm im}P_{t}^{\EPR}={\rm span}\{|\widetilde{fe}\rangle :w(f),w(e)\leq t\}$, where $f,e$ are $q$-bit strings, and ${\rm im}P_1={\rm span}\{|\widetilde{fe}\rangle |0^m\rangle:w(f),w(e)\leq t\}$.
Therefore, what we should prove is that $\ket{\widetilde{fe}}\ket{0^m}\in{\rm im}P_2$ for $w(f),w(e)\leq t$.
We fix such $f,e$ for the rest of the proof.

By \cref{prop:EPR_state}, we have 
$2^{-q/2}\sum_{\substack{x\in C_1/C_2,u\in \bit^q/C_1\\ v\in\bit^q/C_2^{\bot}}}|\xi_{xuv}\rangle\otimes |\xi_{xuv}\rangle =|\widetilde{0^q0^q}\rangle$.
So, we obtain $\ket{\widetilde{fe}} = 2^{-q/2}\allowbreak \sum_{\substack{x\in C_1/C_2,u\in \bit^q/C_1\\ v\in\bit^q/C_2^{\bot}}}Z^fX^e|\xi_{xuv}\rangle\otimes|\xi_{xuv}\rangle$.
Since all $|\xi_{xuv}\rangle$ are orthogonal (\cref{prop:orthonormal_basis}),
for any $u,v$ we have that the unnormalized post-measurement state after measuring $|\widetilde{fe}\rangle$ using $I^{\otimes q}\otimes M_{UV}$ with outcome $(u,v)$ is 
$|\Psi_{uv}\rangle\seteq (I^{\otimes q}\otimes P_{uv})|\widetilde{fe}\rangle=2^{-q/2}\sum_{x\in C_1/C_2}Z^fX^e|\xi_{xuv}\rangle\otimes |\xi_{xuv}\rangle$.

By the definition of $U_{uv}^{EC}$ and $U_{uv}^{dec}$, it holds that
\begin{align}
U_{uv}^{EC}Z^fX^e\ket{\xi_{xuv}} &=\pm U_{uv}^{EC}X^eZ^f \ket{\xi_{xuv}}=\pm \ket{x}\otimes \ket{\Phi_{uvfe}}\\
U_{uv}^{dec} \ket{\xi_{xuv}}&=\ket{x} \otimes \ket{\Phi'_{uvfe}}
\end{align}
 for some quantum states $\ket{\Phi_{uvfe}}$ and $\ket{\Phi'_{uvfe}}$ since the Hamming weight of $f$ and $e$ are less than or equal to $t$.
Thus, the unnormalized state after additionally applying $(U_{uv}^{EC}\otimes U_{uv}^{dec})$ to $|\Psi_{uv}\rangle$ is
\begin{align}
    |\Psi'_{uv}\rangle\seteq (U_{uv}^{EC}\otimes U_{uv}^{dec})|\Psi_{uv}\rangle=2^{-q/2}\sum_{x\in C_1/C_2}\pm|x\rangle\otimes |\Phi_{uvfe}\rangle \otimes |x\rangle\otimes |\Phi'_{uvfe}\rangle \in {\rm im}P_{C_1/C_2}^{\EPR}.
\end{align}
Let $\rho'$ denote the state after applying the steps ``$(u,v)\la$ measure using $I^{\otimes q}\otimes M_{UV}$, apply $(U_{uv}^{EC}\otimes U_{uv}^{dec})$'' to the initial state $|\widetilde{fe}\rangle\langle\widetilde{fe}|$.
Then, we can write $\rho'=\sum_{\substack{u\in \bit^q/C_1\\ v\in\bit^q/C_2^{\bot}} }|\Psi'_{uv}\rangle\langle\Psi'_{uv}|$ and have
\begin{align}
    \Tr (P_{C_1/C_2}^{\EPR}\rho')=\sum_{\substack{u\in \bit^q/C_1\\ v\in\bit^q/C_2^{\bot}} }
    \Tr (P_{C_1/C_2}^{\EPR}|\Psi'_{uv}\rangle\langle \Psi'_{uv}|)=
    \sum_{\substack{u\in \bit^q/C_1\\ v\in\bit^q/C_2^{\bot}} }\Tr (|\Psi'_{uv}\rangle\langle \Psi'_{uv}|)=1.
\end{align}
By definition of $U$, we have that $\Tr_H(U|\widetilde{fe}\rangle|0^m\rangle\langle\widetilde{fe}|\langle 0^m|U^\dagger)=\rho'$.
By the equation above, we obtain 
\[\Tr\left(\left(P_{C_1/C_2}^{\EPR}\otimes I^{\otimes m}\right)\left(U|\widetilde{fe}\rangle|0^m\rangle\langle\widetilde{fe}|\langle 0^m|U^{\dagger}\right)\right)=1.
\]
Thus, we derive $U|\widetilde{fe}\rangle |0^m\rangle \in {\rm im}(P_{C_1/C_2}^{\EPR}\otimes I^{\otimes m})$ and $|\widetilde{fe}\rangle |0^m\rangle\in {\rm im}U^\dagger(P_{C_1/C_2}^{\EPR}\otimes I^{\otimes m})U={\rm im}P_2$.
Therefore, we finished proving ${\rm im}P_1\subseteq {\rm im}P_2$.
This is what we want to show to complete the proof.
\end{proof}
\begin{proposition}\label{prop:Hyb_8_Hyb_9_revoc}
$\Pr[\sfhyb{8}{}=0]\leq \Pr[\sfhyb{9}{}=0].$
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_8_Hyb_9_revoc}]
Let $\rho'$ denote the state in $\sfhyb{8}{}$ before step \ref{step:Hyb_8}, conditioned on that the challenger outputs $\top$. We also let $\rho$ denote the result of tracing out in $\rho'$ all but the last $q$ qubits of $X$ and $Y$.

Then, with $pr_1$, $pr_2$ as in \cref{prop:Decode_EPR_state}, we have
\begin{align}
    &\Pr[\sfhyb{8}{}=0]\\
    &=\Pr[\isEPR=0\wedge ok=1:\sfhyb{8}{}]\\
    &=\Pr[\isEPR=0|ok=1 :\sfhyb{8}{}]\cdot \Pr[ok=1:\sfhyb{8}{}]\\
    &={\rm Pr} [\isEPR=0|\mbox{start with } \rho, (u,v)\la \mbox{measure using } I^{\otimes q}\otimes M_{UV},\\
    & \hspace{1cm}\mbox{apply } U_{uv}^{EC}\otimes U_{uv}^{dec}, \isEPR\la \mbox{measure using } P_{C_1/C_2}^{\EPR}]
    \cdot \Pr[ok=1:\sfhyb{8}{}]\\
    &=(1-pr_2)\Pr[ok=1:\sfhyb{8}{}]\\
    &\leq (1-pr_1)\Pr[ok=1:\sfhyb{9}{}]\\
    &=\Pr[\isEPR=0|ok=1:\sfhyb{9}{}]\cdot\Pr[ok=1:\sfhyb{9}{}]\\
    &=\Pr[\isEPR=0\wedge ok=1:\sfhyb{9}{}]\\
    &=\Pr[\sfhyb{9}{}=0].
\end{align}
In the first inequality, we have used \cref{prop:Decode_EPR_state}
and that $\Pr[ok=1]$ is identical in $\sfhyb{8}{}$ and
$\sfhyb{9}{}$ because up to the measurement of the $M_R$, these games are identical.
In the fifth equation, we have used the fact that $\rho$ is also the state in $\sfhyb{9}{}$ right before the measurement of $u,v$, conditioned on that the challenger outputs $\top$.
%\taiga{Note that, in Unruh's paper, he denotes the calculation above as follows
%\begin{align}
%    &\Pr[\sfhyb{8}{}=0]\\
%    &=\Pr[\isEPR=0\wedge ok=1:\sfhyb{8}{}]\\
%    &=\Pr[\isEPR=0|ok=1 :\sfhyb{8}{}]\cdot \Pr[ok=1:\sfhyb{8}{}]\\
%    &\leq\Pr[\isEPR=0|ok=1 :\sfhyb{8}{}]\\
%    &=(1-pr_2)\Pr[ok=1:\sfhyb{8}{}]\\
%    &\cdots 
%\end{align}.
%But, I think that this is his mistake and his proof should be as I wrote.
%In fact, his third equation does not hold.}
\end{proof}
\begin{proposition}\label{prop:top_implies_EPR}
Let $\rho$ be the initial state of a bipartite system $XY$ where $X$ and $Y$ are $(p+q)$-qubits each.
Consider the following game: Pick $B\la\bit^p$, $Q\la[p+q]_p$.
Apply $(H^B\otimes I^{\otimes q})U_Q$ to $X$ and to $Y$.
Then measure $X$ and $Y$ with $M_R$, outcomes $r,r'$.
Let $ok=1$ iff $r=r'$. Then measure $X'Y'$ using $P_t^{\EPR}$, outcome $\isEPR$.
Then $\Pr[ok=1 \wedge \isEPR=0]\leq 3\sqrt{q}\left(1-\frac{p}{2(p+q)}\right)^{t+1}$.
\end{proposition}
\begin{proof}[Proof of \cref{prop:top_implies_EPR}]
We consider two cases.
\paragraph{The first case: $\rho=|\widetilde{fe}\rangle\langle\widetilde{fe}|$ with $w(f)>t$ or $w(e)>t$.}

Note that when measuring both qubits of $|\widetilde{01}\rangle$ or $|\widetilde{10}\rangle$ in the computational basis, the outcomes will be different with probability $1$.
It also holds that $(H\otimes H)|\widetilde{10}\rangle=|\widetilde{01}\rangle$ and $(H\otimes H)|\widetilde{11}\rangle=-|\widetilde{11}\rangle$.

For a given $Q=\{Q_1,\cdots,Q_p\}$ and $B=B_1\cdots B_q$, for all $i$ we have:
\begin{itemize}
    \item If $f_{Q_i}=1$ and $B_i=1$, then $r_i\neq r'_i$ with probability $1$.
    \item If $e_{Q_i}=1$ and $B_i=0$, then $r_i\neq r'_i$ with probability $1$.
\end{itemize}
In the notation of \cref{prop:Detect_error}, the probability that there is no $i$ such that $Q,B$ satisfying one of these cases is written $P(x)$, where $x^0\seteq e$ and $x^1\seteq f$. 
Then, we have
\begin{align}
    \Pr[ok=1 \wedge \isEPR=0] \leq \Pr[ok=1]\leq P(x)\leq 3\sqrt{p}\left(1-\frac{p}{2(p+q)}\right)^{t+1}.
\end{align}
In the second inequality, we have used \cref{prop:Detect_error}.
For simplicity, let us define $\gamma\seteq 3\sqrt{p}\left(1-\frac{p}{2(p+q)}\right)^{t+1}$.

\paragraph{The second case: $\rho=|\widetilde{fe}\rangle\langle\widetilde{fe}|$ with $w(f),w(e)\leq t$.}
In this case, after applying $(H^B\otimes I^{\otimes q})U_Q$ to both $X$ and $Y$ after measuring the first $p$ qubits in $X$ and $Y$, the state of the last $q$ qubit pairs of $XY$ is $|\widetilde{f'e'}\rangle$
where $f'$ is a subsequence of $f$ and $e'$ is a subsequence of $e$.
In particular $w(e')\leq w(e)\leq t$ and $w(f')\leq w(f)\leq t$. Thus, the measurement $P_t^{\EPR}$ will succeed with probability $1$, hence
\begin{align}
    \Pr[ok=1 \wedge \isEPR=0]\leq \Pr[\isEPR=0]=0\leq \gamma.
\end{align}
Therefore, we have
\begin{align}
\Pr[ok=1 \wedge \isEPR=0]\leq \gamma
\hspace{0.5cm} \mbox{ if } \rho=|\widetilde{fe}\rangle\langle\widetilde{fe}|\mbox{ for some} f,e\in\bit^{p+q}.
\end{align}
Now we consider the case that $\rho=\sum_i \alpha_i|\widetilde{f_ie_i}\rangle\langle \widetilde{f_ie_i}|$
 for some $f_i,e_i\in\bit^{p+q}$ and $\alpha_i\geq 0$, $\sum_i \alpha_i=1$.
 Then,
 \begin{align}
     &\Pr[ok=1\wedge \isEPR=0]\\
    & =\sum_i \alpha_i \Pr[ok=1 \wedge \isEPR=0 |\mbox{using }\rho\seteq |\widetilde{f_ie_i}\rangle\langle \widetilde{f_ie_i}| ]\leq \sum_i\alpha_i\gamma=\gamma.
 \end{align}
 Now we consider the general case of an arbitrary density operator $\rho$. 
We define a projector $P_{eq} \seteq \sum_{\substack{x\in\bit^p\\ y_1,y_2\in\bit^q}}|xy_1\rangle\langle xy_1|\otimes |xy_2\rangle \langle xy_2|$. This measures whether the first $p$ qubits pairs have the same value in the computational basis.
Note that $P_{eq}$ is a tensor product of projectors $P_{eq}^1\seteq |00\rangle \langle 00|+|11\rangle \langle 11|$ and identities.
It also holds that $P_{eq}^1=|\widetilde{00}\rangle \langle \widetilde{00}|+|\widetilde{10}\rangle \langle \widetilde{10}|$.
Thus, $P_{eq}$ is diagonal in the Bell basis. $P_{t}^{\EPR}$ is also diagonal in the Bell basis by definition.

We define $M_{Bell}\seteq \{|\widetilde{fe}\rangle \langle \widetilde{fe}|\}_{f,e\in \bit^{p+q}}$  This is a complete measurement in the Bell basis.
Since $M_{Bell}$ is diagonal in the Bell basis, it commutes with $P_{eq}$ and $P_{t}^{\EPR}$.

Furthermore, since $U_Q\otimes U_Q$ only reorders of the qubit pairs, $M_{Bell}$ and $U_Q\otimes U_Q$ commute if we discard the result of $M_{Bell}$.
(Otherwise, the outcome of $M_{Bell}$ would have to be additionally permuted.)

Since $(H\otimes H)|\widetilde{fe}\rangle =\pm|\widetilde{ef}\rangle$, we have that $(H^B\otimes I^{\otimes q}\otimes H^B\otimes I^{\otimes q})$ commutes with $M_{Bell}$
if we discard the outcome of $M_{Bell}$.
(Otherwise, the bit pairs with $B_i=1$ in the outcome of $M_{Bell}$ would need to be swapped.)

Thus, $M_{Bell}$ commutes with applying $(H^B\otimes I^{\otimes q})U_Q$ to both $X$ and $Y$.
Let $\rho^*$ be the state we get when measuring $\rho$ using $M_{Bell}$ and discarding the outcome.
Then, $\rho^*=\sum_{i}\alpha_i|\widetilde{f_ie_i}\rangle \langle \widetilde{f_ie_i}|$ for some $\alpha_i,f_i,e_i$ with $\alpha_i\geq0$, $\sum_i\alpha_i=1$.

It holds that
\begin{align}
    &{\rm Pr}[ok=1\wedge \isEPR=0: B\la \bit^{p}, Q\la [p+q]_p, \mbox{apply $(H^B\otimes I^{\otimes q})U_Q$ to $X,Y$},\\
    & r,r'\la \mbox{measure $X,Y$ with $M_R$}, \isEPR\la \mbox{measure $X'Y'$ with $P_t^{\EPR}$}]\\
    &={\rm Pr}[ok=1\wedge \isEPR=0: B\la \bit^{p}, Q\la [p+q]_p, \mbox{apply $(H^B\otimes I^{\otimes q})U_Q$ to $X,Y$},\\
    & {\color{blue} ok\la \mbox{measure $X,Y$ with $P_{eq}$}}, \isEPR\la \mbox{measure $X'Y'$ with $P_t^{\EPR}$}]\\
    &={\rm Pr}[ok=1\wedge \isEPR=0: B\la \bit^{p}, Q\la [p+q]_p, \mbox{apply $(H^B\otimes I^{\otimes q})U_Q$ to $X,Y$},\\
    & { ok\la \mbox{measure $X,Y$ with $P_{eq}$}}, \isEPR\la \mbox{measure $X'Y'$ with $P_t^{\EPR}$}, {\color{blue}\mbox{measure $XY$ with $M_{Bell}$}}]\\
    &={\rm Pr}[ok=1\wedge \isEPR=0:  {\color{blue}\mbox{measure $XY$ with $M_{Bell}$}}, B\la \bit^{p}, Q\la [p+q]_p,\\
    &\mbox{apply $(H^B\otimes I^{\otimes q})U_Q$ to $X,Y$},{ ok\la \mbox{measure $X,Y$ with $P_{eq}$}}, \isEPR\la \mbox{measure $X'Y'$ with $P_t^{\EPR}$}]\\
    &={\rm Pr}[ok=1\wedge \isEPR=0:  {\color{blue}\mbox{use $\rho^*$ instead of $\rho$}}, B\la \bit^{p}, Q\la [p+q]_p,\\
    &\mbox{apply $(H^B\otimes I^{\otimes q})U_Q$ to $X,Y$},{ ok\la \mbox{measure $X,Y$ with $P_{eq}$}}, \isEPR\la \mbox{measure $X'Y'$ with $P_t^{\EPR}$}]\\
    &\leq \gamma.
\end{align}
In the first equation, we have used that $P_{eq}$ and $M_R$ operate only on the first $p$ qubit pairs. Thus, they do not touch $X'Y'$. 
In the third equation, we have used that $M_{Bell}$ commutes with applying $(H_B\otimes I^{\otimes q})U_Q$ with $P_t^{\EPR}$ and with $P_{eq}$ as discussed above.
In the first inequality, we have used that $\rho^*$ is of the form $\sum_i \alpha_i|\widetilde{f_ie_i}\rangle\langle \widetilde{f_ie_i}|$.

Since the left hand side of the proceeding calculation is the probability ${\rm Pr}[ok=1 \wedge \isEPR=0]$
from the statement of the proposition, the proposition follows.
\end{proof}

\begin{proposition}\label{prop:Hyb_9_revoc}
$\Pr[\sfhyb{9}{}=0]\leq 3\sqrt{p}\left(1-\frac{p}{2(p+q)}\right)^{t+1}$.
\end{proposition}
\begin{proof}[Proof of \cref{prop:Hyb_9_revoc}]
Let $\rho$ denote the state in $\sfhyb{9}{}$ right before choosing $B,Q$.
Then, the game in \cref{prop:top_implies_EPR} is identical to $\sfhyb{9}{}$.
By \cref{prop:top_implies_EPR}, we have
\begin{align}
\Pr[ok=1 \wedge \isEPR=0: \sfhyb{9}{}]\leq 3\sqrt{p}\left(1-\frac{p}{2(p+q)} \right)^{t+1}.   
\end{align}
\end{proof}

We can now prove \cref{thm:sk_ever_security_wo_rom}.
We need to show that
\begin{align}
    \delta\seteq \abs{\Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,0)=1]-
    \Pr[\expd{\Sigma_{\mathsf{cesk}},\cA}{cert}{ever}{ind}{cpa}(\lambda,1)=1]}
\end{align} 
is negligible. Note that $|C_1/C_2|=2^{k_1-k_2}$.
By \cref{prop:Exp_Hyb_1_revoc}, it holds that
\begin{align}
    \delta =2^{k_1-k_2}\abs{\Pr[\sfhyb{1}{}(0)=1]-\Pr[\sfhyb{1}{}(1)=1]}.
\end{align}
By \cref{prop:Hyb_1_Hyb_2_revoc,prop:Hyb_2_Hyb_3_revoc,prop:Hyb_3_Hyb_4_revoc}
it holds that
\begin{align}
\delta =2^{k_1-k_2}\abs{\Pr[\sfhyb{4}{}(0)=1]-\Pr[\sfhyb{4}{}(1)=1]}.
\end{align}
By \cref{prop:Hyb_4_Hyb_5_revoc,prop:Hyb_5_Hyb_6_revoc}, it holds that
\begin{align}
    \delta\leq 2^{k_1-k_2}\sqrt{\epsilon},
\end{align}
where $\epsilon\seteq \Pr[\sfhyb{6}{}=0]$.
By \cref{prop:Hyb_6_Hyb_7_revoc} it holds that
\begin{align}
    \epsilon\leq \Pr[\sfhyb{7}{}=0]+\mu,
\end{align}
where $\mu$ is the advantage of $\Sigma_{\sk}$.
By \cref{prop:Hyb_7_Hyb_8_revoc,prop:Hyb_8_Hyb_9_revoc}, it holds that
\begin{align}
    \epsilon\leq \Pr[\sfhyb{9}{}=0]+\mu.
\end{align}
By \cref{prop:Hyb_9_revoc}, it holds that
\begin{align}
\epsilon \leq 3\sqrt{p}\left(1-\frac{p}{2(p+q)}\right)^{t+1}+\mu,
\end{align}
where $p,q,t$ are parameters of the protocol.
Putting it all together,
\begin{align}
    \delta\leq \sqrt{2^{2(k_1-k_2)}\cdot 3\sqrt{p}\left(1-\frac{p}{2(p+q)}\right)^{t+1}+2^{2(k_1-k_2)}\cdot\mu} \, .
\end{align}
Here let us define $\mu_1\seteq 2^{2(k_1-k_2)}\cdot 3\sqrt{p}\left(1-\frac{p}{2(p+q)}\right)^{t+1}$.
We have that $2^{2(k_1-k_2)}\mu$ is negligible by assumption.
To show that $\mu_1$ is negligible, let $\ell\seteq k_1-k_2$ and observe that
\begin{align}
    \mu_1/(3\sqrt{p})
    &\leq 2^{2\ell}\left(1-\frac{p}{2(p+q)}\right)^t
    =2^{2\ell}\left(\left(1-\frac{p}{2(p+q)}\right)^{2(p+q)/p}\right)^{\frac{tp}{2(p+q)}}\\
    &\leq 2^{2\ell} e^{-tp/\left(2\left(p+q\right)\right)}=e^{-\frac{1}{2}\left(\frac{tp}{p+q}-4\ell {\rm ln} 2\right)} 
\end{align}
In the first inequality, we have used that $\left(1-1/x\right)^x$ is increasing for $x\geq 1$ and tends to $1/e$.
Since $(tp/(p+q)-4\ell {\rm ln} 2)$ is super-logarithmic by assumption, $\mu_1/(3\sqrt{p})$ is negligible.
Since $p$ is polynomially bounded, $\mu_1$ is negligible.

Since $\mu_1$ and $2^{2(k_1-k_2)}\cdot\mu$ are both negligible, $\delta$ is also negligible.
Therefore, $\Sigma_{\mathsf{cesk}}$ is certified everlasting IND-CPA secure.
\end{proof}

==> Sec_Two_Party.tex <==
{\color{red}
\section{Certified Everlasting Two-Message Two-Party Computation}
In this section, we introduce the notion of certified everlasting two-message two-party computation.
\subsection{Definition}

\begin{definition}[Certified Everlasting Two Message Two-Party Computation]\label{def:two-party}
Let $\Cs_n$ be a family of circuits that takes $n$-bit inputs.
A certified everlasting two-message two-party computation scheme is a tuple of algorithm $\Pi=(\mathsf{CRSGen},\mathsf{Receiver},\mathsf{Send},\mathsf{Derive},\Vrfy)$.
\begin{description}
\item[$\mathsf{CRSGen}(1^\secp)\ra \crs$:]
This is an algorithm supposed to run by a trusted third party that takes $1^\secp$ as input, and outputs a common reference string $\crs$.
\item[$\mathsf{Receiver}(C,\crs,x_\cR)\ra (m_1,r_1)$:]
This is an algorithm supposed to run by a receiver that takes a circuit $C\in\Cs_n$, $\crs$ and a receiver's input $x_\cR$ as input, and outputs a message $m_1$ and an internal state $r_1$.
\item[$\mathsf{Sender}(C,\crs,x_\cS,m_1)\ra (m_2,\vk)$:] 
This is an algorithm supposed to run by a sender that takes $C\in\Cs_n$, $\crs$, a sender's input $x_\cS$ and $m_1$, and outputs a message $m_2$ and a verification key $\vk$.
\item[$\mathsf{Derive}(m_2,r_1)\ra y$:]
This is an algorithm supposed to run by a receiver that takes $m_2$ and $r_1$, and outputs $y$.
\item[$\Delete(m_2)\ra \cert$:]
This is an algorithm supposed to run by a receiver that takes $m_2$ as input, and outputs $\cert$.
\item[$\Vrfy(\vk,\cert)\ra \top /\bot$:]
This is an algorithm supposed to run by a sender that takes $\vk$ and $\cert$, and outputs $\top$ or $\bot$.
\end{description}
\end{definition}

We require that a certified everlasting two-party computation satisfies correctness defined below.
\begin{definition}[Correctness for Certified Everlasting Two-Party Computation]\label{def:correct_ever_two_pary}
There are two types correctness.
The first is evaluation correctness,
and the second is verification correctness.

\paragraph{Evaluation Correctness:}
There exists a negligible function such that for any $\secp\in \N$, $x_\cR,x_\cS\in\bit^n$ and $C\in\Cs_n$,
\begin{align}
\Pr\left[
C(x_\cS,x_\cR)\neq y
\ \middle |
\begin{array}{ll}
\crs\la\mathsf{CRSGen}(1^\secp)\\
(m_1,r_1)\la\mathsf{Receiver}(C,\crs,x_\cR) \\
(m_2,\vk)\la\mathsf{Sender}(C,\crs,x_\cS,m_1)\\
y\la\mathsf{Derive}(m_2,r_1)
\end{array}
\right] 
\leq\negl(\secp).
\end{align}

\paragraph{Verification Correctness:}
There exists a negligible function such that for any $\secp\in \N$, $x_\cR,x_\cS\in\bit^n$ and $C\in\Cs_n$, 
\begin{align}
\Pr\left[
\Vrfy(\vk,\cert)= \bot
\ \middle |
\begin{array}{ll}
\crs\la\mathsf{CRSGen}(1^\secp)\\
(m_1,r_1)\la\mathsf{Receiver}(C,\crs,x_\cR) \\
(m_2,\vk)\la\mathsf{Sender}(C,\crs,x_\cS,m_1)\\
\cert\la\Delete(m_2)
\end{array}
\right] 
\leq\negl(\secp).
\end{align}
\end{definition}




\begin{definition}[One-Side Simulation Security for Two-Party Computation]\label{def:sec_two-party}
There are three types of the security.
The first is statistical receiver's security,
the second is computational sender's security,
and the third is certified everlasting sender's security.
\paragraph{(Semi-Honeset) Statistical Receiver's Security:}
There exists a QPT simulator $\Sim$ such that for all distinguihser $\cD$, $\secp\in\N$ and $x_\cR$
\begin{align}
    \left|
    \Pr\left[
    1\la\cD(C,\crs,m_1)
    \ \middle |
    \begin{array}{ll}
    \crs\la\mathsf{CRSGen}(1^\secp)\\
    (m_1,r_1)\la \mathsf{Receiver}(C,\crs,x_\cR)
    \end{array}
    \right] 
    -
    \Pr\left[
    1\la\cD(C,\crs,m^*)
    \ \middle |
    \begin{array}{ll}
    \crs\la\mathsf{CRSGen}(1^\secp)\\
    m^*\la \Sim(C,\crs)
    \end{array}
    \right] 
    \right|
    \leq \negl(\lambda).
\end{align}


\paragraph{Computational Sender's Security:}
Let $\aux_\cR$ be a quantum side information of a (possibly malicious) QPT receiver $\cR$ that may be entangled with a side information $\aux_\cD$ of a QPT distinguisher $\cD$.
Let $\mathcal{I}[x_\cS](\cdot)$ be an ideal functionality that takes $x'_\cR$ or $\bot$ as input, and outputs $y\la C(x'_\cR,x_\cS)$ in the non-$\bot$ case, and output $\bot$ in the $\bot$ case.
Let $\Sim_\cR=(\Sim_\cR^{(1)},\Sim_\cR^{(2)},\Sim_\cR^{(3)})$ a QPT simulator with the following syntax.
\begin{itemize}
\item $\Sim_\cR^{(1)}(1^\secp)$ generates $(\crs,\tau)$, sends $\crs$ to $\cR(x_\cR,\aux_\cR)$, and sends back $m_1$.
\item $\Sim_\cR^{(2)}(\tau,m_1)$ takes the adversary's and either extracts an input $x'_\cR$ or $\bot$, which it forwards to an ideal functionality $\mathcal{I}[x_\cS](\cdot)$.
In the non-$\bot$ case, $\mathcal{I}[x_\cS]$ computes and returns $y\la C(x_\cS,x'_\cR)$ to the simulator and outputs $\mathsf{ok}$.
In the $\bot$ case, it outputs $\abort$, and the simulator sends $\bot$ to $\cR$ and simulation ends.
\item $\Sim_\cR^{(3)}(\tau,y)$ receives an output $y$ from the ideal functionality and uses it to form a second round message $m_2$, which it sends to $\cR$.
\end{itemize}

The random variable $\mathsf{IDEAL}_{\Pi,C,\cR}(\Sim_\cR,x_\cR,x_\cS,\cR)$ consists of the output of $\cR(x_\cR,\aux_\cR)$ after interacting with the simulator $\Sim_\cR$, along with the output of $\mathcal{I}[x_\cS](\cdot)$.
The random variable $\mathsf{REAL}_{\Pi,C,\cR}(\cR,x_\cR,x_\cS,\aux_\cR)$ consists of $(z,y_\cS)$, where $z$ is $\cR$'s final output after interacting with an honest sender $S$ which behaves according to $\Pi$, and $(y_\cS,\cert)\la \mathsf{Derive}(m_2,r_1)$. 

We say that the protocol $\Pi$ for a circuit $C$ satisfies computational sender's security if there exists a QPT simulator $\Sim_\cR$ such that for all $(x_\cS,x_\cR,\aux_\cR,\aux_\cD)$ and for all QPT distinguisher $\cD$, there exists a negligible function such that
\begin{align}
    \abs{\Pr[\cD(\aux_\cD,\mathsf{REAL}_{\Pi,C,\cR}(\cR,x_\cS,x_\cR,\aux_\cR))=1]-
    \Pr[\cD(\aux_\cD,\mathsf{IDEAL}_{\Pi,C,\cR}(\Sim_\cR,x_\cS,x_\cR,\aux_\cR))=1]
    }\leq \negl(\lambda).
\end{align}


\paragraph{Certified Everlasting Sender's Security:}
Let $\aux_\cR$ be a quantum side information of a (possibly malicious) QPT receiver $\cR$ that may be entangled with a side information $\aux_\cD$ of a QPT distinguisher $\cD$.
Let $\mathcal{I}[x_\cS](\cdot)$ be an ideal functionality that takes $x'_\cR$ or $\bot$ as input, and outputs $y\la C(x'_\cR,x_\cS)$ in the non-$\bot$ case, and output $\bot$ in the $\bot$ case.
Let $\Sim_\cR=(\Sim_\cR^{(1)},\Sim_\cR^{(2)},\Sim_\cR^{(3)},\Sim_\cR^{(4)})$ a QPT simulator with the following syntax.
\begin{itemize}
\item $\Sim_\cR^{(1)}(1^\secp)$ generates $(\crs,\tau)$, sends $\crs$ to $\cR(x_\cS,\aux_\cR)$, and sends back $m_1$.
\item $\Sim_\cR^{(2)}(\tau,m_1)$ takes the adversary's and either extracts an input $x'_\cR$ or $\bot$, which it forwards to an ideal functionality $\mathcal{I}[x_\cS](\cdot)$.
In the non-$\bot$ case, $\mathcal{I}[x_\cS]$ computes and returns $y\la C(x_\cS,x'_\cR)$ to the simulator and outputs $\mathsf{ok}$.
In the $\bot$ case, it outputs $\abort$, and the simulator sends $\bot$ to $\cR$ and simulation ends.
\item $\Sim_\cR^{(3)}(\tau,y)$ receives an output $y$ from the ideal functionality and uses it to form a second round message $m_2$ and a verification key $\vk$, and sends $m_2$ to $\cR$.
\item $\Sim_\cR^{(4)}(\vk,\cert)$ receives a certificate $\cert$ from $\cR$, and outputs $\top$ or $\bot$.
\end{itemize}

When $\Sim_\cR^{(4)}$ outputs $\bot$, $\mathsf{IDEAL}_{\Pi,C,\cR}(\Sim_\cR,x_\cR,x_\cS,\cR)$ is $(\bot,\bot)$.
When $\Sim_\cR^{(4)}$ outputs $\top$,
the random variable $\mathsf{IDEAL}_{\Pi,C,\cR}(\Sim_\cR,x_\cR,x_\cS,\cR)$ is $((z,y_\cS),\top)$, where $z$ is the output of $\cR(x_\cR,\aux_\cR)$ after interacting with the simulator $\Sim_\cR$, and $y_\cS$ is the output of $\mathcal{I}[x_\cS](\cdot)$.
The random variable $\mathsf{REAL}_{\Pi,C,\cR}(\cR,x_\cR,x_\cS,\aux_\cR)$ is $(\bot,\bot)$ when an honest sender $S$'s verification algorithm outputs $\bot$ after interacting with $\cR$.
The random variable $\mathsf{REAL}_{\Pi,C,\cR}(\cR,x_\cR,x_\cS,\aux_\cR)$ is $((z,y_\cS),\top)$, where $z$ is $\cR$'s final output after interacting with an honest sender $S$ which behaves according to $\Pi$, and $y_\cS$ is $S$'s output when an honest sender $S$'s verification algorithm outputs $\bot$ after interacting with $\cR$.

We say that the protocol $\Pi$ for a circuit $C$ satisfies certified everlasting sender's security if there exists a QPT simulator $\Sim_\cR$ such that for all $(x_\cS,x_\cR,\aux_\cR,\aux_\cD)$ and for all unbounded distinguisher $\cD$, there exists a negligible function such that
\begin{align}
    \abs{\Pr[\cD(\aux_\cD,\mathsf{REAL}_{\Pi,C,\cR}(\cR,x_\cS,x_\cR,\aux_\cR))=1]-
    \Pr[\cD(\aux_\cD,\mathsf{IDEAL}_{\Pi,C,\cR}(\Sim_\cR,x_\cS,x_\cR,\aux_\cR))=1]
    }\leq \negl(\lambda).
\end{align}
\end{definition}


\subsection{Construction}
\begin{description}
\item[$\mathsf{CRSGen}(1^\secp)$:]$ $
\begin{itemize}
    \item For $i\in[n]$, compute $\ot.\crs[i]\la\OT.\mathsf{CRSGen}(1^\secp)$.
    \item Output $\crs\seteq\{\ot.\crs[i]\}_{i\in[n]}$.
\end{itemize}
\item[$\mathsf{Receiver}(C,\crs,x_\cR)$:]$ $
\begin{itemize}
    \item Parse $\crs=\{\ot.\crs[i]\}_{i\in[n]}$.
    \item For $i\in[n]$, compute $(\ot.\ot_1[i],\ot.\state[i])\la\OT.\mathsf{Receiver}(\ot.\crs[i],x_\cR[i])$.
    \item Output $m_1\seteq\{\ot.\ot_1[i]\}_{i\in[n]}$ and $r_1\seteq \{\ot.\state[i]\}_{i\in[n]}$.
\end{itemize}
\item[$\mathsf{Sender}(C,\crs,x_\cS,m_1)$:]$ $
\begin{itemize}
    \item Parse $\crs=\{\ot.\crs[i]\}_{i\in[n]}$ and $m_1=\{\ot.\ot_1[i]\}_{i\in[n]}$.
    \item Compute $\{L_{i,\alpha}\}_{i\in[n],\alpha\in\bit}\la\mathsf{GC}.\Samp(1^\secp)$.
    \item Compute $(\widetilde{C}, \gc.\vk ) \la\mathsf{GC}.\Garble(1^\secp,C(\cdot,x_\cS),\{L_{i,\alpha}\}_{i\in[n],\alpha\in\bit})$.
    \item For $i\in[n]$, compute $(\ot.\ot_2[i],\ot.\vk[i])\la\OT.\mathsf{Sender}(\ot.\crs[i], \ot.\ot_1[i],\{L_{i,\alpha}\}_{\alpha\in\bit})$.
    \item Output $m_2\seteq (\{\ot.\ot_2[i]\}_{i\in[n]},\widetilde{C})$ and $\vk\seteq (\{\ot.\vk[i]\}_{i\in[n]},\gc.\vk)$. 
\end{itemize}
\item[$\mathsf{Derive}(m_2,r_1)$:]$ $
\begin{itemize}
    \item Parse $m_2= (\{\ot.\ot_2[i]\}_{i\in[n]},\widetilde{C})$ and $r_1=\{\ot.\state[i]\}_{i\in[n]}$.
    \item For $i\in[n]$, compute $(L_{i,x_{\cR}^*[i]},\widehat{\ot.\ot_2[i]})\la\OT.\mathsf{Derive}(\ot.\state[i],\ot.\ot_2[i])$.
    \item For $i\in[n]$, compute $(y,\widehat{C})\la\mathsf{GC}\Eval(\widetilde{C},\{L_{i,x_\cR^*[i]}\}_{i\in[n]})$.
    \item Output $y$.
\end{itemize}
\item[$\Delete(m_2)$:]$ $
\begin{itemize}
    \item Parse $m_2=(\{\ot.\ot_2[i]\}_{i\in[n]},\widetilde{C})$.
    \item For $i\in[n]$, compute $\ot.\cert[i]\la\OT.\Delete(\ot.\ot_2[i])$.
    \item Compute $\gc.\cert\la\mathsf{GC}.\Delete(\widetilde{C})$.
    \item Output $\cert\seteq (\{\ot.\cert[i]\}_{i\in[n]},\gc.\cert)$.
\end{itemize}
\item[$\Vrfy(\vk,\cert)$:]$ $
\begin{itemize}
    \item Parse $\vk=(\{\ot.\vk[i]\}_{i\in[n]},\gc.\vk)$ and $\cert= (\{\ot.\cert[i]\}_{i\in[n]},\gc.\cert)$.
    \item For $i\in[n]$, compute $\top/\bot\la\OT.\Vrfy(\ot.\vk[i],\ot.\cert[i])$.
    \item Compute $\top/\bot\la\mathsf{GC}.\Vrfy(\mathsf{gc}.\vk,\mathsf{gc}.\cert)$.
    \item Output $\top$ if $\top\la\mathsf{GC}.\Vrfy(\gc.\vk,\gc.\cert)$ and $\top\la\OT.\Vrfy(\ot.\vk[i],\ot.\cert[i])$ for all $i\in[n]$. Otherwise, output $\bot$.
\end{itemize}
\end{description}
}






==> Sec_cut_choose.tex <==
\section{\cref{lem:cut_and_choose_pke}}\label{sec:proof_cut_choose}
We use the following lemma for the proof of our certified everlasting RNCE in~\cref{sec:const_rnce_classic} and  our certified everlasting FE in \cref{sec:const_func_non_adapt}.
The proof is shown with the standard hybrid argument.
It is also easy to see that a similar lemma holds for IND-CPA security.
\begin{lemma}\label{lem:cut_and_choose_pke}
Let $s$ be some polynomial of the security parameter $\lambda$.
Let $\Sigma\seteq(\keygen,\Enc,\Dec,\Delete,\Vrfy)$ be a certified everlasting PKE scheme.
Let us consider the following security experiment 
$\expc{\Sigma,\cA}{multi}{cert}{ever}(\secp,b)$ against $\cA$ consisting of any QPT adversary $\cA_1$ and any unbounded adversary $\cA_2$.
\begin{enumerate}
    \item The challenge generates $(\pk_{i,\alpha},\sk_{i,\alpha})\la\keygen(1^\secp)$ for all $i\in[s]$ and $\alpha\in\bit$,
    and sends $\{\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_1$.
    \item $\cA_1$ chooses $f\in\bit^s$ and $(m_0[1],m_0[2],\cdots, m_0[s],m_1[1],m_1[2], \cdots, m_1[s]) \in\Ms^{2s}$,
    and sends $(f,m_0[1],m_0[2],\\ \cdots ,m_0[s],m_1[1],m_1[2],\cdots, m_1[s] )$ to the challenger.
    \item The challenger computes 
    $
    (\vk_{i,f[i]\oplus 1},\ct_{i,f[i]\oplus 1})\la \Enc(\pk_{i,f[i]\oplus 1},m_b[i])$ for all $i\in[s]$,
    and sends $(\{\sk_{i,f[i]}\}_{i\in [s]},\\ \{\ct_{i,f[i]\oplus 1}\}_{i\in[s]})$ to $\cA_1$.
    \item At some point, $\cA_1$ sends $\{\cert_{i,f[i]\oplus 1}\}_{i\in[s]}$ to the challenger,
    and sends its internal state to $\cA_2$.
    \item The challenger computes $\Vrfy(\vk_{i,f[i]\oplus 1},\cert_{i,f[i]\oplus 1})$ for every $i\in[s]$.
    If all results are $\top$, the challenger outputs $\top$, and sends $\{\sk_{i,f[i]\oplus 1}\}_{i\in [s]}$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$, and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$, then the output of the experiment is $b'$. Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
If the $\Sigma$ satisfies the certified everlasting IND-CPA security,
\begin{align}
\advc{\Sigma,\cA}{multi}{cert}{ever}(\secp)
\seteq \abs{\Pr[ \expb{\Sigma,\cA}{multi}{cert}{ever}(\secp, 0)=1] - \Pr[ \expb{\Sigma,\cA}{multi}{cert}{ever}(\secp, 1)=1] }\leq \negl(\secp)
\end{align}
for any QPT adversary $\cA_1$ and any unbounded adversary $\cA_2$.
\end{lemma}

\begin{proof}[Proof of \cref{lem:cut_and_choose_pke}]
Let us consider the following hybrids for $j\in\{0,1,\cdots ,s\}$.
\begin{description}
\item[$\sfhyb{j}{}$:] $ $
\begin{enumerate}
    \item The challenger generates $(\pk_{i,\alpha},\sk_{i,\alpha})\la\keygen(1^\secp)$ for every $i\in[s]$ and $\alpha\in\bit$, and sends $\{\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_1$.
    \item $\cA_1$ chooses $f\in\bit^s$ and $(m_0[1],m_0[2],\cdots, m_0[s],m_1[1],m_1[2],\cdots, m_1[s]) \in\Ms^{2s}$,
    and sends $(f,m_0[1],m_0[2],\cdots, m_0[s],m_1[1],m_1[2],\cdots, m_1[s] )$ to the challenger.
    \item The challenger computes 
    \begin{align}
    (\vk_{i,f[i]\oplus 1},\ct_{i,f[i]\oplus 1})\la \Enc(\pk_{i,f[i]\oplus 1},m_1[i])
    \end{align}
    for $i\in[j]$ and 
    \begin{align}
    (\vk_{i,f[i]\oplus 1},\ct_{i,f[i]\oplus 1})\la \Enc(\pk_{i,f[i]\oplus 1},m_0[i])
    \end{align}
    for $i\in\{j+1,j+2,\cdots,s\}$,
    and sends $(\{\sk_{i,f[i]}\}_{i\in [s]}, \{\ct_{i,f[i]\oplus 1}\}_{i\in[s]})$ to $\cA_1$.
    \item At some point, $\cA_1$ sends $\{\cert_{i,f[i]\oplus 1}\}_{i\in[s]}$ to the challenger,
    and sends its internal state to $\cA_2$.
    \item The challenger computes $\Vrfy(\vk_{i,f[i]\oplus 1},\cert_{i,f[i]\oplus 1})$ for every $i\in[s]$.
    If all results are $\top$, the challenger outputs $\top$, and sends $\{\sk_{i,f[i]\oplus 1}\}_{i\in [s]}$ to $\cA_2$.
    Otherwise, the challenger outputs $\bot$, and sends $\bot$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item If the challenger outputs $\top$, then the output of the experiment is $b'$. Otherwise, the output of the experiment is $\bot$.
\end{enumerate}
\end{description}
It is clear that $\Pr[\sfhyb{0}{}=1]=\Pr[\expd{\Sigma,\cA}{multi}{cert}{ever}(\secp,0)=1]$ and $\Pr[\sfhyb{s}{}=1]=\Pr[\expd{\Sigma,\cA}{multi}{cert}{ever}(\secp,1)=1]$.
Furthermore, we can show 
\begin{align}
    \abs{\Pr[\sfhyb{j}{}=1]-\Pr[\sfhyb{j+1}{}=1]}\leq\negl(\lambda)
\end{align}
for each $j\in\{0,1,\cdots,s-1\}$.
(Its proof is given below.) From these facts, we obtain \cref{lem:cut_and_choose_pke}.

Let us show the remaining one. To show it, let us assume that $\abs{\Pr[\sfhyb{j}{}=1]-\Pr[\sfhyb{j+1}{}=1]}$ is non-negligible.
Then, we can construct an adversary $\cB$ that can break the certified everlasting IND-CPA security of $\Sigma$ as follows. 

\begin{enumerate}
    \item $\cB$ receives $\pk$ from the challenger of $\expd{\Sigma,\cB}{cert}{ever}{ind}{cpa}(\secp,b)$.
    \item $\cB$ generates $\beta\la\bit$ and sets $\pk_{j+1,\beta}\seteq \pk$. 
    \item $\cB$ generates $(\pk_{i,\alpha},\sk_{i,\alpha})\la\keygen(1^\secp)$ for $i\in\{1,\cdots,j,j+2,\cdots, s\}$ and $\alpha\in\bit$, and $(\pk_{j+1,\beta\oplus 1},\sk_{j+1,\beta\oplus 1})\la\keygen(1^\secp)$.
    \item $\cB$ sends $\{\pk_{i,\alpha}\}_{i\in[s],\alpha\in\bit}$ to $\cA_1$.
    \item $\cA_1$ chooses $f\in\bit^s$ and $(m_0[1],m_0[2],\cdots, m_0[s],m_1[1],m_1[2],\cdots, m_1[s]) \in\Ms^{2s}$,
    and sends $(f,m_0[1],m_0[2],\\ \cdots, m_0[s],m_1[1],m_1[2],\cdots, m_1[s] )$ to the challenger.
    \item If $f[j+1]=\beta$, $\cB$ aborts the experiment, and outputs $\bot$.
    \item $\cB$ computes
    \begin{align}
        (\vk_{i,f[i]\oplus 1},\ct_{i,f[i]\oplus 1})\la \Enc(\pk_{i,f[i]\oplus 1},m_1[i])
    \end{align}
    for $i\in[j]$ and
    \begin{align}
        (\vk_{i,f[i]\oplus 1},\ct_{i,f[i]\oplus 1})\la \Enc(\pk_{i,f[i]\oplus 1},m_0[i])
    \end{align}
    for $i\in\{j+2,\cdots, s\}$.
    \item $\cB$ sends $(m_0[j+1],m_1[j+1])$ to the challenger of $\expd{\Sigma,\cB}{cert}{ever}{ind}{cpa}(\secp,b)$.
    The challenger computes $(\vk_{j+1,f[j+1]\oplus 1},\ct_{j+1,f[j+1]\oplus 1})\la \Enc(\pk_{j+1,f[j+1]\oplus 1},m_b[j+1])$ and sends $\ct_{j+1,f[j+1]\oplus 1}$ to $\cB$.
    \item $\cB$ sends $(\{\sk_{i,f[i]}\}_{i\in [s]}, \{\ct_{i,f[i]\oplus 1}\}_{i\in[s]})$ to $\cA_1$.
    \item $\cA_1$ sends $\{\cert_i\}_{i\in[s]}$ to $\cB$, and sends its internal state to $\cA_2$.
    \item $\cB$ sends $\cert_{j+1}$ to the challenger, and receives $\sk_{j+1,f[j+1]\oplus1}$ or $\bot$ from the challenger.
    If $\cB$ receives $\bot$ from the challenger, it outputs $\bot$ and aborts.
    \item $\cB$ sends $\{\sk_{i,f[i]\oplus 1}\}_{i\in[s]}$ to $\cA_2$.
    \item $\cA_2$ outputs $b'$.
    \item $\cB$ computes $\Vrfy$ for all $\cert_i$, and outputs $b'$ if all results are $\top$. Otherwise, $\cB$ outputs $\bot$.
\end{enumerate}
Since $\pk_{j+1,\beta}$ and $\pk_{j+1,\beta\oplus 1}$ are identically distributed, 
it holds that
$ \Pr[f[j+1]=\beta]=\Pr[f[j+1]=\beta\oplus 1]=\frac{1}{2}$.
If $b=0$ and $f[j+1]=\beta\oplus 1$, $\cB$ simulates $\sfhyb{j}{}$.
Therefore, we have
\begin{align}
\Pr[1\la\cB|b=0]&=\Pr[1\la\cB \wedge f[j+1]=\beta\oplus 1|b=0]\\
                &=\Pr[1\la\cB|b=0, f[j+1]=\beta \oplus 1]\cdot\Pr[f[j+1]=\beta \oplus 1]\\
                &=\frac{1}{2}\Pr[\sfhyb{j}{}=1].
\end{align}
If $b=1$ and $f[j+1]=\beta\oplus 1$, $\cB$ simulates $\sfhyb{j+1}{}$.
Similarly, we have 
$
\Pr[1\la\cB|b=1]=\frac{1}{2}\Pr[\sfhyb{j+1}{}=1]
$.
By assumption, $\abs{\Pr[\sfhyb{j}{}=1]-\Pr[\sfhyb{j+1}{}=1]}$ is non-negligible, and therefore
$\abs{\Pr[1\la\cB|b=0]-\Pr[1\la\cB|b=1]}$ is non-negligible, which contradicts the certified everlasting IND-CPA security of $\Sigma$.
\end{proof}
